Eigenpolytopes, Spectral Polytopes and Edge-Transitivity

Starting from a finite simple graph $G$, for each eigenvalue $\theta$ of its adjacency matrix one can construct a convex polytope $P_G(\theta)$, the so called $\theta$-eigenpolytop of $G$. For some polytopes this technique can be used to reconstruct the polytopes from its edge-graph. Such polytopes (we shall call them spectral) are still badly understood. We give an overview of the literature for eigenpolytopes and spectral polytopes. We introduce a geometric condition by which to prove that a given polytope is spectral (more exactly, $\theta_2$-spectral). We apply this criterion to the edge-transitive polytopes. We show that every edge-transitive polytope is $\theta_2$-spectral, is uniquely determined by this graph, and realizes all its symmetries. We give a complete classification of distance-transitive polytopes.

==> sec/eigenpolytopes.tex <==

\tempnewpage

\section{Motivation}
\label{sec:motivation}

We dive into three curious topics in the interplay between graphs and polytopes, all of which will be addressed in this paper.

\subsection{Reconstructing polytopes from the edge-graph}
\label{sec:reconstructing_polytopes}

Since Steinitz \cite{...} it is known that the edge-graphs of polyhedra are exactly the 3-connected planar graphs, and that any such graph belongs to a unique combinatorial type of polyhedra.
On the other hand, the study of higher-dimensional polytopes taught us that the edge-graph carries very little information about its polytope if $d\ge 4$.

For example, the edge-graph of any simplex is the complete graph.
But so is the edge-graph of every \emph{neighborly polytope}, and so, given only the edge-graph, we will never know from which polytope it was obtained initially.
The same example shows that in many cases not even the dimension of the polytope can be reconstructed.

As a light in the dark, we have the result of Blind and Mani \cite{...} (with its modern proof from Kalai \cite{kalai1988simple}), which states that the combinatorial type of a \emph{simple polytope} can be reconstructed from its edge-graph.
One can then ask what other classes of polytopes allow such a unique reconstruction.
For example, it might be that every \enquote{sufficiently symmetric} polytope is reconstructable in this sense.
%
\begin{question}\label{q:symmetrc_polytopes_with_same_edge_graph}
Can there be two distinct sufficiently symmetric polytopes with the same edge-graph?
\end{question}
%
One might ask \enquote{what counts as sufficient symmetric?}, and this paper shall answer this question partially.
%
%\cref{q:symmetrc_polytopes_with_same_edge_graph} is trivially satisfied for regular polytopes, and the question is not very interesting for this very restrictive symmetry class.
%On the other end of the spectrum
For example, vertex-transitivity is not sufficient:
every~even-dimen\-sional \emph{cyclic polytope} $C(n,2d)$ is neighborly and can be realized in a vertex-transitive way: set the coordinates of the $i$-th vertex to be
%
$$\big(\sin(t_i),\cos(t_i);\sin(2t_i),\cos(2t_i);...;\sin(dt_i),\cos(dt_i)\big)\in\RR^{2d}$$
%
with $t_i=2\pi i/n$. The edge-graph is $K_n$, independent of $d$.

The next candidate in line, \emph{edge-transitivity}, seems more promising.
%Even more, the edge-graph seems to determine edge-transitive polytopes not only up to combinatorial equivalence, but even up to orientation and scale.
And while a complete classification of edge-transitive polytopes might be possible (though, none is currently known), a more satisfying outcome would be a result independent of any such classification.


\subsection{Realizing symmetries of the edge-graph}
\label{sec:realizing_symmetries}

Polytopes are at most as symmetric as there edge-graph.


Any symmetry $T\in\Aut(P)\subset\Ortho(\RR^d)$ of a polytope $P\subset\RR^d$ induces a symmetry $\phi\in\Aut(G_P)\subseteq\Sym(n)$ of the edge-graph.
And thus $\Aut(P)\le\Aut(G_P)$ as abstract groups.

For general polytopes, it cannot be expected that the polytope shows many, or just any symmetries of the edge-graph.
However, one can always try to find a sufficiently symmetric realization of the polytope, so that a maximum of combinatorial symmetries of the edge-graph is realized as geometric symmetries of the polytope.
One can even hope to realize \emph{all} the symmetries of the edge-graph.

In the case of polyhedra, the circle packing version of the Steinitz theorem provides a way to realize all the symmetries of the edge-graph.
Again, higher dimensions tell a different story: there exist 4-dimensional polytopes with edge-graphs that can never be realized as polytopes the edge-graphes of which cannot be realized with all their symmeteries (consider \eg\ the dual of the polytope constructed in \cite{bokowski1984combinatorial}).

Again, it seems that assuming sufficient symmetry of the polytope ensures that the polytope has already \emph{all} the symmetries of its edge-graph.
We can actually proof this in the case of so called \emph{distance-transitive} symmetry, and we hope to find the same in the case of only edge-transitive polytopes.

\begin{question}
Does every sufficiently symmetric polytope realize all the symmetries of its edge-graph?
\end{question}


\subsection{Rigidity and perfect polytopes}
\label{sec:rigid_perfect}

Every polytope can be continuously deformed while preserving its combinatorial type.
In the case of highly symmetric polytopes, one might be additionally interesting in keeping the symmetry properties during the deformation.
A polytope that cannot be deformed without loosing any of its symmetries is be called \emph{rigid} or, occasionally, a \emph{perfect polytope}.

All regular polytopes are examples of such rigid polytopes, and there exist many more.
While quite some examples are known, no general construction procedures has been described.
Again, one might hope to show that all sufficiently symmetric polytopes are rigid, in particular, the edge-transitive polytopes.

%A polytope $P\subset\RR^d$ is called \emph{perfect} if it is the unique most symmetric realization of its combinatorial type.

\begin{question}
Is every sufficiently symmetric polytope rigid?
\end{question}


%\subsection{Spectral graph theory}
%\label{sec:spectral_graph_theory}
%
%Let $P\subset\RR^d$ be your favorite highly symmetric polytope.
%For example, let $P$ be a Platonic solid, as the regular icosahedron.


\subsection{A motivating example}
\label{sec:motivating_example}

Consider your favorite highly symmetric polytope $P\subset\RR^d$.
For demonstration, we choose $P$ to be the \emph{regular dodecahedron}\footnote{Any other platonic solid (or regular polytope) might do the trick. Ideally, your polytope is transitive on vertices and edges.}
%The relevant properties here are that $P$ is inscribed into a sphere of radius $r$, and that all edges are of the same length, say 1.
%So surely, any other regular polytope would fit as well, and many more examples exist in higher dimensions.

Here are some observations:
%
\begin{myenumerate}
	\item $P$ is really symmetric (it is a regular polyhedron). All its symmetries must also be reflected in the edge-graph $G_P$, since any automorphism of $P$ restricts to an automorphism of $G_P$.
	However, it is far from evident whether any particular symmetry of $G_P$ is reflected in $P$ as well? 
	In the case of the dodecahedron, every combinatorial symmetry of the edge-graph is indeed a geomery symmetry of $P$.
	\item The study of higher dimensional polytopes teaches that the edge-graph of a polytope carries usually very little information about the polytope itself.
	For example, the edge-graph of a simplex is a complete graph.
	But so are the edge-graph of all \emph{neighborly polytopes}.
	It was shown in \cite{kalai1988simple} that this problem of reconstruction does not happen for \emph{simple polytopes}, and it is our goal to show that this is also not to be expected for sufficiently symmetric polytope.
	\item A polytope is called \emph{perfect} if its combinatorial type has a unique geometric realization of highest symmetry.
	Many highly symmetric polytopes one immediately thinks about have this property. But many other do not.
	We show that being edge-transitive seems to be the right assumption to ensure being perfect.
\end{myenumerate}







\tempnewpage
\section{Eigenpolytopes and spectral polytopes}
%\label{sec:eigenpolytopes}

One way to connect spectral graph theory to polytope theory is via the construction of the so-called \emph{eigenpolytopes}.
In this section, we will survey this construction and its application primarily to the study of highly symmetric graphs.




%\subsection{Some terminology for polytopes}

From this section on, let $P\subset\RR^d$ denote a $d$-dimensio\-nal convex polytope with $d\ge 2$.
If not stated otherwise, we shall~assume that $P$ is \emph{full-dimensional}, that is, that $P$ is not contained in any proper subspace of $\RR^d$.

Let $\F_\delta(P)$ denote the set of \emph{$\delta$-dimensional faces} of $P$.
Fix some bijection $v\: V\to \F_0(P)$ between $V=\{1,...,n\}$ and the vertices of $P$.
Let $G_P=(V,E)$ be the graph with $ij\in E$ if and only if $\conv\{v_i,v_j\}$ is an edge of $P$.
$G_P$ is called \emph{edge-graph} of $P$, and $v$ the \emph{skeleton} of $P$.
Note that we can consider $v$ as a realization of $G_P$.

%Any unexplained terminology on polytopes can be found in \cite{ziegler2012lectures}.




%The \emph{edge-graph} $G_P$ of $P$ is the graph with vertex set $\F_0(P)$,~and $v,w\in\F_0(P)$ are adjacent in $G_P$ if and only if $\conv\{v,w\}\subseteq P$ is an edge of $P$.
%It is mostly inconvenient that the vertices of $G_P$ are actual points in space, and so we assume that we are actually working with an isomorphic copy of $G_P$ whose vertex set is $V=\{1,...,n\}$.
%This also provides a standard enumeration of the vertices of $P$.
%
%\begin{definition}
%The \emph{skeleton} of $P$ is the realization of $G_P$ that to each \mbox{(graph-)} vertex $i\in V$ in the edge-graph assignes the respective (polytope-)vertex of $P$ (according to the standard enumeration mentioned above).
%\end{definition}
%
%If $v$ is the skeleton of $P$, then $v_i$ is the $i$-th vertex of $P$.



\subsection{Eigenpolytopes}


\begin{definition}
Given a graph $G$ and an eigenvalue $\theta\in \Spec(G)$ of multiplicity $d$. If $v$ is the $\theta$-realization of $G$, then
	%
	$$P_G(\theta):=\conv\{v_i\mid i\in V\}\subset\RR^d$$
	%
	is called \emph{$\theta$-eigenpolytope} of $G$, or just \emph{eigenpolytope} if $\theta$ is not specified.
\end{definition}

The notion of the eigenpolytope goes back to Godsil \cite{godsil1978graphs}, and can~be under\-stood~as a geometric way to study the combinatorial, algebraic~and~spectral properties of a graph.

Several authors investigated the eigenpolytopes of famous graphs or graph families.
For example, Powers \cite{powers1986petersen} gave a description for the face structure of~the~different eigenpolytopes of the Petersen graph, one of which will reappear as distance-transitive polytope in \cref{sec:distance_transitive_polytopes}.
Mohri \cite{mohri1997theta_1} analysed the geometry of the, what he called, \emph{Hamming polytopes}, the $\theta_2$-eigenpolytopes of the Hamming graphs.
As it turns out, but was not realized by himself, these polytopes are merely the cartesian products of regular simplices.
These, as well, are distance-transitive~\mbox{polytopes}. Powers \cite{powers1988eigenvectors} took a first look at the eigenpolytopes of the \emph{distance-regular} graphs. 
Those especially will be discussed in greater detail below.

Finally, Padrol and Pfeifle \cite{padrol2010graph} investigated graph operations and their effect on the associated eigenpolytopes.

Before we proceed, we recall the relevant terminology for polytopes.



\subsection{Spectral polytopes}

Most graphs are not edge-graphs of polytopes (so-called \emph{polytopal} graphs), but eigenpolytope provide an operation that to every graph (and an eigenvalue thereof) assignes such a polytopal graph (the edge-graph of the eigenpolytope).

This operation is most interesting in the case of vertex-transitive graphs.
If $G$ is a vertex-transitive graph on $n$ vertices, every vertex of $G$ becomes a vertex of $P_G(\theta)$ (though maybe several vertices are assgined to the same point).

It seems interesting to ask for when this operation is a fixed point, that is, when is the edge-graph of the eigenpolytope isomorphic to the original graph.



%Eigenpolytopes are also linked to a bunch of open question: for example, which polytopes appear as eigenpolytopes.
%By a slight generalization it is possible to show that \emph{every} polytope appeasr as the eigenpolytope of its edge-graph, when we allow that the non-zero entries of the adjacency matrix are weighted appropriately \cite{izmestiev2010colin}.
%This approach is less relevant in our case, as weighting the matrix might destroy the symmetries formerly present.
%
We are specifically interested in one particular phenomenon associated with eigenpolytopes, that can best be observed in our running example.

%\begin{example}
%Dodecahedral graph.
%\end{example}

\begin{definition}
\quad %Given a polytope $P\subset\RR^d$.
\begin{myenumerate}
	\item A polytope $P$ is called \emph{balanced} \resp\ \emph{spectral}, if this is the case for its skeleton.
	\item A graph is called \emph{spectral} if it is the edge-graph of a spectral polytope.
\end{myenumerate}
\end{definition}

For a polytope, being spectral seems to be a quite exceptional property.
For example, being spectral implies that the polytope realizes all the symmetries of its edge-graph.
So, no neighborly polytope except for the simplex can be spectral.
In contrast, all (centered) neighborly polytopes are balanced, and many neighborly polytopes are eigenpolytopes (\eg\ one of the Petersen-polytopes is neighborly).

If a graph is spectral to eigenvalue $\theta$, then  it is isomorphic to the edge-graph of its $\theta$-eigenpolytop.
However, the converse is not true: the $\theta_3$-realization of the pentagon-graph is a pentagram, whose convex hull is a pentagon. But the pentagon-graph is not $\theta_3$-spectral.
%
\begin{center}
\includegraphics[width=0.7\textwidth]{img/convex_hull_5_gon}
\end{center}

\begin{example}
Every neighborly polytope has eigenvalue $-1$  (if centered appropriately), but none of these is spectral, except for the simplices.
\end{example}

\begin{example}
It is an easy exercise to show that the $d$-cubes and $d$-crosspolytopes are spectral with eigenvalue $\theta_2$.
In fact, it was shows by Licata and Power \cite{licata1986surprising} that also the regular polygons, all simplices, the regular dodecahedron and the regular icosahedron are spectral in this sense.

The only regular polytopes which they were not able to prove spectral were the 24-cell, 120-cell and 600-cell.
However, they conducted numerical experiments hinting in that direction.
\end{example}

%This definition is similar to Powers \emph{self-reproducing} graphs and polytopes~(though the intention might have been the same).
%In Powers original definition, a polytope is called self-reproducing, if it is isomorphic to some eigenpolytope of its edge-graph.
%This is slightly distinct: the image below shows that the regular pentagon is the $\theta_2$- and $\theta_3$-eigenpolytope of its edge-graph.
%%
%\begin{center}
%\includegraphics[width=0.4\textwidth]{img/convex_hull_5_gon}
%\end{center}
%
%
%This definition does probably convey the right mental image, but nevertheless, is quite subtle.
%Consider the following two, actually weaker versions of part $(i)$ of~the definition above:
%%
%\begin{itemize}
%	\item A polytope that is an eigenpolytope of its edge-graph.
%	\item A polytope that is combinatorially equivalent to an eigenpolytope of its edge-graph.
%\end{itemize}

\msays{The $\theta_3$-realization of the cube-graph is a polytope (the tetrahedron) and its edges correspond to edges of the graph, but it is not faithful.}

%\textbf{Facts about eigenpolytopes:}
%\begin{itemize}
%	\item Ismeziev
%	\item Petersen polytopes
%	\item Hamming polytopes
%	\item Blue
%	\item Godsil: distance regular polytopes
%	\item Padrol: operations
%	\item self-reproducing polytopes (Powers)
%\end{itemize}

In a slightly more general setting, Izmestiev \cite{izmestiev2010colin} found that every polytope is~spectral, if we are allowed to add appropriate edge-weights to the edge-graph.
This~results in an adjacency matrix whose entries can be any non-negative real number instead of just zero and one.
This however might break the symmetry in a combinatorially highly symmetric graph and is therefore not our preferred perspective.

First results on this topic were obtained by Licata and Powers \cite{licata1986surprising}, who indentified several polytopes as being spectral.
Among these, all regular polytopes, excluding the exceptional 4-dimensional regular polytopes: 24-cell, 120-cell and 600-cell.

Still kind of \enquote{unexplained} is their finding that the \emph{rhombic dodecahedron} is spectral as well.
Since the edge graph of this polyhedron is not regular, this observation hinges critically on the fact that we consider eigenpolytopes constructed from the adjacency matrix, rather than, say, the Laplace matrix.

Godsil \cite{godsil1998eigenpolytopes} classified all spectral graphs among the distance-regular graphs (for a definition, see \cref{sec:distance_transitive_realizations}). 
He found that these are the following:

\begin{theorem}[Godsil, \cite{...}]
\label{res:spectral_distance_regular_graphs}
Let $G$ be a distance-regular graph. 
If $G$ is $\theta_2$-spectral,~then $G$ is one of the following:
%
\begin{enumerate}[label=$(\text{\roman*}\,)$]
	\item a cycle graph $C_n,n\ge 3$,
	\item the edge-graph of the dodecahedron,
	\item the edge-graph of the icosahedron,
	\item the complement of a disjoint union of edges,
	\item a Johnson graph $J(n,k)$,
	\item a Hamming graph $H(d,q)$,
	\item a halved $n$-cube $\nicefrac12 Q_n$,
	\item the Schläfli graph, or
	\item the Gosset graph.
\end{enumerate}
\end{theorem}

One remarkable fact about this list, which seems to have gone unnoticed, is that all these graphs are actually \emph{distance-transitive}.

In general there was not found a single polytope (or graph) that is $\theta_i$-spectral for any $i\not=2$ (assuming that the graph has at least one edge).
It is not implausible to conjecture that skeleta of polytopes can have, if at all, only eigenvalue $\theta_2$.
This comes from the study of so-called \emph{nodal domains}.

%\begin{theorem}
%If the skeleton of a polytope has an eigenvalue, then this eigenvalue is $\theta_2$.
%%
%\begin{proof}
%\TODO
%\end{proof}
%\end{theorem}


There is a remarkable construction due to Izmestiev \cite{izmestiev2010colin}.

\begin{theorem}[Izmestiev \cite{izmestiev2010colin}, Theorem 2.4]\label{res:izmestiev}
Let $P\subset\RR^d$ be a polytope, $G_P$ its~edge-graph and $v\:V\to\RR^d$ its skeleton. For $c=(c_1,...,c_n)\in\RR^n$ define
%
$$P^\circ(c):=\{x\in\RR^d\mid\<x,v_i\>\le c_i\text{ for all $i\in V$}\}.$$
%
Note that $P^\circ=P^\circ(1,...,1)$ is the polar dual of $P$.
The matrix $X\in\RR^{n\x n}$ with~compo\-nents
%
$$X_{ij}:=-\frac{\partial^2 \vol(P^\circ(c))}{\partial c_i\partial c_j}\Big|_{c=(1,...,1)}$$
%
has the following properties:
%
\begin{myenumerate}
	%\item whenever $ij\in E$, and $\sigma_i,\sigma_j\in\F_{d-1}(P^\circ)$ are the dual faces to $v_i$ \resp\ $v_j$ in the dual polytope $P^\circ=P^\circ(1,...,1)$, 
	%then
	%
	%$$X_{ij}=\frac{\vol(\sigma_i\cap\sigma_j)}{\|v_i\|\|v_j\|\sin\angle(v_i,v_j)},$$
	
	\item $X_{ij}< 0$ whenever $ij\in E(G_P)$,
	\item $X_{ij}=0$  whenever $ij\not\in E(G_P)$,
	%\item $X_{ii}> 0$ for all $i\in V(G_P)$,
	\item $XM=0$, where $M$ is the arrangement matrix of $v$,
	\item $X$ has a unique negative eigenvalue, and this eigenvalue is simple,
	\item $\dim\ker X=d$.
\end{myenumerate}
\end{theorem}

One can view the matrix $X$ (or better, $-X$) as kind of an adjacency matrix of~a vertex- and edge-weighted version of $G_P$.
Part $(iii)$ states that $v$ is balanced~with eigenvalue zero.
Since $\rank M=d$, part $(v)$ states that the arrangement space~$U:=$ $\Span M$ is already the whole eigenspace.
And part $(iv)$ states that zero is the second largest eigenvalue of $-X$.


\begin{theorem}\label{res:implies_spectral}
Let $P\subset\RR^d$ be a polytope, and $X\in\RR^{n\x n}$ the associated matrix~defined as in \cref{res:izmestiev}. If we have that
%
\begin{myenumerate}
	\item $X_{ii}$ is independent of $i\in V(G_P)$, and
	\item $X_{ij}$ is independent of $ij\in E(G_P)$,
\end{myenumerate}
%
then $P$ is spectral with eigenvalue $\theta_2$.
%
\begin{proof}
By assumption there are $\alpha,\beta\in\RR$, $\beta>0$, so that $X_{ii}=\alpha$ for all vertices~$i\in$ $V(G_P)$, and $X_{ij}=-\beta$ for all edges $ij\in E(G_P)$.
We then find
%
$$X=\alpha \Id - \beta A\quad\implies\quad (*)\;A=\frac\alpha\beta \Id-\frac1\beta X,$$
%
where $A$ is the adjacency matrix of $G_P$.
By \cref{res:izmestiev} $(iv)$ and $(v)$, the matrix $X$ has second smallest eigenvalue zero of multiplicity $d$.
By \cref{res:izmestiev}  $(iii)$, the columns of $M$ are the corresponding eigenvectors.
Since $\rank M=d$ we find that these are all the eigenvectors, in particular, that the arrangement space $U:=\Span M$ is the 0-eigenspace of $X$.

By $(*)$, $A$ (that is, $G_P$) has then second \emph{largest} eigenvalue $\theta_2=\alpha/\beta$ of multiplicity $d$ with eigenspace $U$.
The skeleton of $P$ is then the $\theta_2$-realization of $G_P$ and $P$ is spectral.
\end{proof}
\end{theorem}

\begin{corollary}
If $P\subset\RR^d$ is simultaneously vertex- and edge-transitive, then $P$ is spectral with eigenvalue $\theta_2$.
\end{corollary}


It seems tempting to conjecture that the spectral polytopes are \emph{exactly} the polytopes that satisfy the conditions $(i)$ and $(ii)$ in \cref{res:implies_spectral}.
This would give an interesting geometric characterization of eigenpolytopes.
Izmestiev proved the following:
for $ij\in E$ let $\sigma_i,\sigma_j\in\F_{d-1}(P^\circ)$ be the dual facets to the vertices $v_i$ and $v_j$ in $P$. Then holds
%
$$X_{ij}= \frac{\vol_{d-2}(\sigma_i\cap\sigma_j)}{\|v_i\|\|v_j\|\sin\angle(v_i,v_j)}.$$
%
There seems to be no equally elementary formula for $X_{ii},i\in V$, but its value can be derived from $XM=0$, which implies
%
$$X_{ii} v_i = -\sum_{\mathclap{j\in N(i)}} M_{ij} v_j.$$

It seems out of reach to prove this fact.
There are many balanced polytopes that are not spectral (\eg\ all appropriately centered neighborly polytopes that are not simplices).
Further, there are polytope for which being spectral appears completely exceptional, \eg\ the \emph{rhombic dodecahedron} (already mentioned by Licata and Powers \cite{licata1986surprising}).



\subsection{Applications}

Spectral polytopes turn out to be exactly the kind of polytopes we need to address the problems listed in \cref{sec:motivation}.

For example, for fixed $i\in\NN$ consider the set of all $\theta_i$-spectral polytopes.
Given the edge-graph $G_P$ of some polytope in this set, this uniquely determines the polytope, simply since it can be reconstruced via the $\theta_i$-realizaion of $G_P$.
In other~words, the $\theta_i$-spectral polytopes are uniquely determined by their edge-graph.

Also, each $\theta_i$-spectral polytope realizes all the symmetries of its edge-graph by \cref{res:spectral_implies_symmetric}.

The question then is how large the class of these polytopes is, and whether their members are easily recognized.
For example, has every family of vertex-transitive polytopes with the same edge graph a spectral representative?
If so, this would imply that every vertex-transitive edge-graph can be realized as a polytope with all symmetries.



\section{Edge-transitive polytopes}

\subsection{Arc-transitive polytopes}
\label{sec:arc_transitive_polytopes}

Our final goal would be to establish that every arc-transitive polytope is spectral, or more precisely, $\theta_2$-spectral.
To anticipate~
the outcome, we were not able to prove this.
However, we also observe that this statement is true for \emph{all} known arc-transitive polytopes.

In the last section we have learned that the skeleton of an arc-transitive polytope is of full local dimension, hence irreducible, spherical, rigid and has an eigenvalue.

\begin{definition}
Given a polytope $P\subset\RR^d$.
\begin{myenumerate}
	\item $P$ is called \emph{rigid} if it cannot be continuously deformed without changing its combinatorial type or symmetry group.
	\item $P$ is called \emph{perfect} if any essentially distinct but combinatorially equivalent polytope $Q\subset\RR^d$ has a smaller symmetry group than $P$, that is $\Aut(Q)\subset\Aut(P)$.
\end{myenumerate}
\end{definition}

\enquote{Essentially distinct} in $(ii)$ means that $P$ and $Q$ are not just reoriented or~rescaled versions of one another.

If a polytope is perfect, then it is rigid.
It seems to be open whether the converse holds in general.
In theory it could happen that a combinatorial type might have two \enquote{most symmetric} realizations as a polytope, and those cannot be continuously deformed into each other.



\begin{theorem}
An arc-transitive polytope $P\subset\RR^d$ is $\theta_2$-spectral.
%
\begin{proof}
The skeleton of $P$ is an arc-transitive realization of $G_P$ of full local dimension, hence has an eigenvalue $\theta\in\Spec(G)$ according to \cref{res:...}.
The tricky part is to show that $\theta=\theta_2$.

For this, we use the following fact:
Let $v$ be the skeleton of $P$ and define
%
$$P^\circ(\mathbf c) = P^\circ(c_1,...,c_n):=\{x\in\RR^d\mid \<x,v_i\>\le c_i\text{ for all $i\in V$}\}.$$
%
Finally, consider the matrix
%
$$M_{ij}:=-\frac{\partial^2\mathrm{vol}(P(\mathbf c))}{\partial c_i \partial c_j}\Big|_{\mathbf c=(1,...,1)}.$$
%
Since $P$ is edge-transitive, $M_{ij}$ contains the same value for all $ij\in E$.
Since $P$ is vertex-transitive, $M_{ii}$ does not depend in $i\in V$.
Finally, it is proven in \cite{...} that $M_{ij}=0$ whenever $ij\not\in E$, and that $M$ has a single negative eigenvalue which is simple.
Apparently, there are $\alpha,\beta\in\RR$ so that $M=\alpha A+\beta\Id$, where $A$ is the adjacency matrix of $M$.
\end{proof}
\end{theorem}


\begin{theorem}
If $P\subset\RR^d$ is an arc-transitive polytope, then
%
\begin{myenumerate}
	\item $P$ is rigid,
	\item $\Aut(P)$ is irreducible,
	\item any projection $\pi_U(P)$ onto a subspace $U\subseteq\RR^d$ is either not arc-transitive~or has a different edge-graph as $P$.
\end{myenumerate}
Furthermore, there is an eigenvalue $\theta\in\Spec(G_P)$ of the edge-graph $G_P$ \resp\ its~associated Laplacian eigenvalue $\lambda=\theta-\deg(G_P)$, so that the following holds:
\begin{myenumerate}
  \setcounter{enumi}{3}
	\item if $P$ has edge length $\ell$ and circumradius $r$, then
	%
	$$\frac\ell r=\sqrt{\frac{2\lambda}{\deg(G_P)}}.$$
	\item if the polar polytope $P^\circ$ has dihedral angle $\alpha$, then
	%
	$$\cos\alpha=-\frac{\theta}{\deg(G_P)}.$$
\end{myenumerate}
\end{theorem}

\begin{conjecture}\label{conj:arc_transitve}
Each arc-transitive polytope $P\subset\RR^d$ is $\theta_2$-spectral, and satisfies
%
\begin{myenumerate}
	\item $P$ is perfect,
	\item $P$ realizes all the symmetries of its edge-graph,
	\item $P$ is the only arc-transitive polytope (up to reorientation and rescaling) with edge-graph $G_P$.
\end{myenumerate}
\end{conjecture}

Probably in, in all these result, the eigenvalue $\theta$ \resp\ $\lambda$ can be replaced with $\theta_2$ \resp\ $\lambda_2$, but we were not able to prove that.
However, it holds in any single case of arc-transitive polytope that we have checked.

\begin{example}
There are many ways to compute the circumradius of an $n$-simplex with unit edge-length, and here is another one:

The complete graph $K_n$ is arc-transitive and has spectrum $\{(-1)^{n-1},n^1\}$. The second largest eigenvalue $\theta_2=-1$ gives rise to an $(n-1)$-dimensional polytope with edge-graph $K_n$, that is, the $(n-1)$-dimensional simplex.
Assuming edge length $\ell=1$, we can compute its circumradius:
%
$$r=\sqrt{\frac{\deg(G)}{\lambda_2}} = \sqrt{\frac{\deg(G)}{\deg(G)-\theta_2}} = \sqrt{\frac{n-1}{n-1-(-1)}} = \sqrt{1-\frac1n}.$$

\end{example}

\begin{example}
Compute the dihedral angle of the rhombic dodecahedron and the rhombic triacontahedron.
\end{example}

But this technique can also be used the other way around, namely, concluding from the knowledge of the metric properties of a polytope and the eigenvalues of its edge-graph to the fact that it is spectral.

\begin{example}
We show that all regular polytopes are in fact $\theta_2$-spectral, as was already conjectured by Licata and Powers \cite{licata1986surprising}.

The essential facts we are using are some tabulated metric and spectral properties of these polytopes, \eg\ found in \cite{buekenhout1998number}.

\begin{itemize}
\item
Remarkable, the 24-cell has edge-length $\ell$ identical to circumradius $r$.
This determines the Laplacian eigenvalue of its skeleton:
%
$$1=\frac\ell r=\sqrt{\frac{2\lambda}{\deg(G)}} \quad\implies\quad \lambda=\frac12\deg(G) = 4.$$
%
One checks  that $4$ is exactly the second largest Laplacian eigenvalue of its edge-graph, and that this eigenvalue  has multiplicity four.

\item
600-cell: $3(1+\sqrt{5})$

\item
120-cell: $2\phi-1$
\end{itemize}

\begin{center}
\begin{tabular}{c|rrrr}
polytope & $\ell$ & $r$ & $\lambda_2$ & $\deg(G_P)$ \\
\hline
$\overset{\phantom.}24$-cell & $1$ & $1$ & $4$ & $8$ \\
$120$-cell & $3-\sqrt 5$ & $2\sqrt 2$ & $2\phi-1$ &  $4$ \\
$600$-cell & $2/\phi$ & $2$ & $3(1+\sqrt 5)$ & $12$
\end{tabular}
\end{center}



\end{example}


\begin{theorem}
If a polytope has a connected, full-dimensional and spanning edge-orbit, then it is perfect.
\end{theorem}







\newpage

\section{Edge- and vertex-transitive polytopes}

The goal of this section is to show that every polytope $P\subset\RR^d$ that is simultane\-ously vertex- and edge-transitive is an eigenpolytope to the second smallest eigenvalue of its edge-graph.
Note that being only edge-transitive is just slightly weaker than being vertex- and edge-transitive, as it was shown in \cite{winter2020polytopes} that edge-transitivity of convex polytopes in dimension $d\ge 4$ implies vertex-transitivity anyway.


\begin{theorem}\label{res:vertex_edge_transitive_is_theta2_realization}
If $P\subset\RR^d$ is vertex-transitive and edge-transitive, then it is the~$\theta_2$-eigenpolytopes of its edge-graph.
%
\begin{proof}
Let $X\in\RR^{n\x n}$ be the matrix defined in \cref{res:izmestiev}.
Since $P$ is transitive on vertices, there is a number $\alpha\in\RR$ with $X_{ii}=\alpha$ for all $i\in V$.
Since $P$ is edge-transitive, there is a number $\beta<0$ so that $X_{ij}=\beta$ for all $ij\in E(G_P)$.
Since we also have $X_{ij}=0$ for all $ij\not\in E(G_P)$, we find that $X$ must be of the form
%
$$X= \alpha \Id - \beta A \quad\implies\quad A=\alpha\Id-\frac1\beta X,$$
%
where $A$ is the adjacency matrix of $G_P$.

$X$ has a single negative eigenvalue, which is simple, and $\dim\ker X=d$.
In other words, its second smallest eigenvalue is zero and has multiplicity $d$.
Consequently, $A$ has second \emph{largest} eigenvalue $\theta_2=\alpha$ of multiplicity $d$ to the same eigenvectors as $X$.

Let $v$ be the skeleton of $P$ with arranegment matrix $M$ and arrangement space $U$.
Since $XM=0$ and $\rank M=d$, we find that the $U=\Span M$ must be the $0$-eigenspace of $X$, hence the $\theta_2$-eigenspace of $A$.
Thus, $v$ is the $\theta_2$-realization of $G_P$ and $P$ is spectral.
\end{proof}
\end{theorem}

The argument of \cref{res:vertex_edge_transitive_is_theta2_realization} cannot be easily generalized to any weaker form of symmetry.
For example, one would like to proof that every spectral polytope has eigenvalue $\theta_2$, or more generally, every balanced polytope has eigenvalue $\theta_2$.

\begin{corollary}
If $P\subset\RR^d$ is vertex- and edge-transitive, then holds:
%
\begin{myenumerate}
	\item $\Aut(P)$ is irreducible,
	\item $P$ is the unique simultaneously vertex- and edge-transitive polytope for which the edge-graph is isomorphic to $G_P$,
	\item $P$ realizes all symmetries of its edge-graph,
	\item $P$ is a perfect (rigid) polytope,
	\item $P$ is the unique most symmetric realization of its combinatorial type,
	\item if $P$ has edge-length $\ell$ and circumradius $r$, then
	%
	$$\Big[\frac \ell r \Big]^2 = \frac{2\lambda_2(G_P)}{\deg(G_P)} = 2\Big(1-\frac{\theta_2(G_P)}{\deg(G_P)}\Big).$$
	%
	\item if the polar dual $P^\circ$ has dihedral angle $\alpha$, then
	%
	$$\cos(\alpha)=-\frac{\theta_2(G_P)}{\deg(G_P)}.$$
\end{myenumerate}
\end{corollary}





\section{Distance-transitive polytopes}

\subsection{Distance-transitive polytopes}
\label{sec:distance_transitive_polytopes}

In general, there is no apparent reason for why a spectral polytope must be $\theta_2$-spectral.
In the case of distance-transitive polytopes there can be found an easy argument involving the cosine sequence of its skeleton.
The argument is based on the number of sign changes in $u_\delta$ and the so called \emph{two-piece property} for embedded graphs.

\begin{definition}
A realization $v$ is said to have the \emph{two-piece property} (or TPP),~if every hyperplane cuts it into at most two pieces.
More formally, given any vector $x\in \RR^d$ and scalar $c\in\RR$, the induced subgraphs
%
$$
G_+:=G[\,i\in V\mid \<x,v_i\>\ge c\,]
\quad\text{and}\quad
G_-:=G[\,i\in V\mid \<x,v_i\>\le c\,]
$$
%
must be connected (if non-empty).
\end{definition}

The image below shows two symmetric realizations of the cycle graph $C_5$, one~of which has the TPP (left), and one of which has not (right).

%\begin{center}
%\includegraphics[width=0.5\textwidth]{img/5_gon_cut}
%\end{center}

We are going to use the following fact:

\begin{theorem}[\cite{...}, Theorem xx]
The skeleton of a polytope has the TPP.
%
\begin{proof}[Sketch of proof.]
Let $v$ be the skeleton of a polytope, $x\in\RR^d$ and $c\in \RR$.

Let $i_+\in V$ be the vertex which maximizes the functional $\<v_\cdot,x\>$.
By the simplex algorithm, every vertex on the \enquote{positive} side of the hyperplane $\<\cdot,x\>=c$ can reach $v_{i_+}$ by a path in the edge-graph that is non-decreasing in $\<v_\cdot,x\>$.
Hence the positive side is connected if non-empty.
Equivalently for the negative side.

\end{proof}
\end{theorem}

\begin{theorem}
A distance-transitive polytope $P$ is $\theta_2$-spectral.
%
\begin{proof}
Let $v$ be the full-dimensional and distance-transitive realization of $P$.
Since it is also arc-transitive, it has an eigenvalue (by \cref{cref:...}).
By \cref{res:...} it must then be the $\theta_k$-realization of $G_P$.

Now consider cutting $v$ by the hyperplane $v_i^\bot$ for some $i\in V$.
The number of components left after the cut is exactly one more than the number of sign changes of the cosine sequence $u_\delta$.
From \cref{res:...} we know that there are exactly $k-1$ sign changes for the $\theta_k$-realization, hence $k$ pieces after the cut.

Since $v$ is the skeleton of a polytope, we have the TPP, and $k\le 2$ pieces.
Since $v$ cannot be the trivial $\theta_1$-realization of $G_P$, it must be the $\theta_2$-realization, and $P$ the $\theta_2$-eigenpolytope.
\end{proof}
\end{theorem}

\begin{corollary}
Let $P$ be a distance-transitive polytope.
%
\begin{myenumerate}
	\item Among distance-transitive polytopes, $P$ is uniquely determined by its edge-graph.
	\item $P$ realizes all the symmetries of its edge-graph.
	\item $P$ is the unique most symmetric realization of its combinatorial type.
\end{myenumerate}
\end{corollary}

Godsil's classification of the $\theta_2$-spectral distance-regular graphs (see \cref{res:spectral_distance_regular_graphs}; all of which~turned out to be distance-transitive) allows a complete classification of distance-tran\-sitive polytopes.

\begin{theorem}\label{res:distance_transitive_classification}
If $P\subset\RR^d$ is a distance-transitive polytope, then it is one of the following:
%
\begin{enumerate}[label=$(\text{\roman*}\,)$]
	\item a regular polygon $(d=2)$,
	\item the regular dodecahedron $(d=3)$,
	\item the regular icosahedron $(d=3)$,
	\item a cross-polytopes, that is, $\conv\{\pm e_1,...,\pm e_d\}$ where $\{e_1,...,e_d\}\subset\RR^d$ is the standard basis of $\RR^d$,
	\item a hyper-simplex $\Delta(d,n)$, that is, the convex hull of all vectors $v\in\{0,1\}^{d+1}$ with exactly $k$ 1-s,
	\item a cartesian power of a regular simplex (this includes hypercubes),
	\item a demi-cube, that is, the convex hull of all vectors $v\in\{-1,1\}^d$ with~an~even number of 1-s,
	\item the $2_{21}$-polytope, also called Gosset-polytope $(d=6)$,
	\item the $3_{21}$-polytope, also called Schläfli-polytope $(d=7)$.
\end{enumerate}
%
The order of this list agrees with the list of graphs in \cref{res:spectral_distance_regular_graphs}.
\end{theorem}

Note that the list in \cref{res:distance_transitive_classification} contains many polytopes that are not regular, and contains all regular polytopes except for the 24-cell, 120-cell and 600-cell.
The distance-transitive polytopes thus form a distinct class of remarkably symmetric polytopes which is not immediately related to the class of regular polytopes.

Noteworthy however, is that all the distance-transitive polytopes are \emph{Wythoffian poly\-topes}, that is, they are orbit polytopes of finite reflection groups.
\Cref{fig:distance_transitive_Coxeter} shows the Coxeter-Dynkin diagrams of these polytopes.

\begin{figure}
\centering
\includegraphics[width=0.9\textwidth]{img/distance_transitive_Coxeter}
\caption{Coxeter-Dynkin diagrams of distance-transitive polytopes.}
\label{fig:distance_transitive_Coxeter}
\end{figure}


==> v.2 - arXiv/sec/eigenpolytopes.tex <==

\tempnewpage

\section{Motivation}
\label{sec:motivation}

We dive into three curious topics in the interplay between graphs and polytopes, all of which will be addressed in this paper.

\subsection{Reconstructing polytopes from the edge-graph}
\label{sec:reconstructing_polytopes}

Since Steinitz \cite{...} it is known that the edge-graphs of polyhedra are exactly the 3-connected planar graphs, and that any such graph belongs to a unique combinatorial type of polyhedra.
On the other hand, the study of higher-dimensional polytopes taught us that the edge-graph carries very little information about its polytope if $d\ge 4$.

For example, the edge-graph of any simplex is the complete graph.
But so is the edge-graph of every \emph{neighborly polytope}, and so, given only the edge-graph, we will never know from which polytope it was obtained initially.
The same example shows that in many cases not even the dimension of the polytope can be reconstructed.

As a light in the dark, we have the result of Blind and Mani \cite{...} (with its modern proof from Kalai \cite{kalai1988simple}), which states that the combinatorial type of a \emph{simple polytope} can be reconstructed from its edge-graph.
One can then ask what other classes of polytopes allow such a unique reconstruction.
For example, it might be that every \enquote{sufficiently symmetric} polytope is reconstructable in this sense.
%
\begin{question}\label{q:symmetrc_polytopes_with_same_edge_graph}
Can there be two distinct sufficiently symmetric polytopes with the same edge-graph?
\end{question}
%
One might ask \enquote{what counts as sufficient symmetric?}, and this paper shall answer this question partially.
%
%\cref{q:symmetrc_polytopes_with_same_edge_graph} is trivially satisfied for regular polytopes, and the question is not very interesting for this very restrictive symmetry class.
%On the other end of the spectrum
For example, vertex-transitivity is not sufficient:
every~even-dimen\-sional \emph{cyclic polytope} $C(n,2d)$ is neighborly and can be realized in a vertex-transitive way: set the coordinates of the $i$-th vertex to be
%
$$\big(\sin(t_i),\cos(t_i);\sin(2t_i),\cos(2t_i);...;\sin(dt_i),\cos(dt_i)\big)\in\RR^{2d}$$
%
with $t_i=2\pi i/n$. The edge-graph is $K_n$, independent of $d$.

The next candidate in line, \emph{edge-transitivity}, seems more promising.
%Even more, the edge-graph seems to determine edge-transitive polytopes not only up to combinatorial equivalence, but even up to orientation and scale.
And while a complete classification of edge-transitive polytopes might be possible (though, none is currently known), a more satisfying outcome would be a result independent of any such classification.


\subsection{Realizing symmetries of the edge-graph}
\label{sec:realizing_symmetries}

Polytopes are at most as symmetric as there edge-graph.


Any symmetry $T\in\Aut(P)\subset\Ortho(\RR^d)$ of a polytope $P\subset\RR^d$ induces a symmetry $\phi\in\Aut(G_P)\subseteq\Sym(n)$ of the edge-graph.
And thus $\Aut(P)\le\Aut(G_P)$ as abstract groups.

For general polytopes, it cannot be expected that the polytope shows many, or just any symmetries of the edge-graph.
However, one can always try to find a sufficiently symmetric realization of the polytope, so that a maximum of combinatorial symmetries of the edge-graph is realized as geometric symmetries of the polytope.
One can even hope to realize \emph{all} the symmetries of the edge-graph.

In the case of polyhedra, the circle packing version of the Steinitz theorem provides a way to realize all the symmetries of the edge-graph.
Again, higher dimensions tell a different story: there exist 4-dimensional polytopes with edge-graphs that can never be realized as polytopes the edge-graphes of which cannot be realized with all their symmeteries (consider \eg\ the dual of the polytope constructed in \cite{bokowski1984combinatorial}).

Again, it seems that assuming sufficient symmetry of the polytope ensures that the polytope has already \emph{all} the symmetries of its edge-graph.
We can actually proof this in the case of so called \emph{distance-transitive} symmetry, and we hope to find the same in the case of only edge-transitive polytopes.

\begin{question}
Does every sufficiently symmetric polytope realize all the symmetries of its edge-graph?
\end{question}


\subsection{Rigidity and perfect polytopes}
\label{sec:rigid_perfect}

Every polytope can be continuously deformed while preserving its combinatorial type.
In the case of highly symmetric polytopes, one might be additionally interesting in keeping the symmetry properties during the deformation.
A polytope that cannot be deformed without loosing any of its symmetries is be called \emph{rigid} or, occasionally, a \emph{perfect polytope}.

All regular polytopes are examples of such rigid polytopes, and there exist many more.
While quite some examples are known, no general construction procedures has been described.
Again, one might hope to show that all sufficiently symmetric polytopes are rigid, in particular, the edge-transitive polytopes.

%A polytope $P\subset\RR^d$ is called \emph{perfect} if it is the unique most symmetric realization of its combinatorial type.

\begin{question}
Is every sufficiently symmetric polytope rigid?
\end{question}


%\subsection{Spectral graph theory}
%\label{sec:spectral_graph_theory}
%
%Let $P\subset\RR^d$ be your favorite highly symmetric polytope.
%For example, let $P$ be a Platonic solid, as the regular icosahedron.


\subsection{A motivating example}
\label{sec:motivating_example}

Consider your favorite highly symmetric polytope $P\subset\RR^d$.
For demonstration, we choose $P$ to be the \emph{regular dodecahedron}\footnote{Any other platonic solid (or regular polytope) might do the trick. Ideally, your polytope is transitive on vertices and edges.}
%The relevant properties here are that $P$ is inscribed into a sphere of radius $r$, and that all edges are of the same length, say 1.
%So surely, any other regular polytope would fit as well, and many more examples exist in higher dimensions.

Here are some observations:
%
\begin{myenumerate}
	\item $P$ is really symmetric (it is a regular polyhedron). All its symmetries must also be reflected in the edge-graph $G_P$, since any automorphism of $P$ restricts to an automorphism of $G_P$.
	However, it is far from evident whether any particular symmetry of $G_P$ is reflected in $P$ as well? 
	In the case of the dodecahedron, every combinatorial symmetry of the edge-graph is indeed a geomery symmetry of $P$.
	\item The study of higher dimensional polytopes teaches that the edge-graph of a polytope carries usually very little information about the polytope itself.
	For example, the edge-graph of a simplex is a complete graph.
	But so are the edge-graph of all \emph{neighborly polytopes}.
	It was shown in \cite{kalai1988simple} that this problem of reconstruction does not happen for \emph{simple polytopes}, and it is our goal to show that this is also not to be expected for sufficiently symmetric polytope.
	\item A polytope is called \emph{perfect} if its combinatorial type has a unique geometric realization of highest symmetry.
	Many highly symmetric polytopes one immediately thinks about have this property. But many other do not.
	We show that being edge-transitive seems to be the right assumption to ensure being perfect.
\end{myenumerate}







\tempnewpage
\section{Eigenpolytopes and spectral polytopes}
%\label{sec:eigenpolytopes}

One way to connect spectral graph theory to polytope theory is via the construction of the so-called \emph{eigenpolytopes}.
In this section, we will survey this construction and its application primarily to the study of highly symmetric graphs.




%\subsection{Some terminology for polytopes}

From this section on, let $P\subset\RR^d$ denote a $d$-dimensio\-nal convex polytope with $d\ge 2$.
If not stated otherwise, we shall~assume that $P$ is \emph{full-dimensional}, that is, that $P$ is not contained in any proper subspace of $\RR^d$.

Let $\F_\delta(P)$ denote the set of \emph{$\delta$-dimensional faces} of $P$.
Fix some bijection $v\: V\to \F_0(P)$ between $V=\{1,...,n\}$ and the vertices of $P$.
Let $G_P=(V,E)$ be the graph with $ij\in E$ if and only if $\conv\{v_i,v_j\}$ is an edge of $P$.
$G_P$ is called \emph{edge-graph} of $P$, and $v$ the \emph{skeleton} of $P$.
Note that we can consider $v$ as a realization of $G_P$.

%Any unexplained terminology on polytopes can be found in \cite{ziegler2012lectures}.




%The \emph{edge-graph} $G_P$ of $P$ is the graph with vertex set $\F_0(P)$,~and $v,w\in\F_0(P)$ are adjacent in $G_P$ if and only if $\conv\{v,w\}\subseteq P$ is an edge of $P$.
%It is mostly inconvenient that the vertices of $G_P$ are actual points in space, and so we assume that we are actually working with an isomorphic copy of $G_P$ whose vertex set is $V=\{1,...,n\}$.
%This also provides a standard enumeration of the vertices of $P$.
%
%\begin{definition}
%The \emph{skeleton} of $P$ is the realization of $G_P$ that to each \mbox{(graph-)} vertex $i\in V$ in the edge-graph assignes the respective (polytope-)vertex of $P$ (according to the standard enumeration mentioned above).
%\end{definition}
%
%If $v$ is the skeleton of $P$, then $v_i$ is the $i$-th vertex of $P$.



\subsection{Eigenpolytopes}


\begin{definition}
Given a graph $G$ and an eigenvalue $\theta\in \Spec(G)$ of multiplicity $d$. If $v$ is the $\theta$-realization of $G$, then
	%
	$$P_G(\theta):=\conv\{v_i\mid i\in V\}\subset\RR^d$$
	%
	is called \emph{$\theta$-eigenpolytope} of $G$, or just \emph{eigenpolytope} if $\theta$ is not specified.
\end{definition}

The notion of the eigenpolytope goes back to Godsil \cite{godsil1978graphs}, and can~be under\-stood~as a geometric way to study the combinatorial, algebraic~and~spectral properties of a graph.

Several authors investigated the eigenpolytopes of famous graphs or graph families.
For example, Powers \cite{powers1986petersen} gave a description for the face structure of~the~different eigenpolytopes of the Petersen graph, one of which will reappear as distance-transitive polytope in \cref{sec:distance_transitive_polytopes}.
Mohri \cite{mohri1997theta_1} analysed the geometry of the, what he called, \emph{Hamming polytopes}, the $\theta_2$-eigenpolytopes of the Hamming graphs.
As it turns out, but was not realized by himself, these polytopes are merely the cartesian products of regular simplices.
These, as well, are distance-transitive~\mbox{polytopes}. Powers \cite{powers1988eigenvectors} took a first look at the eigenpolytopes of the \emph{distance-regular} graphs. 
Those especially will be discussed in greater detail below.

Finally, Padrol and Pfeifle \cite{padrol2010graph} investigated graph operations and their effect on the associated eigenpolytopes.

Before we proceed, we recall the relevant terminology for polytopes.



\subsection{Spectral polytopes}

Most graphs are not edge-graphs of polytopes (so-called \emph{polytopal} graphs), but eigenpolytope provide an operation that to every graph (and an eigenvalue thereof) assignes such a polytopal graph (the edge-graph of the eigenpolytope).

This operation is most interesting in the case of vertex-transitive graphs.
If $G$ is a vertex-transitive graph on $n$ vertices, every vertex of $G$ becomes a vertex of $P_G(\theta)$ (though maybe several vertices are assgined to the same point).

It seems interesting to ask for when this operation is a fixed point, that is, when is the edge-graph of the eigenpolytope isomorphic to the original graph.



%Eigenpolytopes are also linked to a bunch of open question: for example, which polytopes appear as eigenpolytopes.
%By a slight generalization it is possible to show that \emph{every} polytope appeasr as the eigenpolytope of its edge-graph, when we allow that the non-zero entries of the adjacency matrix are weighted appropriately \cite{izmestiev2010colin}.
%This approach is less relevant in our case, as weighting the matrix might destroy the symmetries formerly present.
%
We are specifically interested in one particular phenomenon associated with eigenpolytopes, that can best be observed in our running example.

%\begin{example}
%Dodecahedral graph.
%\end{example}

\begin{definition}
\quad %Given a polytope $P\subset\RR^d$.
\begin{myenumerate}
	\item A polytope $P$ is called \emph{balanced} \resp\ \emph{spectral}, if this is the case for its skeleton.
	\item A graph is called \emph{spectral} if it is the edge-graph of a spectral polytope.
\end{myenumerate}
\end{definition}

For a polytope, being spectral seems to be a quite exceptional property.
For example, being spectral implies that the polytope realizes all the symmetries of its edge-graph.
So, no neighborly polytope except for the simplex can be spectral.
In contrast, all (centered) neighborly polytopes are balanced, and many neighborly polytopes are eigenpolytopes (\eg\ one of the Petersen-polytopes is neighborly).

If a graph is spectral to eigenvalue $\theta$, then  it is isomorphic to the edge-graph of its $\theta$-eigenpolytop.
However, the converse is not true: the $\theta_3$-realization of the pentagon-graph is a pentagram, whose convex hull is a pentagon. But the pentagon-graph is not $\theta_3$-spectral.
%
\begin{center}
\includegraphics[width=0.7\textwidth]{img/convex_hull_5_gon}
\end{center}

\begin{example}
Every neighborly polytope has eigenvalue $-1$  (if centered appropriately), but none of these is spectral, except for the simplices.
\end{example}

\begin{example}
It is an easy exercise to show that the $d$-cubes and $d$-crosspolytopes are spectral with eigenvalue $\theta_2$.
In fact, it was shows by Licata and Power \cite{licata1986surprising} that also the regular polygons, all simplices, the regular dodecahedron and the regular icosahedron are spectral in this sense.

The only regular polytopes which they were not able to prove spectral were the 24-cell, 120-cell and 600-cell.
However, they conducted numerical experiments hinting in that direction.
\end{example}

%This definition is similar to Powers \emph{self-reproducing} graphs and polytopes~(though the intention might have been the same).
%In Powers original definition, a polytope is called self-reproducing, if it is isomorphic to some eigenpolytope of its edge-graph.
%This is slightly distinct: the image below shows that the regular pentagon is the $\theta_2$- and $\theta_3$-eigenpolytope of its edge-graph.
%%
%\begin{center}
%\includegraphics[width=0.4\textwidth]{img/convex_hull_5_gon}
%\end{center}
%
%
%This definition does probably convey the right mental image, but nevertheless, is quite subtle.
%Consider the following two, actually weaker versions of part $(i)$ of~the definition above:
%%
%\begin{itemize}
%	\item A polytope that is an eigenpolytope of its edge-graph.
%	\item A polytope that is combinatorially equivalent to an eigenpolytope of its edge-graph.
%\end{itemize}

\msays{The $\theta_3$-realization of the cube-graph is a polytope (the tetrahedron) and its edges correspond to edges of the graph, but it is not faithful.}

%\textbf{Facts about eigenpolytopes:}
%\begin{itemize}
%	\item Ismeziev
%	\item Petersen polytopes
%	\item Hamming polytopes
%	\item Blue
%	\item Godsil: distance regular polytopes
%	\item Padrol: operations
%	\item self-reproducing polytopes (Powers)
%\end{itemize}

In a slightly more general setting, Izmestiev \cite{izmestiev2010colin} found that every polytope is~spectral, if we are allowed to add appropriate edge-weights to the edge-graph.
This~results in an adjacency matrix whose entries can be any non-negative real number instead of just zero and one.
This however might break the symmetry in a combinatorially highly symmetric graph and is therefore not our preferred perspective.

First results on this topic were obtained by Licata and Powers \cite{licata1986surprising}, who indentified several polytopes as being spectral.
Among these, all regular polytopes, excluding the exceptional 4-dimensional regular polytopes: 24-cell, 120-cell and 600-cell.

Still kind of \enquote{unexplained} is their finding that the \emph{rhombic dodecahedron} is spectral as well.
Since the edge graph of this polyhedron is not regular, this observation hinges critically on the fact that we consider eigenpolytopes constructed from the adjacency matrix, rather than, say, the Laplace matrix.

Godsil \cite{godsil1998eigenpolytopes} classified all spectral graphs among the distance-regular graphs (for a definition, see \cref{sec:distance_transitive_realizations}). 
He found that these are the following:

\begin{theorem}[Godsil, \cite{...}]
\label{res:spectral_distance_regular_graphs}
Let $G$ be a distance-regular graph. 
If $G$ is $\theta_2$-spectral,~then $G$ is one of the following:
%
\begin{enumerate}[label=$(\text{\roman*}\,)$]
	\item a cycle graph $C_n,n\ge 3$,
	\item the edge-graph of the dodecahedron,
	\item the edge-graph of the icosahedron,
	\item the complement of a disjoint union of edges,
	\item a Johnson graph $J(n,k)$,
	\item a Hamming graph $H(d,q)$,
	\item a halved $n$-cube $\nicefrac12 Q_n$,
	\item the Schläfli graph, or
	\item the Gosset graph.
\end{enumerate}
\end{theorem}

One remarkable fact about this list, which seems to have gone unnoticed, is that all these graphs are actually \emph{distance-transitive}.

In general there was not found a single polytope (or graph) that is $\theta_i$-spectral for any $i\not=2$ (assuming that the graph has at least one edge).
It is not implausible to conjecture that skeleta of polytopes can have, if at all, only eigenvalue $\theta_2$.
This comes from the study of so-called \emph{nodal domains}.

%\begin{theorem}
%If the skeleton of a polytope has an eigenvalue, then this eigenvalue is $\theta_2$.
%%
%\begin{proof}
%\TODO
%\end{proof}
%\end{theorem}


There is a remarkable construction due to Izmestiev \cite{izmestiev2010colin}.

\begin{theorem}[Izmestiev \cite{izmestiev2010colin}, Theorem 2.4]\label{res:izmestiev}
Let $P\subset\RR^d$ be a polytope, $G_P$ its~edge-graph and $v\:V\to\RR^d$ its skeleton. For $c=(c_1,...,c_n)\in\RR^n$ define
%
$$P^\circ(c):=\{x\in\RR^d\mid\<x,v_i\>\le c_i\text{ for all $i\in V$}\}.$$
%
Note that $P^\circ=P^\circ(1,...,1)$ is the polar dual of $P$.
The matrix $X\in\RR^{n\x n}$ with~compo\-nents
%
$$X_{ij}:=-\frac{\partial^2 \vol(P^\circ(c))}{\partial c_i\partial c_j}\Big|_{c=(1,...,1)}$$
%
has the following properties:
%
\begin{myenumerate}
	%\item whenever $ij\in E$, and $\sigma_i,\sigma_j\in\F_{d-1}(P^\circ)$ are the dual faces to $v_i$ \resp\ $v_j$ in the dual polytope $P^\circ=P^\circ(1,...,1)$, 
	%then
	%
	%$$X_{ij}=\frac{\vol(\sigma_i\cap\sigma_j)}{\|v_i\|\|v_j\|\sin\angle(v_i,v_j)},$$
	
	\item $X_{ij}< 0$ whenever $ij\in E(G_P)$,
	\item $X_{ij}=0$  whenever $ij\not\in E(G_P)$,
	%\item $X_{ii}> 0$ for all $i\in V(G_P)$,
	\item $XM=0$, where $M$ is the arrangement matrix of $v$,
	\item $X$ has a unique negative eigenvalue, and this eigenvalue is simple,
	\item $\dim\ker X=d$.
\end{myenumerate}
\end{theorem}

One can view the matrix $X$ (or better, $-X$) as kind of an adjacency matrix of~a vertex- and edge-weighted version of $G_P$.
Part $(iii)$ states that $v$ is balanced~with eigenvalue zero.
Since $\rank M=d$, part $(v)$ states that the arrangement space~$U:=$ $\Span M$ is already the whole eigenspace.
And part $(iv)$ states that zero is the second largest eigenvalue of $-X$.


\begin{theorem}\label{res:implies_spectral}
Let $P\subset\RR^d$ be a polytope, and $X\in\RR^{n\x n}$ the associated matrix~defined as in \cref{res:izmestiev}. If we have that
%
\begin{myenumerate}
	\item $X_{ii}$ is independent of $i\in V(G_P)$, and
	\item $X_{ij}$ is independent of $ij\in E(G_P)$,
\end{myenumerate}
%
then $P$ is spectral with eigenvalue $\theta_2$.
%
\begin{proof}
By assumption there are $\alpha,\beta\in\RR$, $\beta>0$, so that $X_{ii}=\alpha$ for all vertices~$i\in$ $V(G_P)$, and $X_{ij}=-\beta$ for all edges $ij\in E(G_P)$.
We then find
%
$$X=\alpha \Id - \beta A\quad\implies\quad (*)\;A=\frac\alpha\beta \Id-\frac1\beta X,$$
%
where $A$ is the adjacency matrix of $G_P$.
By \cref{res:izmestiev} $(iv)$ and $(v)$, the matrix $X$ has second smallest eigenvalue zero of multiplicity $d$.
By \cref{res:izmestiev}  $(iii)$, the columns of $M$ are the corresponding eigenvectors.
Since $\rank M=d$ we find that these are all the eigenvectors, in particular, that the arrangement space $U:=\Span M$ is the 0-eigenspace of $X$.

By $(*)$, $A$ (that is, $G_P$) has then second \emph{largest} eigenvalue $\theta_2=\alpha/\beta$ of multiplicity $d$ with eigenspace $U$.
The skeleton of $P$ is then the $\theta_2$-realization of $G_P$ and $P$ is spectral.
\end{proof}
\end{theorem}

\begin{corollary}
If $P\subset\RR^d$ is simultaneously vertex- and edge-transitive, then $P$ is spectral with eigenvalue $\theta_2$.
\end{corollary}


It seems tempting to conjecture that the spectral polytopes are \emph{exactly} the polytopes that satisfy the conditions $(i)$ and $(ii)$ in \cref{res:implies_spectral}.
This would give an interesting geometric characterization of eigenpolytopes.
Izmestiev proved the following:
for $ij\in E$ let $\sigma_i,\sigma_j\in\F_{d-1}(P^\circ)$ be the dual facets to the vertices $v_i$ and $v_j$ in $P$. Then holds
%
$$X_{ij}= \frac{\vol_{d-2}(\sigma_i\cap\sigma_j)}{\|v_i\|\|v_j\|\sin\angle(v_i,v_j)}.$$
%
There seems to be no equally elementary formula for $X_{ii},i\in V$, but its value can be derived from $XM=0$, which implies
%
$$X_{ii} v_i = -\sum_{\mathclap{j\in N(i)}} M_{ij} v_j.$$

It seems out of reach to prove this fact.
There are many balanced polytopes that are not spectral (\eg\ all appropriately centered neighborly polytopes that are not simplices).
Further, there are polytope for which being spectral appears completely exceptional, \eg\ the \emph{rhombic dodecahedron} (already mentioned by Licata and Powers \cite{licata1986surprising}).



\subsection{Applications}

Spectral polytopes turn out to be exactly the kind of polytopes we need to address the problems listed in \cref{sec:motivation}.

For example, for fixed $i\in\NN$ consider the set of all $\theta_i$-spectral polytopes.
Given the edge-graph $G_P$ of some polytope in this set, this uniquely determines the polytope, simply since it can be reconstruced via the $\theta_i$-realizaion of $G_P$.
In other~words, the $\theta_i$-spectral polytopes are uniquely determined by their edge-graph.

Also, each $\theta_i$-spectral polytope realizes all the symmetries of its edge-graph by \cref{res:spectral_implies_symmetric}.

The question then is how large the class of these polytopes is, and whether their members are easily recognized.
For example, has every family of vertex-transitive polytopes with the same edge graph a spectral representative?
If so, this would imply that every vertex-transitive edge-graph can be realized as a polytope with all symmetries.



\section{Edge-transitive polytopes}

\subsection{Arc-transitive polytopes}
\label{sec:arc_transitive_polytopes}

Our final goal would be to establish that every arc-transitive polytope is spectral, or more precisely, $\theta_2$-spectral.
To anticipate~
the outcome, we were not able to prove this.
However, we also observe that this statement is true for \emph{all} known arc-transitive polytopes.

In the last section we have learned that the skeleton of an arc-transitive polytope is of full local dimension, hence irreducible, spherical, rigid and has an eigenvalue.

\begin{definition}
Given a polytope $P\subset\RR^d$.
\begin{myenumerate}
	\item $P$ is called \emph{rigid} if it cannot be continuously deformed without changing its combinatorial type or symmetry group.
	\item $P$ is called \emph{perfect} if any essentially distinct but combinatorially equivalent polytope $Q\subset\RR^d$ has a smaller symmetry group than $P$, that is $\Aut(Q)\subset\Aut(P)$.
\end{myenumerate}
\end{definition}

\enquote{Essentially distinct} in $(ii)$ means that $P$ and $Q$ are not just reoriented or~rescaled versions of one another.

If a polytope is perfect, then it is rigid.
It seems to be open whether the converse holds in general.
In theory it could happen that a combinatorial type might have two \enquote{most symmetric} realizations as a polytope, and those cannot be continuously deformed into each other.



\begin{theorem}
An arc-transitive polytope $P\subset\RR^d$ is $\theta_2$-spectral.
%
\begin{proof}
The skeleton of $P$ is an arc-transitive realization of $G_P$ of full local dimension, hence has an eigenvalue $\theta\in\Spec(G)$ according to \cref{res:...}.
The tricky part is to show that $\theta=\theta_2$.

For this, we use the following fact:
Let $v$ be the skeleton of $P$ and define
%
$$P^\circ(\mathbf c) = P^\circ(c_1,...,c_n):=\{x\in\RR^d\mid \<x,v_i\>\le c_i\text{ for all $i\in V$}\}.$$
%
Finally, consider the matrix
%
$$M_{ij}:=-\frac{\partial^2\mathrm{vol}(P(\mathbf c))}{\partial c_i \partial c_j}\Big|_{\mathbf c=(1,...,1)}.$$
%
Since $P$ is edge-transitive, $M_{ij}$ contains the same value for all $ij\in E$.
Since $P$ is vertex-transitive, $M_{ii}$ does not depend in $i\in V$.
Finally, it is proven in \cite{...} that $M_{ij}=0$ whenever $ij\not\in E$, and that $M$ has a single negative eigenvalue which is simple.
Apparently, there are $\alpha,\beta\in\RR$ so that $M=\alpha A+\beta\Id$, where $A$ is the adjacency matrix of $M$.
\end{proof}
\end{theorem}


\begin{theorem}
If $P\subset\RR^d$ is an arc-transitive polytope, then
%
\begin{myenumerate}
	\item $P$ is rigid,
	\item $\Aut(P)$ is irreducible,
	\item any projection $\pi_U(P)$ onto a subspace $U\subseteq\RR^d$ is either not arc-transitive~or has a different edge-graph as $P$.
\end{myenumerate}
Furthermore, there is an eigenvalue $\theta\in\Spec(G_P)$ of the edge-graph $G_P$ \resp\ its~associated Laplacian eigenvalue $\lambda=\theta-\deg(G_P)$, so that the following holds:
\begin{myenumerate}
  \setcounter{enumi}{3}
	\item if $P$ has edge length $\ell$ and circumradius $r$, then
	%
	$$\frac\ell r=\sqrt{\frac{2\lambda}{\deg(G_P)}}.$$
	\item if the polar polytope $P^\circ$ has dihedral angle $\alpha$, then
	%
	$$\cos\alpha=-\frac{\theta}{\deg(G_P)}.$$
\end{myenumerate}
\end{theorem}

\begin{conjecture}\label{conj:arc_transitve}
Each arc-transitive polytope $P\subset\RR^d$ is $\theta_2$-spectral, and satisfies
%
\begin{myenumerate}
	\item $P$ is perfect,
	\item $P$ realizes all the symmetries of its edge-graph,
	\item $P$ is the only arc-transitive polytope (up to reorientation and rescaling) with edge-graph $G_P$.
\end{myenumerate}
\end{conjecture}

Probably in, in all these result, the eigenvalue $\theta$ \resp\ $\lambda$ can be replaced with $\theta_2$ \resp\ $\lambda_2$, but we were not able to prove that.
However, it holds in any single case of arc-transitive polytope that we have checked.

\begin{example}
There are many ways to compute the circumradius of an $n$-simplex with unit edge-length, and here is another one:

The complete graph $K_n$ is arc-transitive and has spectrum $\{(-1)^{n-1},n^1\}$. The second largest eigenvalue $\theta_2=-1$ gives rise to an $(n-1)$-dimensional polytope with edge-graph $K_n$, that is, the $(n-1)$-dimensional simplex.
Assuming edge length $\ell=1$, we can compute its circumradius:
%
$$r=\sqrt{\frac{\deg(G)}{\lambda_2}} = \sqrt{\frac{\deg(G)}{\deg(G)-\theta_2}} = \sqrt{\frac{n-1}{n-1-(-1)}} = \sqrt{1-\frac1n}.$$

\end{example}

\begin{example}
Compute the dihedral angle of the rhombic dodecahedron and the rhombic triacontahedron.
\end{example}

But this technique can also be used the other way around, namely, concluding from the knowledge of the metric properties of a polytope and the eigenvalues of its edge-graph to the fact that it is spectral.

\begin{example}
We show that all regular polytopes are in fact $\theta_2$-spectral, as was already conjectured by Licata and Powers \cite{licata1986surprising}.

The essential facts we are using are some tabulated metric and spectral properties of these polytopes, \eg\ found in \cite{buekenhout1998number}.

\begin{itemize}
\item
Remarkable, the 24-cell has edge-length $\ell$ identical to circumradius $r$.
This determines the Laplacian eigenvalue of its skeleton:
%
$$1=\frac\ell r=\sqrt{\frac{2\lambda}{\deg(G)}} \quad\implies\quad \lambda=\frac12\deg(G) = 4.$$
%
One checks  that $4$ is exactly the second largest Laplacian eigenvalue of its edge-graph, and that this eigenvalue  has multiplicity four.

\item
600-cell: $3(1+\sqrt{5})$

\item
120-cell: $2\phi-1$
\end{itemize}

\begin{center}
\begin{tabular}{c|rrrr}
polytope & $\ell$ & $r$ & $\lambda_2$ & $\deg(G_P)$ \\
\hline
$\overset{\phantom.}24$-cell & $1$ & $1$ & $4$ & $8$ \\
$120$-cell & $3-\sqrt 5$ & $2\sqrt 2$ & $2\phi-1$ &  $4$ \\
$600$-cell & $2/\phi$ & $2$ & $3(1+\sqrt 5)$ & $12$
\end{tabular}
\end{center}



\end{example}


\begin{theorem}
If a polytope has a connected, full-dimensional and spanning edge-orbit, then it is perfect.
\end{theorem}







\newpage

\section{Edge- and vertex-transitive polytopes}

The goal of this section is to show that every polytope $P\subset\RR^d$ that is simultane\-ously vertex- and edge-transitive is an eigenpolytope to the second smallest eigenvalue of its edge-graph.
Note that being only edge-transitive is just slightly weaker than being vertex- and edge-transitive, as it was shown in \cite{winter2020polytopes} that edge-transitivity of convex polytopes in dimension $d\ge 4$ implies vertex-transitivity anyway.


\begin{theorem}\label{res:vertex_edge_transitive_is_theta2_realization}
If $P\subset\RR^d$ is vertex-transitive and edge-transitive, then it is the~$\theta_2$-eigenpolytopes of its edge-graph.
%
\begin{proof}
Let $X\in\RR^{n\x n}$ be the matrix defined in \cref{res:izmestiev}.
Since $P$ is transitive on vertices, there is a number $\alpha\in\RR$ with $X_{ii}=\alpha$ for all $i\in V$.
Since $P$ is edge-transitive, there is a number $\beta<0$ so that $X_{ij}=\beta$ for all $ij\in E(G_P)$.
Since we also have $X_{ij}=0$ for all $ij\not\in E(G_P)$, we find that $X$ must be of the form
%
$$X= \alpha \Id - \beta A \quad\implies\quad A=\alpha\Id-\frac1\beta X,$$
%
where $A$ is the adjacency matrix of $G_P$.

$X$ has a single negative eigenvalue, which is simple, and $\dim\ker X=d$.
In other words, its second smallest eigenvalue is zero and has multiplicity $d$.
Consequently, $A$ has second \emph{largest} eigenvalue $\theta_2=\alpha$ of multiplicity $d$ to the same eigenvectors as $X$.

Let $v$ be the skeleton of $P$ with arranegment matrix $M$ and arrangement space $U$.
Since $XM=0$ and $\rank M=d$, we find that the $U=\Span M$ must be the $0$-eigenspace of $X$, hence the $\theta_2$-eigenspace of $A$.
Thus, $v$ is the $\theta_2$-realization of $G_P$ and $P$ is spectral.
\end{proof}
\end{theorem}

The argument of \cref{res:vertex_edge_transitive_is_theta2_realization} cannot be easily generalized to any weaker form of symmetry.
For example, one would like to proof that every spectral polytope has eigenvalue $\theta_2$, or more generally, every balanced polytope has eigenvalue $\theta_2$.

\begin{corollary}
If $P\subset\RR^d$ is vertex- and edge-transitive, then holds:
%
\begin{myenumerate}
	\item $\Aut(P)$ is irreducible,
	\item $P$ is the unique simultaneously vertex- and edge-transitive polytope for which the edge-graph is isomorphic to $G_P$,
	\item $P$ realizes all symmetries of its edge-graph,
	\item $P$ is a perfect (rigid) polytope,
	\item $P$ is the unique most symmetric realization of its combinatorial type,
	\item if $P$ has edge-length $\ell$ and circumradius $r$, then
	%
	$$\Big[\frac \ell r \Big]^2 = \frac{2\lambda_2(G_P)}{\deg(G_P)} = 2\Big(1-\frac{\theta_2(G_P)}{\deg(G_P)}\Big).$$
	%
	\item if the polar dual $P^\circ$ has dihedral angle $\alpha$, then
	%
	$$\cos(\alpha)=-\frac{\theta_2(G_P)}{\deg(G_P)}.$$
\end{myenumerate}
\end{corollary}





\section{Distance-transitive polytopes}

\subsection{Distance-transitive polytopes}
\label{sec:distance_transitive_polytopes}

In general, there is no apparent reason for why a spectral polytope must be $\theta_2$-spectral.
In the case of distance-transitive polytopes there can be found an easy argument involving the cosine sequence of its skeleton.
The argument is based on the number of sign changes in $u_\delta$ and the so called \emph{two-piece property} for embedded graphs.

\begin{definition}
A realization $v$ is said to have the \emph{two-piece property} (or TPP),~if every hyperplane cuts it into at most two pieces.
More formally, given any vector $x\in \RR^d$ and scalar $c\in\RR$, the induced subgraphs
%
$$
G_+:=G[\,i\in V\mid \<x,v_i\>\ge c\,]
\quad\text{and}\quad
G_-:=G[\,i\in V\mid \<x,v_i\>\le c\,]
$$
%
must be connected (if non-empty).
\end{definition}

The image below shows two symmetric realizations of the cycle graph $C_5$, one~of which has the TPP (left), and one of which has not (right).

%\begin{center}
%\includegraphics[width=0.5\textwidth]{img/5_gon_cut}
%\end{center}

We are going to use the following fact:

\begin{theorem}[\cite{...}, Theorem xx]
The skeleton of a polytope has the TPP.
%
\begin{proof}[Sketch of proof.]
Let $v$ be the skeleton of a polytope, $x\in\RR^d$ and $c\in \RR$.

Let $i_+\in V$ be the vertex which maximizes the functional $\<v_\cdot,x\>$.
By the simplex algorithm, every vertex on the \enquote{positive} side of the hyperplane $\<\cdot,x\>=c$ can reach $v_{i_+}$ by a path in the edge-graph that is non-decreasing in $\<v_\cdot,x\>$.
Hence the positive side is connected if non-empty.
Equivalently for the negative side.

\end{proof}
\end{theorem}

\begin{theorem}
A distance-transitive polytope $P$ is $\theta_2$-spectral.
%
\begin{proof}
Let $v$ be the full-dimensional and distance-transitive realization of $P$.
Since it is also arc-transitive, it has an eigenvalue (by \cref{cref:...}).
By \cref{res:...} it must then be the $\theta_k$-realization of $G_P$.

Now consider cutting $v$ by the hyperplane $v_i^\bot$ for some $i\in V$.
The number of components left after the cut is exactly one more than the number of sign changes of the cosine sequence $u_\delta$.
From \cref{res:...} we know that there are exactly $k-1$ sign changes for the $\theta_k$-realization, hence $k$ pieces after the cut.

Since $v$ is the skeleton of a polytope, we have the TPP, and $k\le 2$ pieces.
Since $v$ cannot be the trivial $\theta_1$-realization of $G_P$, it must be the $\theta_2$-realization, and $P$ the $\theta_2$-eigenpolytope.
\end{proof}
\end{theorem}

\begin{corollary}
Let $P$ be a distance-transitive polytope.
%
\begin{myenumerate}
	\item Among distance-transitive polytopes, $P$ is uniquely determined by its edge-graph.
	\item $P$ realizes all the symmetries of its edge-graph.
	\item $P$ is the unique most symmetric realization of its combinatorial type.
\end{myenumerate}
\end{corollary}

Godsil's classification of the $\theta_2$-spectral distance-regular graphs (see \cref{res:spectral_distance_regular_graphs}; all of which~turned out to be distance-transitive) allows a complete classification of distance-tran\-sitive polytopes.

\begin{theorem}\label{res:distance_transitive_classification}
If $P\subset\RR^d$ is a distance-transitive polytope, then it is one of the following:
%
\begin{enumerate}[label=$(\text{\roman*}\,)$]
	\item a regular polygon $(d=2)$,
	\item the regular dodecahedron $(d=3)$,
	\item the regular icosahedron $(d=3)$,
	\item a cross-polytopes, that is, $\conv\{\pm e_1,...,\pm e_d\}$ where $\{e_1,...,e_d\}\subset\RR^d$ is the standard basis of $\RR^d$,
	\item a hyper-simplex $\Delta(d,n)$, that is, the convex hull of all vectors $v\in\{0,1\}^{d+1}$ with exactly $k$ 1-s,
	\item a cartesian power of a regular simplex (this includes hypercubes),
	\item a demi-cube, that is, the convex hull of all vectors $v\in\{-1,1\}^d$ with~an~even number of 1-s,
	\item the $2_{21}$-polytope, also called Gosset-polytope $(d=6)$,
	\item the $3_{21}$-polytope, also called Schläfli-polytope $(d=7)$.
\end{enumerate}
%
The order of this list agrees with the list of graphs in \cref{res:spectral_distance_regular_graphs}.
\end{theorem}

Note that the list in \cref{res:distance_transitive_classification} contains many polytopes that are not regular, and contains all regular polytopes except for the 24-cell, 120-cell and 600-cell.
The distance-transitive polytopes thus form a distinct class of remarkably symmetric polytopes which is not immediately related to the class of regular polytopes.

Noteworthy however, is that all the distance-transitive polytopes are \emph{Wythoffian poly\-topes}, that is, they are orbit polytopes of finite reflection groups.
\Cref{fig:distance_transitive_Coxeter} shows the Coxeter-Dynkin diagrams of these polytopes.

\begin{figure}
\centering
\includegraphics[width=0.9\textwidth]{img/distance_transitive_Coxeter}
\caption{Coxeter-Dynkin diagrams of distance-transitive polytopes.}
\label{fig:distance_transitive_Coxeter}
\end{figure}


==> v.2 - arXiv/sec/future.tex <==

\tempnewpage
\section{Conclusion and open questions}
\label{sec:future}

In this paper we have studied \emph{eigenpolytopes} and \emph{spectral polytopes}.
The former are polytopes constructed from a graph and one of its eigenvalues.
A polytope is spectral if it is the eigenpolytopes of its edge-graph.
These are of interest because spectral graph theory then ensures a strong interplay between the combinatorial properties of the edge-graph and the geometric properties of the polytope.

The study of eigenpolytopes and spectral polytopes has left us with many open questions.
Most notably, how to detect spectral polytopes purely from their geome\-try.
We introduced a tool (\cref{res:implies_spectral}), which was sufficient to proof that (most) edge-transitive polytopes are spectral.
We do not know how much more general it can be applied.

\begin{question}
\label{q:characterization}
Does \cref{res:implies_spectral} already characterize $\theta_2$-spectral polytopes (or even spectral polytopes in general)?
\end{question}

If the answer is affirmative, this would provide a geometric characterization of polytopes that are otherwise defined purely in terms of spectral graph theory.
The result of Izmestiev suggests that polytopes with sufficiently regular geometry are $\theta_2$-spectral: the entry of the matrix $X$ in \cref{res:izmestiev} at index $ij\in E$ can be~expressed as
%
$$X_{ij}=\frac{\vol(\sigma_i\cap\sigma_j)}{\|v_i\|\|v_j\|\sin\angle(v_i,v_j)},$$
%
where $\sigma_i$ and $\sigma_j$ are the facets of the polar dual $P^\circ$ that correspond to the vertices $v_i,v_j\in\F_0(P)$.
Because of this formula, it might be actually easier to classify the polar duals of $\theta_2$-spectral polytopes.

An affirmative answer to \cref{q:characterization} would also mean a negative answer to the following:

\begin{question}
\label{q:not_theta_2}
Is there a $\theta_k$-spectral polytope/graph for some $k\not=2$?
\end{question}

The answer is known to be negative for edge-transitive polytopes/graphs (see \cref{res:edge_transitive_spectral_graph}), but unknown in general.

The second-largest eigenvalue $\theta_2$ is special for other reasons too.
Even if a graph is not $\theta_2$-spectral, it seems to still imprint its adjacency information onto the edge-graph of its $\theta_2$-eigenpolytope.

\begin{question}
\label{q:realizing_edges}
Given an edge $ij\in E$ of $G$, if $v_i$ and $v_j$ (as defined in \cref{def:eigenpolytope}) are distinct vertices of the $\theta_2$-eigenpolytope $P_G(\theta_2)$, is then also $\conv\{v_i,v_j\}$ an edge of $P_G(\theta_2)$?
\end{question}

This was proven for distance-regular graphs in \cite{godsil1998eigenpolytopes}, and is not necessarily true for eigenvalues other than $\theta_2$.

All known spectral polytopes are exceptionally symmetric.
It is unclear whether this is true in general.

\begin{question}
\label{q:trivial_symmetry}
Are there spectral polytopes with trivial symmetry group?
\end{question}

An example for \cref{q:trivial_symmetry} must be asymmetric, yet with a reasonably large eigenspaces.
Such graphs exist among the distance-regular graphs, but all spectral distance-regular graphs were determined in \cite{godsil1998eigenpolytopes} (see also \cref{res:spectral_distance_regular_graphs}) and turned out to be distance-transitive, \ie\ highly symmetric.

A clear connection between being spectral and being symmetric is missing.
To emphasize our ignorance, we ask the following:

\begin{question}
\label{q:spectral_non_vertex_transitive}
Can we find more spectral polytopes that are \emph{not vertex-transitive}?
What characterizes them?
\end{question}

The single known spectral polytope that is \emph{not} vertex-transitive is the \emph{rhombic dodecahedron} (see \cref{fig:edge_transitive}).
The fact that it is spectral appears purely accidental, as there seems to be no reason for it to be spectral, except that we can explicitly check that it is. For comparison, the highly related \emph{rhombic triacontahedron} is not spectral.

On the other hand, vertex-transitive spectral polytopes might be quite common.

\begin{question}
\label{q:specific_instance}
Let $P\subset\RR^d$ be a polytope with the following properties:
%
\begin{myenumerate}
	\item $P$ is vertex-transitive,
	\item $P$ realizes all the symmetries of its edge-graph, and
	\item $\Aut(P)$ is irreducible.
\end{myenumerate}
%
Is $P$ (combinatorially equivalent to) a spectral polytope? %Or at least an eigenpolytope?
\end{question}

No condition in \cref{q:specific_instance} can be dropped.
If we drop vertex-transitivity,~we could take some polytope whose edge-graph has trivial symmetry and only small eigenspaces. Dropping $(ii)$ leaves vertex-transitive neighborly polytopes, for which we know that these are mostly not spectral (except for the simplex).
Dropping $(iii)$ leaves us with the prisms and anti-prisms, the eigenspaces of their edge-graphs are rarely of dimension greater than two.

%\cref{q:specific_instance} has equally interesting consequences if it is only true for the eigenpolytope case.
%For example, several polytopes with relevance in integer optimization seem to be eigenpolytopes, \eg\ the Birkhoff polytope or the traveling salesman polytopes.
%This would allow a formulation of the respective optimization problem in the language of spectral graph theory.
%Also, this gives a way to study the symmetry groups of these polytopes (which are oftem much larger than expected from their definition).


Finally, we wonder whether these spectral techniques can be any help in classifying the edge-transitive polytopes.

\begin{question}
Can we classify the edge-transitive graphs that are spectral, and~by this, the edge-transitive polytopes?
\end{question}

\begin{question}
Can the existence of half-transitive polytopes be excluded by using spectral graph theory (see \cref{sec:arc_transitive})?
\end{question}







\iffalse


\hrulefill




We have seen that in some situations computing the eigenpolytope of the edge-graph of a polytope results in the same polytope again.
Polytopes/graphs for which this happens are called \emph{spectral}.
We have introduced a tool for proving that certain geometrically well-behaved polytopes are necessarily $\theta_2$-spectral.

It is open whether spectral polytopes exist to other eigenvalues than $\theta_2$:

\begin{question}
\label{q:not_theta_2}
Is there a $\theta_k$-spectral polytope/graph for some $k\not=2$?
\end{question}

We have seen that the answer is negative for the distance-transitive (actually distance-regular) graphs (see \cref{res:distance_regular_theta_k}).
Our hope is that the proof can~be~extended to a larger class of graphs as \eg\ 1-walk-regular or arc-transitive graphs.

Even if a graph is not $\theta_2$-spectral, it seems to still imprint its adjacency information on the edge-graph of its $\theta_2$-eigenpolytope: 

\begin{question}
\label{q:realizing_edges}
Let $G$ be a graph with $\theta_2$-eigenpolytope $P=P_G(\theta_2)$.
For each~$i\in$ $V$ let $v_i\in\RR^d$ be as defined in \cref{def:eigenpolytope}.
Now, if $ij\in E$ and $v_i\not= v_j$ are distinct vertices of $P$, is then also $\conv\{v_i,v_j\}$ an edge of $P$?
\end{question}

The answer is affirmative for distance-regular graphs as shown by Godsil in \cite{godsil1998eigenpolytopes}.


%\begin{question}
%Is there a combinatorial type of polytopes that has two realizations of maximal degree of symmetry while being incomparable as groups?
%\end{question}

%\begin{question}
%Is a rigid polytope always perfect?
%\end{question}

%\begin{question}
%If $\Sigma\subseteq\Aut(G)$ is arc-transitive, and for every $i\in V$ the stabilizer~of $\{i\}\cup N(i)$ in $\Sigma$ is trivial, is then every \msays{faithful} irreducible $\Sigma$-realization automatically of full local dimension?
%\msays{Yes, the dodecahedron}
%\end{question}

All known spectral polytopes are highly symmetric.
We therefore ask the following:

\begin{question}
\label{q:trivial_symmetry}
Are there spectral polytopes with trivial symmetry group?
%Can we even find more spectral polytopes (besides the rhombic dodecahedron) that are \emph{not vertex-transitive}?
\end{question}

To construct an example, one has to find a graph with no non-trivial symmetries, but whose eigenspaces are still reasonably large.
Such graphs can be found among the distance-regular graphs.
However, all spectral graphs among these were already determined by Godsil and all of them turned out to be distance-transitive.

A clear connection between being spectral and being symmetric is missing.
To emphasize our ignorance, we have the following:

\begin{question}
Can we find more spectral polytopes that are \emph{not vertex-transitive}?
What characterizes them?
%What characterizes the spectral polytopes that are not vertex-transitive?
\end{question}

Only one such polytope is known: the \emph{rhombic dodecahedron}.
We know that it spectral by explicit computation, but a systematic proof of this fact (that admits a generalization) is missing.
%For this polytope, no systematic reason is known for why it is spectral, except that we can check that it is by computation.

In general, how else can one characterize spectral polytopes?
The result of~Izmes\-tiev suggests that polytopes with sufficiently regular geometry are $\theta_2$-spectral.
In fact, the value of the matrix $X$ in \cref{res:izmestiev} at an index $ij\in E$ can be given~explicitly
%
$$X_{ij}=\frac{\vol(\sigma_i\cap\sigma_j)}{\|v_i\|\|v_j\|\sin\angle(v_i,v_j)},$$
%
where $\sigma_i$ and $\sigma_j$ are the facets of the polar dual $P^\circ$ that correspond to the vertices $v_i,v_j\in\F_0(P)$.
Because of this, it might be actually easier to classify the polar duals of $\theta_2$-spectral polytopes.

\begin{question}
\label{q:characterization}
Does \cref{res:implies_spectral} already characterize $\theta_2$-spectral polytopes (or even spectral polytopes in general)?
\end{question}

There are very specific classes of polytopes that might have spectral of their combiantorial type:

\begin{question}
\label{q:specific_instance}
Let $P\subset\RR^d$ be a polytope with the following properties:
%
\begin{myenumerate}
	\item $P$ is vertex-transitive,
	\item $P$ realizes all the symmetries of its edge-graph, and
	\item $\Aut(P)$ is irreducible.
\end{myenumerate}
%
Is $P$ (combinatorially equivalent to) a spectral polytope? Or at least an eigenpolytope?
\end{question}

We know that $P$ in \cref{q:specific_instance} is not necessarily spectral if we drop any of the conditions.
If we drop vertex-transitivity we could take some polytope with trivial symmetry. Dropping $(ii)$ gives the neighborly polytopes, for which we know that these are only balanced, but mostly not spectral (except for the simplex).
Dropping $(iii)$ gives us the prisms and anti-prisms which mostly do not have eigenspaces of dimension three or higher.

\cref{q:specific_instance} has equally interesting consequences if it is only true for the eigenpolytope case.
For example, several polytopes with relevance in integer optimization seem to be eigenpolytopes, \eg\ the Birkhoff polytope or the traveling salesman polytopes.
This would allow a formulation of the respective optimization problem in the language of spectral graph theory.
Also, this gives a way to study the symmetry groups of these polytopes (which are oftem much larger than expected from their definition).

Finally, we wonder whether these spectral techniques can be any help in classifying edge-transitive polytopes.

\begin{question}
Can we classify the edge-transitive polytopes, or equivalently, the simultaneously vertex- and edge-transitive graphs that are spectral?
\end{question}

\begin{question}
Can spectral graph theory help to show that no half-transitive polyopes exist?
\end{question}

\fi



==> v.2 - arXiv/sec/introduction.tex <==

\section{Introduction}
\label{sec:introduction}

\emph{Eigenpolytopes} are a construction in the intersection of combinatorics and geometry, using techniques from spectral graph theory.
Eigenpolytopes provide a way~to associate several polytopes to a finite simple graph, one for each eigenvalues of~its adjacency matrix.
A formal definition can be found in \cref{sec:def_eigenpolytope}.

\vspace{0.5em}
\begin{center}
\includegraphics[width=0.7\textwidth]{img/cube_intro_pic}
\end{center}
\vspace{0.5em}

Eigenpolytopes can be applied from two directions:
for the first, one starts~from a given graph, computes its eigenpolytopes, and tries to deduce, from the geometry and combinatorics of these polytopes, something about the original~graph.
For the other direction, one starts with a polytope, asks whether it is an eigenpolytope, and if so, for which graphs, which eigenvalues, and how these relate to the original polytope.
Eigenpolytopes have several interesting geometric and algebraic properties, and establishing that a family of polytopes consists of eigenpolytopes opens up their study to the techniques of spectral graph theory.

For some graphs the connection to their eigenpolytopes is especially strong: it can happen  that a graph is the edge-graph of one of its eigenpolytopes, or equivalently, that a polytope is an eigenpolytope of its edge-graph.
Such graphs/polytopes are quite special and we shall call them \emph{spectral}.
For example, all regular polytopes are spectral, but there are many others.
Their properties are not well-understood.

We survey the literature of eigenpolytope and spectral polytopes.
We establish a technique with which to prove that certain polytopes are spectral polytopes and we apply it to \emph{edge-transitive} polytopes. That are polytopes for which the Euclidean symmetry group $\Aut(P)\subset\Ortho(\RR^d)$ acts transitively on the set of edge $\F_1(P)$.
As we shall explain, this characterization suffices to proves that an edge-transitive polytope is uniquely determined by its edge-graph, and also realizes all its combinatorial symmetries.
A complete classification of edge-transitive polytopes is not known as of yet.
However, using results on eigenpolytopes, we are able to give a complete classification of a sub-class of the edge-transitive polytopes, namely, the \emph{distance-transitive polytopes}.

%Besides this results, we aim to give an extensive literature overview of eigenpolytopes, including the first perspective \enquote{from the graph to the polytope}.
%A phenomenon that seems to haev attracted peoples attention repeatedly, is when a polytope is the eigenpolytope of its edge-graph.
%We shall call these polytopes \emph{spectral}.
%...
%
%The prerequisite for this paper is a mild dose of spectral graph theory.
%It might be helpful to already have heard about spectral realizations, but we also get away without mentioning this concept explicitly.
%In case of doubt, consider \cite{winter2020symmetric}, where we previously discussed spectral realizations of highly symmetric graphs.
%The proofs of some statements will be just cited from this paper.


\subsection{Outline of the paper}

\cref{sec:eigenpolytopes} starts with a motivating example for directing the reader towards the definition of the \emph{eigenpolytope} as well as the phenomenon of \emph{spectral} graphs and polytopes.
We include a literature overview for~\mbox{eigenpolytopes} and spectral polytopes.

In \cref{sec:balanced_spectral} we give a first rigorous definition for the notion \enquote{spectral polytope} via \emph{balanced polytopes}. The latter is a notion related to the rigidity theory.
%This highlights the rigidity theory perspective of that idea.

In \cref{sec:izmestiev} we introduce the, as of yet, most powerful tool for proving that~certain polytopes are spectral.

In the final section, \cref{sec:edge_transitive}, we apply this result to \emph{edge-transitive} polytopes.
It is a simple corollary of the previous section that these are $\theta_2$-spectral.
We explore the implications of this finding: edge-transitive polytopes (in dimension $d\ge 4$) are uniquely determined by the edge-graph and realize all of its symmetries.~%
We~discuss sub-classes, such as the arc-, half- and distance-transitive polytopes.
We close with a complete classification of the latter (based on a result of Godsil).





%The idea itself has spawned several times and appears too immediate to not yield any interesting results.
%
%In easy terms, one starts with a finite, simple graph $G$ and chooses an eigenvalue $\theta\in\Spec(G)$ (\ie\ of its adjacency or Laplace matrix).
%From this, one constructs a polytope $P_G(\theta)$, the so-called \emph{$\theta$-eigenpolytope}.
%If the eigenvalue had multiplicity $d$, then the polytope has dimension $d$.
%One hence expects the most interesting results for graphs with large eigenspaces.
%
%The hope then is that the geometry and combinatorics of $P_G(\theta)$ tells us something deep about $G$.
%Results of this form are not too abundant.
%Still, people have asked other questions about eigenpolytope, and the answeres turn out to be interesting.



\tempnewpage

\section{Eigenpolytopes and spectral polytopes}
\label{sec:eigenpolytopes}

\subsection{A motivating example}
\label{sec:example}

Let $G=(V,E)$ be the edge-graph of the cube, with vertex set $V=\{1,...,8\}$,~num\-bers assigned to the vertices as in the figure below.
%
\begin{figure}[h!]
\centering
\includegraphics[width=0.48\textwidth]{img/cube}
\end{figure}

\noindent
The spectrum of that graph (\ie\ of its adjacency matrix) is $\{(-3)^1,(-1)^3,1^3,3^1\}$.
Most often, one denotes the largest eigenvalue by $\theta_1$, the second-largest by $\theta_2$, and so on.
In spectral graph theory, there exists the general rule of thumb that the most exciting eigenvalue of a graph is not its largest, but its \emph{second-largest} eigenvalue $\theta_2$ (which is related to the \emph{algebraic connectivity} of $G$).

For the edge-graph of the cube, we have $\theta_2=1$,~of multiplicity \emph{three}.
And here are three linearly independent eigenvectors to $\theta_2$:
%
%\begin{align*}
%u_1^\top &= (+ 1,+ 1,+ 1,+ 1,-1,-1,-1,-1), \\
%u_2^\top &= (+ 1,+ 1,- 1,- 1,+1,+1,-1,-1), \\
%u_3^\top &= (+ 1,- 1,+ 1,- 1,+1,-1,+1,-1), \\
%\end{align*}
%

\vspace{0.5em}

\begin{center}
\raisebox{-3.3em}{\includegraphics[width=0.23\textwidth]{img/cube_eigenvector}}
\qquad
$
u_1 = \begin{pmatrix}
\phantom+1\\ \phantom+1 \\ \phantom+1 \\ \phantom+1 \\ -1 \\ -1 \\ -1 \\ -1
\end{pmatrix},\quad
u_2 = \begin{pmatrix}
\phantom+1\\ \phantom+1 \\ -1 \\ -1 \\ \phantom+1 \\ \phantom+1 \\ -1 \\ -1
\end{pmatrix},\quad
u_3 = \begin{pmatrix}
\phantom+1\\ -1 \\ \phantom+1 \\ -1 \\ \phantom+1 \\ -1 \\ \phantom+1 \\ -1
\end{pmatrix}.
$
\end{center}

\vspace{0.7em}
\noindent
We can write these more compactly in a single matrix $\Phi\in\RR^{8\x 3}$:

\vspace{0.4em}
\begin{center}
$\Phi= \;\begin{blockarray}{(lll)r}%\begin{block}{(ccc)c}
\phantom+1 & \phantom+1 & \phantom+1\;\; &\text{\quad \footnotesize $\leftarrow v_1$}\\
\phantom+1 & \phantom+1 & -1 & \text{\quad \footnotesize $\leftarrow v_2$} \\
\phantom+1 & -1 & \phantom+1 & \text{\quad \footnotesize $\leftarrow v_3$} \\
\phantom+1 & -1 & -1 & \text{\quad \footnotesize $\leftarrow v_4$} \\
-1 & \phantom+1 & \phantom+1 & \text{\quad \footnotesize $\leftarrow v_5$} \\
-1 & \phantom+1 & -1 & \text{\quad \footnotesize $\leftarrow v_6$} \\
-1 & -1 & \phantom+1 & \text{\quad \footnotesize $\leftarrow v_7$} \\
-1 & -1 & -1 & \text{\quad \footnotesize $\leftarrow v_8$} \\
%\end{block}
\end{blockarray}.$
%
\qquad
\raisebox{-4.2em}{\includegraphics[width=0.4\textwidth]{img/cube_coordinates}}
\end{center}

We now take a look at the rows of that matrix, of which it has exactly eight.~These rows are naturally assigned to the vertices of $G$ (assign $i\in V$ to the $i$-th row of~$\Phi$), and each row can be interpreted as~a~vec\-tor in $\RR^3$.

If we place each vertex $i\in V$ at the position $v_i\in\RR^3$ given by the $i$-th row of $\Phi$, we find that this embedds the graph $G$ \emph{exactly} as the skeleton of a cube (see the figure above).
In other words: if we compute the convex hull of the $v_i$, we get back the polyhedron from which we have started.
What a coincidence, isn't it?

This example was specifically chosen for its nice numbers, but in~fact,~the same works out as well for many other polytopes, inclu\-ding all the regular polytopes~in all dimension.
One probably learns to appreciate this magic when suddenly in~need for the vertex coordinates of some not so nice polytope, say, the regular dodecahedron or 120-cell.
With this technique in the toolbox, these coordinates are just one eigenvector-computation away (we included a short Mathematica script in \cref{sec:appendix_mathematica}).
Note also, that we never specified~the~dim\-en\-sion of~the~embed\-ding, but it just so happened, that the second-largest eigenvalue has the right multiplicity.
This phenomenon definitely deserves an explanation.

%Now, a short reality check: could this have been a coincidence?
%In fact, \emph{no}.
%The same works perfectly well for all the other regular polytopes (always making use of the second-largest eigenvalue).

\subsubsection*{On the choice of eigenvectors}
\label{sec:choice_of_eigenvectors}

One might object that the chosen eigenvectors $u_1, u_2$ and $u_3$ look suspiciously cherry-picked, and we may not get such a nice result if we would have chosen just any eigenvectors.
And this is true.
For an appropriate choice of these vectors, we can, instead of a cube, get a cuboid, or a parallelepiped.
In fact, we can obtain any \emph{linear} transformations of the cube.
\emph{But}, we can also get \emph{only} linear transformations, and nothing else.
The reason is the following well~know  fact from linear algebra:

\begin{theorem}
\label{res:same_column_span}
Two matrices $\Phi,\Psi\in\RR^{n\x d}$ have the same column span, \ie~$\Span \Phi=\Span \Psi$, if and only if their rows are related by an invertible linear transformation, \ie\ $\Phi=\Psi T$ for some $T\in\GL(\RR^d)$.
\end{theorem}

\noindent
%Since the rows of our matrices are the coordinates of the $v_i$, this explains our the comment concerning linear transformations.
In our case, the column span is the $\theta_2$-eigenspace, and the rows are the coordinates of the $v_i$.
We say that any two polytopes constructed in this way are \emph{linearly equivalent}.

The only notable property of the chosen basis in the example is, that the vectors $u_1, u_2$ and $u_3$ are orthogonal and of the same length.
Any other choice of such a basis of~the~\mbox{$\theta_2$-eigen}\-space (\eg\ an orthonormal basis) would also have given a cube, but reoriented, rescaled and probably with less nice coordinates.
For details on how this choice relates to the orientation, see \eg\ \cite[Theorem 3.2]{winter2019geometry}.


\subsection{Eigenpolytopes}
\label{sec:def_eigenpolytope}

We compile our example into a definition.

\begin{definition}\label{def:eigenpolytope}
Start with a graph $G=(V,E)$, an eigenvalue $\theta\in\Spec(G)$ thereof, as well as an orthonormal basis $\{u_1,...,u_d\}\subset\RR^n$  of the $\theta$-eigenspace. 
We define the \emph{eigenpolytope matrix} $\Phi\in\RR^{n\x d}$ as the matrix in which the $u_i$ are the columns:\phantom{mm}
%
\begin{equation}
\label{eq:eigenpolytope_matrix}
\Phi :=\begin{pmatrix}
		\mid & & \mid \\
		u_1 & \!\!\cdots\!\!\! & u_d \\
		\mid & & \mid		
	\end{pmatrix}=
\begin{pmatrix}
	\;\horzbar\!\!\!\! & v_1\T & \!\!\!\!\horzbar\;\; \\
	& \vdots & \\[0.4ex]
	\;\horzbar\!\!\!\! & v_n\T & \!\!\!\!\horzbar\;\;
\end{pmatrix}.
\end{equation}
%
Let $v_i\in\RR^d$ denote the $i$-th row of $\Phi$.
The polytope
%
$$P_G(\theta):=\conv\{v_i\mid i\in V\}\subset\RR^d$$
%
is called \emph{$\theta$-eigenpolytope} (or just \emph{eigenpolytope}) of $G$.
\end{definition}

For later use we define the \emph{eigenpolytope map} 
%
\begin{equation}
\label{eq:eigenpolytope_map}
\phi:V\ni i\mapsto v_i\in\RR^d
\end{equation}
%
that to each vertex $i\in V$ assignes the $i$-th row of the eigenpolytope matrix.

Note that the basis $\{u_1,...,u_d\}\subset\Eig_G(\theta)$ in \cref{def:eigenpolytope} is explicitly chosen~to be an \emph{orthonormal basis}.
This is not strictly necessarily, but this choice is convenient from a geometric point of view: 
a different choice for this basis gives the same~poly\-tope, but with a different orientation rather than, say, transformed~by~a~general linear transformation.
This preserves metric properties and is closer to how polytopes are usually consider up to rigid motions.
We can also reasonably speak of \emph{the} $\theta$-eigenpolytope, as any two differ only by orientation.
%Symmetries of polytopes are often considered as rigid motions.

%Note again that the choice of the basis $u_1,...,u_d\in\RR^d$ only controls the orientation of the eigenpolytope, but has no influence on its combinatorial type, etc.

%More generally, to any polytope $P\subset\RR^d$ with vertices labeled $v_1,...,v_n\in \F_0(P)$, we can associate a matrix $M$, in which the $v_i$ are the rows.
%We shall call this matrix the \emph{arrangement matrix} of $P$.
%Because \cref{def:eigenpolytope} chooses an \emph{orthonormal} basis of eigenvectors, we have the special case $M\T M=\Id$.

With this terminology in place, our observation in the example of \cref{sec:example}~can be summarized as \enquote{the cube is the $\theta_2$-eigenpolytope of its edge-graph}, or alternatively as \enquote{the cube-graph is the edge-graph of its $\theta_2$-eigenpolytope}.
%
Here is~a~depic\-tion of all the eigenpolytopes of the cube-graph, one for each eigenvalue:

\vspace{0.5em}
\begin{center}
\includegraphics[width=0.7\textwidth]{img/cube_eigenpolytopes}
\end{center}

\noindent
We observe that the phenomenon from \cref{sec:example} only happens for $\theta_2$.
In general, the $\theta_1$-eigenpolytope of a regular graph will always be a single point (which is, why we rarely care about the largest eigenvalue).
Also, whenever a graph is bipartite, the eigenpolytope to the smallest eigenvalue is 1-dimensional, hence a line segment.

We are now free to compute the eigenpolytopes of all kinds of graphs, \mbox{including} graphs which are not the edge-graph of any polytope (so-called \emph{non-polytopal} graphs).
It is then little surprising that no edge-graph of any of its eigenpolytope gives the original graph again.

But even if we start from a polytopal graph, one is not guaranteed to find an eigen\-polytope that has the initial graph as its edge-graph (\eg\ the edge-graph of the triangular prism has no eigenvalue of multiplicity three, hence no eigenpolytope of dimension three, see also \cref{ex:prism}).
Equivalently, if one starts with a polytope, it~is~not guaranteed that this polytope is the eigenpolytope of its edge-graph (or even combinatorially equivalent to it).

\begin{example}
\label{ex:neighborly_1}
A \emph{neighorly polytope} is a polytope whose edge-graph is the complete graph $K_n$.
The spectrum of $K_n$ is $\{(-1)^{n-1},(n-1)^1\}$.
One checks that~the~eigenpolytopes are a single point (for $\theta_1=n-1$) and the regular simplex of dimension $n-1$ (for $\theta_2=-1$).

Consequently, no neighborly polytope other than a simplex is combinatorially equivalent to an eigenpolytope of its edge-graph.
\end{example}

That a graph and its eigenpolytope translate into each other as well as in the case of the cube in \cref{sec:example} is a very special phenomenon, to which we shall give a name:
%Both situations are very special.
a polytope (or graph) for which this happens, will be called \emph{spectral}\footnote{There was at least one previous attempt to give a name to this phenomenon, namely, in \cite{licata1986surprising}, where it was called \emph{self-reproducing}.}.
We cannot formalize this definition right away, as there is some subtlety we have to discuss first (we give a formal definition in \cref{sec:balanced_spectral}, see \cref{def:spectral}).

\begin{example}
\label{ex:pentagon}
The image below shows two spectral realizations of the 5-cycle $C_5$\footnote{Spectral realizations are essentially defined like eigenpolytopes, assinging coordinates $v_i\in\RR^d$ to each vertex $i\in V$ (as in \cref{def:eigenpolytope}), but without taking the convex hull. Instead, one draws the edges between adjacent vertices.}.
%
\begin{center}
\includegraphics[width=0.4\textwidth]{img/C5}
\end{center}
%
The left image~shows the realization to the second-largest eigenvalue $\theta_2$, the right image shows the realization to the smallest eigenvalue $\theta_3$.
In both cases, the convex hull (the actual eigenpolytope) is a regular pentagon, whose edge-graph is $C_5$ again.
But we see that only in the case of $\theta_2$ the edges of the graphs get properly mapped into the edges of the pentagon.

While it is true that the 5-cycle $C_5$ is the edge-graph of its $\theta_3$-eigenpolytope, the adjacency informations gets scrambled in the process:
while, say, vertex 1 and 2 are adjacent in $C_5$, their images $v_1$ and $v_2$ do not form an edge in the $\theta_3$-eigenpolytope.
We do not want to call this \enquote{spectral}, as the adjacency information is not preserved.

The same can happen in higher dimensions too, \eg\ with $G$ being the edge-graph of the dodecahedron:
%
\begin{center}
\includegraphics[width=0.55\textwidth]{img/dodecahedron_eigenpolytopes_2}
\end{center}

\end{example}


%\begin{definition}
%Let $P\subset\RR^d$ be a polytope, and $G=(V,E)$ a graph.
%\begin{myenumerate}
%\item $P$ is said to be  \emph{$\theta$-spectral} (or just \emph{spectral}) if it is the $\theta$-eigenpolytope of its edge-graph (up to scale and orientation)\footnote{One could think of a weaker version where we require that the polytope is only \emph{combinatorially equivalent} to the eigenpolytope if its edge-graph, but we make not use of this in this paper.}.
%\item $G$ is said to be \emph{$\theta$-spectral} (or just \emph{spectral}) if it is the edge-graph~of~its~$\theta$-eigenpolytope.
%\end{myenumerate}
%\end{definition}

\begin{observation}
\label{res:theta_2_observations}
From studying many examples, there are two interesting observations to be made, both concern $\theta_2$, none of which is rigorously proven: %, and both involve the second-largest eigenvalue $\theta_2$.
%
\begin{myenumerate}
\item
It appears as if only $\theta_2$ can give rise to spectral polytopes/graphs.
At~least, all known examples are $\theta_2$-spectral (see also \cref{q:not_theta_2}). Some considerations on nodal domains make this plausible, but no proof is known in the general case (a proof is known in certain special cases, see \cref{res:edge_transitive_spectral_graph}).
\item
If $i\in V$ is a vertex of $G$, then $v_i$ is not necessarily a vertex of every~eigenpolytope ($v_i$ might end up in the interior of $P_G(\theta)$ or one of its faces).
And even if $v_i,v_j\in\F_0(P_G(\theta))$ are distinct vertices and $ij\in E$ is an edge of $G$, it is still not necessarily true that $\conv\{v_i,v_j\}$ is also an edge of the~eigen\-polytope (as seen in \cref{ex:pentagon}).

However, this seems to be no concern in the case $\theta_2$.
It appears as if all edges of $G$ become edges of the $\theta_2$-eigenpolytope, even if $G$ is not spectral (under mild assumptions on the end vertices of the edge).
In other words, the adjacency information of $G$ gets imprinted on the edge-graph of the $\theta_2$-eigenpolytope, whether $G$ is spectral or not.
This is known to be true only in the case of distance-regular graphs \cite[Theorem 3.3 (b)]{godsil1998eigenpolytopes}, but unproven~in general (see also \cref{q:realizing_edges})
\end{myenumerate}

\end{observation}



%
%\begin{itemize}
%	\item Whenever a polytope is spectral, then it is $\theta_2$-spectral.
%	In other words, this interesting coincidence never happens for any eigenvalue other than $\theta_2$.
%	\item
%	Each edge of a graph gives an edge in the $\theta_2$-eigenpolytope.
%	That is, if $ij\in E(G)$, then $\conv\{v_i,v_j\}$ is an edge of $P_G(\theta_2)$.
%\end{itemize}


%The eigenpolytope construction can be approached from two direction:
%first, one already has a graph, and wonders what polytopes will emerge as its eigenpolytopes and what this tells us about the graph.
%Second, we are given a polytope, and we wonder whether it is the eigenpolytope of a graph.


%
%\begin{theorem}
%Every combinatorial symmetry of $G$ is a Euclidean symmetry of any eigenpolytope.
%More precisely, if $\sigma\in\Aut(G)\subseteq\Sym(V)$ is a symmetry of $G$, and $\Pi_\sigma\in\Perm(\RR^n)$ is the associated permutation matrix, then
%%
%$$T_\sigma:=M\T ...$$
%\end{theorem}



\subsection{Litarture}

Eigenpolytope were first introduced by Godsil \cite{godsil1978graphs} in 1978.
Godsil proved the existence of a group homomorphism $\Aut(G)\to\Aut(P_G(\theta))$, \ie\, any combinatorial symmetry of the graph translates into a Euclidean symmetry of the polytope.
%
From that, he deduces results about the combinatorial symmetry group of the original graph.


We say more about the group homomorphism: for every $\theta\in\Spec(G)$ we have
%
\begin{theorem}[\!\cite{godsil1978graphs}, Theorem 2.2]
\label{res:realizing_symmetries}
%Let $\theta\in\Spec(G)$ be an eigenavlue of $G$ of multiplicity $d$, and~$\Phi\in\RR^{n\x d}$ be the matrix defined in \eqref{eq:eigenpolytope_matrix}.
If $\sigma\in\Aut(G)\subseteq\Sym(n)$ is a symmetry of $G$, and $\Pi_\sigma\in\Perm(\RR^n)$ is the associated permutation matrix, then
%
$$T_\sigma:=\Phi\T \Pi_\sigma \Phi \;\in\; \Ortho(\RR^d),\qquad (\text{$\Phi$ is the eigenpolytope matrix})$$
%
is a Euclidean symmetry of the eigenpolytope $P_G(\theta)$ that also permutes the $v_i$ as~prescribed by $\sigma$, \ie\ $T_\sigma\circ \phi = \phi\circ\sigma$, or $T_\sigma v_i = v_{\sigma(i)}$ for all $i\in V$.
%
%\begin{proof}
%\TODO
%\end{proof}
\end{theorem}

This result is also proven (more generally for spectral graph realizations) in \cite[Corollary 2.9]{winter2020symmetric}.

\cref{res:realizing_symmetries} explicitly uses that eigenpolytopes are defined using an  \emph{orthonormal} bases rather than any basis of the eigenspace, to conclude that the symmetries $T_\sigma$ are \emph{orthogonal} matrices.
%From that, Godsil deduced results about the combinatorial symmetry group of the original graph.
Also, the statement of \cref{res:realizing_symmetries} is not too satisfying in general, as it can happen that non-trivial~symmetries of $G$ are mapped to the identity transformation.
We not necessarily have $\Aut(G)\cong\Aut(P_G(\theta))$.

Several authors construct the eigenpolytopes of certain famous graphs or graph families.
Powers \cite{powers1986petersen} computed the eigenpolytopes of the \emph{Petersen graph}, which he termed the \emph{Petersen polytopes} (one of which will appear as a distance-transitive polytope in \cref{sec:distance_transitive}).
The same author also investigates eigenpolytopes of general distance-regular graphs in \cite{powers1988eigenvectors}.
In \cite{mohri1997theta_1}, Mohri described the face structure of the \emph{Hamming polytopes}, the $\theta_2$-eigenpolytopes of the Hamming graphs.
Seemingly unknown to the author, these polytopes can also by described as the cartesian powers of regular simplices (also distance transitive, see \cref{sec:distance_transitive}).

There exists a wonderful enumeration of the eigenpolytopes (actually, spectral realizations) of the edge-graphs of all uniform polyhedra in \cite{blueSpectral}. Sadly, this write-up was never published formally.
This provides empirical evidence that every uniform polyhedron % (including the Platonic solids, Archimedean solids, prisms and anti-prisms)
has a spectral realization.
The same question might then be asked for uniform polytopes in higher dimensions.

Rooney \cite{rooney2014spectral} used the combinatorial structure of the eigenpolytope (the size of their facets) to deduce statements about the size of cocliques in a graph.

In \cite{padrol2010graph}, the authors investigates how common graph operations translate to operations on their eigenpolytopes.

Particular attention was given to the eigenpolytopes of distance-regular graphs \cite{powers1988eigenvectors,godsil1998eigenpolytopes,godsil1995euclidean}.
It was shown that in a $\theta_2$-eigenpolytope of a distance-regular graph~$G$,~every edge of $G$ corresponds to an edge of the eigenpolytope \cite{godsil1998eigenpolytopes}.
Consequently, $G$~is a spanning subgraph of the edge-graph of the eigenpolytope.
It remains open if the same holds for less regular graphs, \eg\ 1-walk regular graphs or arc-transitive graphs (see also \cref{q:realizing_edges}).

The observation that some polytopes are the eigenpolytopes %(actually, $\theta_2$-eigen\-polytopes) 
of their edge-graph (\ie\ they are \emph{spectral} in our terminology) was made repeatedly, \eg\ in \cite{godsil1995euclidean} and \cite{licata1986surprising}. 
In the latter, this was shown for all regular polytopes, excluding the exceptional 4-dimensional polytopes, the 24-cell, 120-cell and 600-cell.
This gap was filled in \cite{winter2020symmetric} via general considerations concerning spectral realizations of arc-transitive graphs.
In sum, all regular polytopes are known to be $\theta_2$-spectral.
%In \cite{licata1986surprising} numerical experiments have been undertaken that suggest that other polytopes are $\theta_2$-spectral.

The next major result for spectral polytopes was obtained by Godsil in \cite{godsil1998eigenpolytopes}, where he was able to classify all $\theta_2$-spectral distance-regular graphs (see also \cref{sec:distance_transitive}):

\begin{theorem}[\!\cite{godsil1998eigenpolytopes}, Theorem 4.3]
\label{res:spectral_distance_regular_graphs}
Let $G$ be distance-regular. 
If $G$ is $\theta_2$-spectral,~then $G$ is one of the following:
%
\begin{enumerate}[label=$(\text{\roman*}\,)$]
	\item a cycle graph $C_n,n\ge 3$,
	\item the edge-graph of the dodecahedron,
	\item the edge-graph of the icosahedron,
	\item the complement of a disjoint union of edges,
	\item a Johnson graph $J(n,k)$,
	\item a Hamming graph $H(d,q)$,
	\item a halved $n$-cube $\nicefrac12 Q_n$,
	\item the Schläfli graph, or
	\item the Gosset graph.
\end{enumerate}
\end{theorem}

A second look at this list reveals a remarkable \enquote{coincidence}: while the generic distance-regular graph has few or no symmetries, all the graphs in this list are highly symmetric, in fact, \emph{distance-transitive} (a definition will be given in \cref{sec:distance_transitive}).

It is a widely open question whether being spectral is a property solely reserved for highly symmetric graphs and polytopes (see also \cref{q:trivial_symmetry}).
There is only a single known spectral polytope that is not vertex-transitive (see also \cref{rem:edge_not_vertex} and \cref{q:spectral_non_vertex_transitive}).







\section{Balanced and spectral polytopes}
\label{sec:balanced_spectral}

In this section we give a second  approach to \emph{spectral polytopes} that circumvents the mentioned subtleties.

For the rest of the paper, let $P\subset\RR^d$ denote a full-dimensional polytope in~dimen\-sion $d\ge 2$ with vertices $v_1,...,v_n\in\F_0(P)$.
We disinguish the \emph{skeleton} of $P$, which is the graph with vertex set $\F_0(P)$ and edge set $\F_1(P)$, from the~\mbox{\emph{edge-graph}}~$G_P=(V,E)$ of $P$, which is isomor\-phic to the skeleton, but has vertex set $V=\{1,...,n\}$. The isomorphism will be denoted
%
\begin{equation}
\label{eq:vertex_map}
\psi:V\ni i\mapsto v_i\in\F_0(P),
\end{equation}
%
and we call it the \emph{skeleton map}.


% and $G_P=(V,E)$ its edge-graph.
%We shall assume that $G_P$ has vertex~set $V=\{1,...,n\}$, and so has so be distinguished from the \emph{skeleton} of $P$, whose vertices and edges are $\F_0(P)$ and $\F_1(P)$ respectively.
%Still, they are isomorphic via some isomorphism
%%
%\begin{equation}
%\label{eq:vertex_map}
%\psi:V\ni i\mapsto v_i\in\F_0(P),
%\end{equation}
%
%Then $v_1,...,v_n\in\F_0(P)$ is an enumeration of the vertices of $P$.

% $G_P=(\F_0(P),\F_1(P))$ its edge-graph with vertex set $V=\{1,...,n\}$, and for all $i\in V$, $v_i\in\F_0(P)$ the associated vertex of $P$.

\subsection{Balanced polytopes}

\begin{definition}
The polytope $P$ is called \emph{$\theta$-balanced} (or just \emph{balanced}) for some~real number $\theta\in\RR$, if
%
\begin{equation}
\label{eq:balanced}
\sum_{\mathclap{j\in N(i)}} v_j = \theta v_i,\quad\text{for all $i\in V$},
\end{equation}
%
where $N(i):=\{j\in V\mid ij\in E\}$ denotes the \emph{neighborhood} of a vertex $i\in V$.
\end{definition}

One way to interpret the balancing condition \eqref{eq:balanced} is as a kind of self-stress~con\-dition on the skeleton of $P$ (the term \enquote{balanced} is motivated from this).
For each edge $ij\in E$, the vector $v_j-v_i$ is parallel to the edge $\conv\{v_i,v_j\}$.
If $P$ is $\theta$-balanced, at each vertex $i\in V$ we have the equation
%
$$\sum_{\mathclap{j\in N(i)}} (v_j-v_i) = \sum_{\mathclap{j\in N(i)}} v_j - \deg(i) v_i = \big(\theta-\deg(i)\big)v_i.$$
%
This equation can be interpreted as two forces that cancel each other out: on the left, a contracting force along each edge (proportion only to the length of that edge), and on the right, a force repelling each vertex away from the origin (proportional to the distance of that vertex from the origin, and proportional to $\theta-\deg(i)$).

%In rigidity theory, one can interpret this line as follows: if each edge is contracting with a force proportional to its length, and each vertex is repelled from the origin with a force propotional to $\theta-\deg(i)$ and its distance from that origin, then $P$ is balanced.

A second interpretation of \eqref{eq:balanced} is via spectral graph theory.
Define the matrix
%
\begin{equation}
\label{eq:arrangement_matrix}
\Psi :=
\begin{pmatrix}
	\;\horzbar\!\!\!\! & v_1\T & \!\!\!\!\horzbar\;\; \\
	& \vdots & \\[0.4ex]
	\;\horzbar\!\!\!\! & v_n\T & \!\!\!\!\horzbar\;\;
\end{pmatrix}
\end{equation}
%
in which the $v_i$ are the rows. 
This matrix will be called the \emph{arrangement matrix} of $P$.
Note that the skeleton map $\psi$ assignes $i\in V$ to the $i$-th row of $\Psi$.
%The definition of $\Psi$ and $\psi$, and their connection, suggests a similarity to the matrix $\Phi$ and the map $\phi$ from \cref{def:eigenpolytope}. We shall come back to that later.
%
Since we use that $P\subset\RR^d$ is full-dimensional,~we have $\rank \Psi=d$.

\begin{observation}\label{res:eigenvalue}
Suppose that $P$ is $\theta$-balanced. 
The defining equation \eqref{eq:balanced} can be equivalently written as the matrix equation $A\Psi=\theta \Psi$.
In this form,~it~is~apparent that $\theta$ is an eigenvalue of the adjacency matrix $A$, and the columns of $\Psi$ are $\theta$-eigenvectors, or $\Span\Psi\subseteq\Eig_{G_P}(\theta)$.
\end{observation}

We have seen that for a balanced polytope, the columns of $\Psi$ must be eigenvectors.
But they are not necessarily a complete set of~$\theta$-eigen\-vectors, \ie\ they not necessarily span the whole eigenspace.

\begin{example}
\label{ex:neighborly}
Every centered neighborly polytope $P$ is balanced, but except if it is a simplex, it is not spectral (the latter was shown in \cref{ex:neighborly_1}).
Centered~means that
%
$$\sum_{i\in V} v_i = 0.$$
%
Since $P$ is neighborly, we have $G_P=K_n$ and  $N(i)=V\setminus\{i\}$ for all $i\in V$. Therefore
%
$$\sum_{\mathclap{j\in N(i)}} v_j = \sum_{\mathclap{j\in V}} v_j - v_i = -v_i,\quad\text{for all $i\in V$}.$$
%
And indeed, $K_n$ has spectrum $\{(-1)^{n-1},(n-1)^1\}$.
So $P$ is $(-1)$-balanced.
\end{example}

The last example shows that every neighborly polytopes can be made balanced by merely translating it.
More generally, many polytopes have a realization (of~their combinatorial type) that is balanced.
But other polytopes do not:

\begin{example}
\label{ex:prism}
Let $P\subset\RR^3$ be a triangular prism.

The spectrum of the edge-graph of $P$ is $\{(-2)^2,0^2,1^1,3^1\}$.
Note that there~is~no eigenvalue of multiplicity greater than~two.
In particular, we cannot choose three linearly independent eigenvectors to a common eigenvalue.
But if $P$ were balanced, then \cref{res:eigenvalue} tells us that the columns of the arrangement matrix $\Psi$ would be three eigenvectors to the same eigenvalue (linearly independent, since $\rank \Psi=3$), which is not possible.
And so, no realization of $P$ can be balanced.
\end{example}

\subsection{Spectral graphs and polytopes}

In the extreme case, when the columns of $\Psi$ span the whole eigenspace, we can finally give a compact definition of what we want~to~consider as \emph{spectral}:

\begin{definition}
\label{def:spectral}\quad
%Let $P\subset\RR^d$ be a polytope, and $G$ be a graph.
%
\begin{myenumerate}
	\item A polytope $P$ is called \emph{$\theta$-spectral} (or just \emph{spectral}), if its arrangement matrix $\Psi$ satisfies $\Span \Psi=\Eig_{G_P}(\theta)$.
	\item A graph is said to be \emph{$\theta$-spectral} (or just \emph{spectral}) if it is (isomorphic to) the edge-graph of~a $\theta$-spectral polytope.
\end{myenumerate}
\end{definition}

This definition is now perfectly compatible with our initial motivation for the~term \enquote{spectral} in \cref{sec:def_eigenpolytope}.
%We make some effort to connect the old and new perspective:

%The following corollary shows that everything we have considered $\theta$-spectral so far is collected under this definition.
%On the other hand, the 5-cycle is not $\theta_3$-spectral.
%A $\theta$-eigenpolytope $G$ satisfies $\Span M=\Eig_G(\theta)$ by definition, and so, if $G=G_P$ we have


%\begin{lemma}
%$P$ is $\theta$-spectral if and only if both of the following hold:
%%
%\begin{myenumerate}
%	\item $P$ is linearly equivalent to the $\theta$-eigenpolytope of its edge-graph, and
%	\item this linear map $T\in\GL(\RR^d)$ from $(ii)$ satisfies $\Psi=\Phi T$.
%\end{myenumerate}
%\end{lemma}



\begin{lemma}\quad
\label{res:naive}
\begin{myenumerate}
	\item If a polytope $P$ is $\theta$-spectral, then $P$ is linearly equivalent to the $\theta$-eigenpoly\-tope of its edge-graph (see also \cref{res:naive_polytope}).
	\item If a graph $G$ is $\theta$-spectral, then $G$ is (isomorphic to) the edge-graph of its~$\theta$-eigen\-polytope (see also \cref{res:naive_graph}).
\end{myenumerate}
\end{lemma}



In both cases, the converse is \emph{not} true.
This is intentional, to avoid the problems mentioned in \cref{ex:pentagon}.
Both statement will be proven below by formulating a more technical condition that is then actually equivalent to being spectral.


%\begin{proposition}
%\label{res:naive_polytope}
%Let $P$ be a polytope with arrangement matrix $\Psi$, $G_P$ its edge-graph, $P_{G_P}(\theta)$ the $\theta$-eigenpolytope of its edge-graph, and $\Phi$ the matrix \eqref{eq:eigenpolytope_matrix}~defined for $P_{G_P}(\theta)$ in \cref{def:eigenpolytope}.
%
%Then, the polytope $P$ is $\theta$-spectral {if and only if} $P$ and $P_{G_P}(\theta)$ are linearly equivalent via a linear map $T\in\GL(\RR^d)$ that satisfies $\Phi=\Psi T$.
%\end{proposition}

%This also proves \cref{res:naive} $(i)$.

%
%\begin{proposition}
%\label{res:naive_graph}
%Let $G$ be a graph, $P_G(\theta)=:Q$ its $\theta$-eigenpolytope, $G_Q$ the edge-graph thereof, and $\Phi$ the matrix \eqref{eq:eigenpolytope_matrix} defined for $P_{G}(\theta)$ in \cref{def:eigenpolytope}.
%
%Then, the graph $G$ is $\theta$-spectral if and only if $G$ is isomorphic to the edge-graph of its $\theta$-eigenpolytope via some isomorphism $\sigma:V(G)\to V(G_Q)$ that satisfies $\Phi=\Pi_\sigma \Psi$, where $\Psi$ is the arrangement matrix of some $\theta$-spectral polytope $P$ with edge-graph $G$ .
%\end{proposition}

\begin{proposition}
\label{res:naive_polytope}
A polytope $P$ is $\theta$-spectral if and only if it is linearly equivalent to the $\theta$-eigenpolytope of its edge-graph via some linear map $T\in\GL(\RR^d)$ for which the following diagram commutes:
%
\begin{equation}
\label{eq:diagram_polytope}
\begin{tikzcd}
P \arrow[r, "T"] & P_{G_P}(\theta)                           \\
                 & G_P \arrow[lu, "\psi"] \arrow[u, "\phi"']
\end{tikzcd}
\end{equation}
%
where $\phi$ and $\psi$ denote the eigenpolytope map and skeleton map respectively.
\end{proposition}

%Recall the definitions of $\phi$ and $\psi$.
%The map $\phi:V(G)\to\RR^d\supseteq P_G(\theta)$ from~\eqref{eq:eigenpolytope_map} is defined whenever we compute an eigenpolytope of a graph $G$.
%The map $\psi:V(G_P)$ $\to \F_0(P)$ from \eqref{eq:vertex_map} is defined whenever we have a polytope $P$ and its edge-graph $G_P$.
%These maps enumerate the rows of the matrices $\Phi$ and $\Psi$ respectively.

\begin{proof}%[Proof of \cref{res:naive_polytope}]
By definition, the $\theta$-eigenpolytope of $G_P$ satisfies $\Span \Phi=\Eig_{G_P}(\theta)$, where $\Phi$ is the corresponding eigenpolytope matrix.

Now, by definition, $P$ is $\theta$-spectral if and only if $\Span \Psi = \Eig_{G_P}(\theta)$, where $\Psi$ is its arrangement matrix.
But by \cref{res:same_column_span}, $\Phi$ and $\Psi$ have the same span if and only of their rows are related by some invertible linear map $T\in\GL(\RR^d)$, that is, $\Psi T=\Phi$, or $T\circ \psi=\phi$. The latter expresses exactly that \eqref{eq:diagram_polytope} commutes.
\end{proof}

This also proves \cref{res:naive} $(i)$.
%Proving the equivalent statement for \cref{res:naive} $(ii)$ is more tedious.


\begin{proposition}
\label{res:naive_graph}
A graph $G$ is $\theta$-spectral if and only if the eigenpolytope map~$\phi\:$ $V(G)\to \RR^d$ provides an isomorphism between $G$ and the skeleton of its $\theta$-eigenpoly\-tope $P_G(\theta)$.
%
\begin{proof}
Suppose first that $G$ is $\theta$-spectral.
Then there is a $\theta$-spectral polytope $Q$~with edge-graph~$G_Q=G$ and skeleton map $\psi\:V(G_Q)\to\F_0(Q)$.
By \cref{res:naive} $(i)$, $Q$ is linearly equivalent to $P_G(\theta)$ via some linear map $T\in\GL(\RR^d)$.
%
By \cref{res:naive_polytope}, the eigenpolytope map satisfies $\phi=T\circ \psi$.
Since $T$ induces an isomorphism between the skeleta of $Q$ and $P_G(\theta)$, and $\psi$ is an isomorphism between $G$ and the skeleton of $Q$, we find that $\phi$ must be an isomorphism between $G$ and the skeleton of $P_G(\theta)$.
This shows one direction.



For the converse, suppose that $\phi$ is an isomorphism.
Set $P:=P_G(\theta)$ and let~$G_P$ be its edge-graph with skeleton map $\psi\:V(G_P)\to \F_0(P)$.
Then $\sigma:=\psi^{-1}\circ\phi$ is a graph isomorphism between $G$ and $G_P$.
So, since $G\cong G_P$, each eigenpolytope of $G$ is also an eigenpolytope of $G_P$.
We can therefore choose $P_{G_P}(\theta)=P_G(\theta)$, with corresponding eigenpolytope map $\phi':=\sigma^{-1}\circ\phi$.
In sum, the outer square in the following diagram commutes:
%
\begin{center}
\begin{tikzcd}
G \arrow[r, "\sigma"] \arrow[d, "\phi"'] & G_P \arrow[d, "\phi'"] \arrow[ld, "\psi"'] \\
\mathllap{P:=\,}P_G(\theta) \arrow[r, "\Id"']    & P_{G_P}(\theta)                           
\end{tikzcd}
\end{center}
%
Also, by construction of $\sigma$, the upper triangle commutes.
In conclusion, the lower triangle must commute as well, which is exactly \eqref{eq:diagram_polytope} with $T=\Id$. This proves that $P$~is $\theta$-spectral via \cref{res:naive_polytope}.
Since $G$ is isomorphic to $G_P$, $G$ is $\theta$-spectral.
\end{proof}
\end{proposition}

\noindent
This also proves \cref{res:naive} $(ii)$.



\iffalse

\begin{proposition}
\label{res:naive_graph}
A graph $G$ is $\theta$-spectral if and only if it is isomorphic to the edge-graph~of its $\theta$-eigenpolytope $P:=P_G(\theta)$ via some isomorphism $\sigma\:V(G)\to V(G_P)$ for which the following diagram commutes:
%
\begin{equation}
\label{eq:diagram}
\begin{tikzcd}
G \arrow[rd, "\phi"'] \arrow[r, "\sigma"] & G_P \arrow[d, "\psi"] \\
                                          & P_G(\theta)\mathrlap{\,:=P        }
\end{tikzcd}
\end{equation}
%
\begin{proof}
First, suppose that $G$ is $\theta$-spectral.
By definition, there exists a $\theta$-spectral polytope $Q$ with edge-graph $G_Q=G$, and let $\psi_Q\:V(G_Q)\to\F_0(Q)$ be the map \eqref{eq:vertex_map} (we use subscripts since there will be further such maps).


Since $Q$ is $\theta$-spectral, \cref{res:naive} $(i)$ states that $Q$ and $P_{G_Q}(\theta)=P_G(\theta)= P$ are linearly equivalent via some map $T\in\GL(\RR^d)$.
Let $\psi_P\:V(G_P)\to\F_0(P)$ be~the corresponding map \eqref{eq:vertex_map} for $P$.

We can then define the isomorphism as $\sigma:=\psi_Q\circ T\circ \psi_P^{-1}$ (all involved maps are invertible and preserve adjacency).
The following diagram then commutes:
%
\begin{center}
\begin{tikzcd}
\mathllap{G=\,}G_Q \arrow[r, "\sigma"] \arrow[d, "\psi_Q"'] & G_P \arrow[d, "\psi_P"] \\
Q \arrow[r, "T"']                                               & P\mathrlap{\,=P_G(\theta)}                      
\end{tikzcd}
\end{center}
%
We can now insert the diagonal arrow $\phi\: V(G)\to\RR^d\supseteq P_G(\theta)$ given by \eqref{eq:eigenpolytope_map}.
%
\begin{center}
\begin{tikzcd}
\mathllap{G=\,}G_Q \arrow[r, "\sigma"] \arrow[d, "\psi_Q"'] \arrow[rd, "\phi"] & G_P \arrow[d, "\psi_P"] \\
Q \arrow[r, "T"']                                               & P\mathrlap{\,:= P_G(\theta)}                      
\end{tikzcd}
\end{center}
%
Since $Q$ is spectral, the the lower triangle commutes by \cref{res:naive_polytope}.
Since also the outer square commutes, we find that the upper triangle (which is exactly \eqref{eq:diagram}) commutes as well, and we are done.

For the other direction, suppose that there is an isomorphism $\sigma:V(G)\to V(G_P)$ so that \eqref{eq:diagram} commutes.
Since $G$ and $G_P$ are isomorphic, $P=P_G(\theta)$ can be consider as a $\theta$-eigenpolytope of $G_P$ as well, thus $P=P_{G_P}(\theta)$.

If $\phi$ is the map \eqref{eq:eigenpolytope_map} for the eigenpolytope of $G$, then because $G_P$ uses the same eigenpolytope, $\phi\circ\sigma^{-1}$ is the respective map \eqref{eq:eigenpolytope_map} for the eigenpolytope of $G_P$.
The following diagram then commutes:

\begin{center}
\begin{tikzcd}
G \arrow[rd, "\phi"'] \arrow[r, "\sigma"] & G_P \arrow[rd, "\phi\circ\sigma^{-1}"]  &                 \\
                                            & \mathllap{P=:\,}P_G(\theta) \arrow[r, "\Id"']                    & P_{G_P}(\theta)
\end{tikzcd}
\end{center}
%
We can now insert the vertical arrow $\psi\: V(G_P)\to \F_0(P)$ given by \eqref{eq:vertex_map}.
%
\begin{center}
\begin{tikzcd}
G \arrow[rd, "\phi"'] \arrow[r, "\sigma"] & G_P \arrow[rd, "\phi\circ\sigma^{-1}"] \arrow[d, "\psi"] &                 \\
                                            & \mathllap{P=:\,}P_G(\theta) \arrow[r, "\Id"']                    & P_{G_P}(\theta)
\end{tikzcd}
\end{center}
%
The left triangle is exactly \eqref{eq:diagram}, hence commutes by assumption. 
The outer parallelogram commutes by construction, and so we find that the right triangle commutes as well.
This triangle is exactly \eqref{eq:diagram_polytope} from \cref{res:naive_polytope} with $T=\Id$.
This shows that $P
$ is $\theta$-spectral, and since $G\cong G_P$ is the edge-graph of $P$, we found that $G$ is $\theta$-spectral, and we are done.
\end{proof}
\end{proposition}

\fi

\iffalse

\begin{lemma}
If $P$ is linearly equivalent to the $P_{G_P}(\theta)$, and this linear map $T\in\GL(\RR^d)$ satisfies $\Phi=\Psi T$, then $P$ is $\theta$-spectral.
\end{lemma}



\begin{lemma}
If $G$ is isomorphic to the edge-graph of $P_G(\theta)=:Q$, and the isomorphism $\sigma\:V(G)\to V(G_Q)$ saitsies $\Phi=\Pi_\sigma \Psi$, then $G$ is $\theta$-spectral.
\end{lemma}




\begin{lemma}
\label{res:naive_polytope}
If $P$ is $\theta$-spectral, then $P$ is linearly equivalent to the $\theta$-eigenpolytope of its edge-graph. The converse is not true.

However, $P$ is $\theta$-spectral if and only if $P$ is linearly equivalent to $P_{G_P}(\theta)$ via~some map $T\in\GL(\RR^d)$, and $T$ additionally satisfies $T \phi(i) = \psi(i)$ for all $i\in V$, where~$\phi\:$ $V(G_P)\to\RR^d$ and $\psi\:V(G_P)\to\F_0(P)$ are the maps defined in \eqref{eq:eigenpolytope_map} \resp\ \eqref{eq:vertex_map}.

%We make this more precise: if $G=(V,E)$ with $V=\{1,...,n\}$ is isomorphic to the edge-graph of $P$ via an isomorphism $\phi:V\ni i\mapsto w_i\in\F_0(P)$, and $\psi:V\ni i\mapsto v_i\in\RR^d$ is the map defined in \cref{def:eigenpolytope}, then there is a linear map $T\in\GL(\RR^d)$ between $P$ and $P_G(\theta)$ with $Tw_i=v_i$ for all $i\in V$.
%
\begin{proof}
By definition, the $\theta$-eigenpolytope of $G_P$ satisfies $\Span \Phi=\Eig_{G_P}(\theta)$, where $\Phi$ is as defined in \eqref{eq:eigenpolytope_matrix}.

Now, by definition, $P$ is $\theta$-spectral if and only if $\Span \Psi = \Eig_{G_P}(\theta)$, where $\Psi$ is its arrangement matrix \eqref{eq:arrangement_matrix}.
But by \cref{res:same_column_span}, $\Phi$ and $\Psi$ can have the same span if and only of their rows are related by some invertible linear map $T\in\GL(\RR^d)$, that is, $T\phi(i)=\psi(i)$ for all $i\in V$.

A counterexample for the initial converse was given in \cref{ex:pentagon}.
\end{proof}
\end{lemma}

\begin{corollary}
If $P$ is $\theta$-spectral, then so is $G_P$ and $P_{G_P}(\theta)$.
\end{corollary}

The respective statement for graphs is the following:

\begin{lemma}
\label{res:naive_graph}
If $G$ is $\theta$-spectral, then $G$ is isomorphic to the edge-graph of its $\theta$-eigenpolytope. The converse is not true.

However, $G$ is $\theta$-spectral if and only if it is isomorphic to the edge-graph of its $\theta$-eigenpolytope, and the isomorphism is given by $\phi\:V\to\RR^d$~as~de\-fined in \eqref{eq:eigenpolytope_map}.
%
\begin{proof}
Let $Q:=P_G(\theta)$ be the $\theta$-eigenpolytope of $G$.
Then we try to prove $G\cong G_Q$.

If $G$ is $\theta$-spectral, then there is a $\theta$-spectral polytope $P$ with edge-graph $G_P\cong G$.
By this, $P_{G_P}(\theta)\cong P_G(\theta)=Q$.
By \cref{res:naive_polytope}, $P$ is linearly~equivalent to~$P_{G_P}(\theta)$, hence linearly equivalent to $Q$.
In particular, $G_P\cong G_Q$, and so we found $G\cong G_P\cong G_Q$.

A counterexample for the initial converse was given in \cref{ex:pentagon}.
\end{proof}
\end{lemma}


\fi

\iffalse

\begin{corollary}
\quad
\begin{myenumerate}
	\item If a polytope $P$ is $\theta$-spectral, then it is the $\theta$-eigenpolytope of its edge-graph (up to some invertible linear transformation).
	\item If a graph $G$ is $\theta$-spectral, then it is (isomorphic to) the edge-graph of its $\theta$-eigenpolytope.
	\item If a graph $G$ is $\theta$-spectral, then its $\theta$-eigenpolytope is $\theta$-spectral.
	
\end{myenumerate}
\end{corollary}

\begin{corollary}
\label{res:naive_definition}
If $P$ is $\theta$-spectral, then it is the $\theta$-eigenpolytope of its edge-graph (up to invertible linear transformation).%, in particular, its $\theta$-eigenpolytope is $\theta$-spectral.
%
\begin{proof}
If $P$ is $\theta$-spectral with arrangement matrix $M'$, then by \mbox{\cref{def:spectral} $(i)$} we have $\Span M'=\Eig_{G_P}(\theta)$.
Let further $M$ be the matrix \eqref{eq:eigenpolytope_matrix} used in \cref{def:eigenpolytope} to define the  $\theta$-eigenpolytope of $G_P$.
By definition we have $\Span M=\Eig_{G_P}(\theta)$.

By \cref{res:same_column_span}, since $M$ and $M'$ have the same column span, their rows are related by an invertible linear transformation.
These rows are the vertices of $P$ and $P_{G_P}(\theta)$ respectively, finishing the proof.
\end{proof}
\end{corollary}

The converse of \cref{res:naive_definition} is not true.
This is intentional, since we do not want confiurations as in \cref{ex:pentagon} to be called \enquote{spectral}.
%This also fits perfectly with our intention.

%Also note the following equivalent definitions for being spectral:

\begin{corollary}
\label{res:spectral_graph_naive}
If a graph $G$ is $\theta$-spectral, then $\phi\:V\ni i\mapsto v_i\in\RR^d$ (as \mbox{introduced} in \cref{def:eigenpolytope}) is an isomorphism between $G$ and the edge-graph of $P_G(\theta)$.
That includes
%
\begin{myenumerate}
	\item for all $i\in V$ holds $v_i\in\F_0(P_G(\theta))$.
	\item for distinct $i,j\in V$ holds $v_i\not= v_j$.
	\item $ij\in E$ if and only if $\conv\{v_i,v_j\}\in\F_1(P_G(\theta))$.
%	\item $i\mapsto v_i$ is an isomorphism between $G$ and the edge-graph $P_G(\theta)$.
\end{myenumerate}
%
\begin{proof}
Since $G$ is $\theta$-spectral, it is (isomorphic to) the edge-graph of some $\theta$-spectral polytope $P$.

Recall that $n$ denotes the number of vertices of $G$.
Since $P_G(\theta)$ is the convex hull of $v_1,...,v_n$, $P_G(\theta)$ has at most $n$ vertices, and $\phi$ is surjective.
Since $P_G(\theta)$ is combinatorially equivalent to $P$ (by \cref{res:naive_definition}), $P_G(\theta)$ has exactly $n$ vertices, and $\phi$ must also be injective.
This also shows $(i)$ and $(ii)$.

\end{proof}
\end{corollary}

Note that not every graph that is isomorphic to the edge-graph of its $\theta$-eigenpoly\-tope is also $\theta$-spectral (again, consider \cref{ex:pentagon}).
However, if the isomorphism is the one from \cref{res:spectral_graph_naive}, then this conclusion is valid.


\iffalse

\begin{lemma}
If $P\subset\RR^d$ is a (full-dimensional) polytope, then the following are~equivalent:
%
\begin{myenumerate}
	\item $P$ is $\theta$-spectral,
	\item $P$ is $\theta$-balanced and the eigenvalue $\theta$ has multiplicity $d$.
\end{myenumerate}
%
If $G$ is a graph, then the following are equivalent:
%
\begin{myenumerate}
\setcounter{enumi}{2}
	\item $G$ is $\theta$-spectral,
	\item the $\theta$-eigenpolytope of $G$ is $\theta$-spectral with edge-graph $G$,
	\item $G$ is isomorphic to the edge-graph of its $\theta$-eigenpolytope, with isomorphism $V\ni i\mapsto v_i\in\RR^d$ (as constructed in \cref{def:eigenpolytope}).
\end{myenumerate}
%
\begin{proof}
By \cref{res:eigenvalue}, the balancing equation \eqref{eq:balanced} is equivalent to $\Span M\subseteq\Eig_G(\theta)$.
Recall that the rank~of~$M$~is~$d$.
Now, $\theta$ having multiplicity $d$ (\ie\ $(ii)$) is equivalent to $\dim\Eig_G(\theta)=d=\rank M$. This is then equivalent to $M=\Eig_G(\theta)$ which is $(i)$.

If $G$ is $\theta$-spectral then it is  (isomorphic to) the edge-graph of \emph{some} $\theta$-spectral polytope $P$.
But \cref{res:naive_definition} states that $P$ is (up to linear transformation) the $\theta$-eigenpolytope of its edge-graph, or, since isomorphic, the $\theta$-eigenpolytope of $G$.

\end{proof}
\end{lemma}

\fi

\fi


It is also possible to give a definition of spectral graphs purely in terms of graph theory, without any explicit reference to polytopes:

\begin{lemma}
\label{res:spectral_2}
A graph $G$ is $\theta$-spectral if and only if it satisfies both of the following:
%
\begin{myenumerate}
	\item for each vertex $i\in V$ exists a $\theta$-eigenvector $u=(u_1,...,u_n)\in\Eig_G(\theta)$~whose single largest component is $u_i$, or equivalently,
%
$$\Argmax_{k\in V} u_k = \{i\}.$$
	\item any two vertices $i,j\in V$ form an edge $ij\in E$ in $G$ if and only~if there is a $\theta$-eigenvector $u=(u_1,...,u_n)\in\Eig_G(\theta)$ whose only two largest components are $u_i$ and $u_j$, or equivalently,
%
$$\Argmax_{k\in V} u_k = \{i,j\}.$$
\end{myenumerate}
%
\end{lemma}

This characterization of spectral graphs can be interpreted as follows: a spectral graph can be reconstructed from knowing a single eigenspace, rather than, say, all eigenspaces and their associated eigenvalues.

\begin{proof}[Proof of \cref{res:spectral_2}]


Let $P_G(\theta)\subset\RR^d$ be the $\theta$-eigenpolytope of $G$ with eigenpolytope matrix $\Phi$ and eigenpolytope map $\phi\:V\ni i\mapsto v_i\in\RR^d$.

Since $\Span\Phi=\Eig_G(\theta)$, the eigenvectors $u=(u_1,...,u_n)\in\Eig_G(\theta)$ are exactly the vectors that can be written as $u=\Phi x$ for some $x\in\RR^d$.
If then $e_k\in\RR^n$ denotes the $k$-th standard basis vector, we have
%
$$u_k = \<u,e_k\> = \<\Phi x, e_k\> = \<x,\Phi\T\! e_k\> = \<x, v_k\>.$$
%
Therefore, there is a $\theta$-eigenvector $u=(u_1,...,u_n)\in\Eig_G(\theta)$ with
%
$\Argmax_{k\in V} u_k = \{i_1,...,i_m\}$
%
if and only if there is a vector $x\in\RR^d$ with
%
$$\Argmax_{k\in V} \<x,v_k\> = \{i_1,...,i_m\}.$$
%
But this last line is exactly what it means for $\conv\{v_{i_1},...,v_{i_m}\}$ to be a face of $P_G(\theta)$ $=\conv\{v_1,...,v_n\}$ (and $x$ is a normal vector of that face).

In this light, we can interpret $(i)$ as stating that $v_1,...,v_n$ form $n$ distinct vertices of $P_G(\theta)$, and $(ii)$ as stating that $\conv\{v_i,v_j\}$ is an edge of $P_G(\theta)$ if and only if $ij\in E$.
And this means exactly that $\phi$ is a graph isomorphism between $G$ and the skeleton of $P_G(\theta)$.
By \cref{res:naive_graph}, this is equivalent to $G$ being $\theta$-spectral.
%
%
%
%
%
%
%
%The set of vertices of the $\theta$-eigenpolytope $P:=P_G(\theta)\subset\RR^d$ is a~sub\-set of $\{v_1,...,v_n\}$, where the $v_i$ are as defined in \cref{def:eigenpolytope}.
%
%By the usual definition of \enquote{face of a polytope}, a set of points $\{v_{i_1},...,v_{i_m}\}\subseteq P$ is now the vertex set of a face of the $\theta$-eigenpolytope if and only of there is a vector~$x\in$ $\RR^d$ (a normal vector) with
%%
%$$\Argmax_{k\in V} \<x,v_k\> = \{i_1,...,i_m\}.$$
%%
%If $\Phi$ is the matrix \eqref{eq:eigenpolytope_matrix}, $u=(u_1,...,u_n):=\Phi x$, and $e_k\in\RR^n$ the $k$-th canonical~basis vector, then
%%
%$$\<x,v_k\> = \<x,\Phi\T\! e_k\> = \<\Phi x,e_k\> = \<u,e_k\> = u_k.$$
%%
%And since $x\mapsto u:=\Phi x$ defines an isomorphism between $\RR^d$ and $\Span \Phi=\Eig_G(\theta)$, we found that $\{v_{i_1},...,v_{i_m}\}\subseteq P$ is the vertex set of a face of $P$ if and only if there~is a~$\theta$-eigenvector $u\in\Eig_G(\theta)$ with
%%
%$$\Argmax_{k\in V} u_k = \{i_1,...,i_m\}.$$
%
%By the previous considerations, $(i)$ is equivalent to: the $v_1,...,v_n$ form distinct vertices of $P$; and $(ii)$ is equivalent~to: $\conv\{v_i,v_j\}$ is an edge of $P$ if and only if $ij\in E$.
%In conclusion, $(i)$ and $(ii)$ in combination are equivalent to: the map $\phi\:i\mapsto v_i$ is an isomorphism between $G$ and the skeleton of $P_G(\theta)$.
%By \cref{res:naive_graph}, this is equivalent to $G$ being $\theta$-spectral.
%In still other words, $(i)$ and $(ii)$ combined are equivalent to $G$ being isomorphic to the skeleton of $P$.
\end{proof}




\iffalse

If the graph satisfies  $(i)$ and $(ii)$, then the map $\sigma:=\psi^{-1}\circ\phi:V(G)\to V(G_P)$ is bijective because of $(i)$, and a graph isomorphism because of $(ii)$.
This isomorphism makes \eqref{eq:diagram} commute by definition, and so $G$ is $\theta$-spectral by \cref{res:naive_graph}.


Conversely, if $G$ is $\theta$-spectral, then it is isomorphic to the edge-graph $G_P$ of its $\theta$-eigenpolytope via some isomorphism $\sigma\: V(G)\to V(G_P)$ that makes \eqref{eq:diagram} commute.

We first note that that implies that $P_G(\theta)$ has exactly the vertices $v_1,...,v_n$, which means that $G$ satisfies $(i)$.

Since $\sigma$ and $\psi$ are graph isomorphisms, so is $\psi\circ\sigma$, and since \eqref{eq:diagram} commutes, also $\phi$.
This means $ij\in E$ if and only if $\conv\{\phi(i),\phi(k)\}=\conv\{v_i,v_j\}\in P_G(\theta)$.
This is equivalent to $(ii)$, and we are done.
%








Suppose that $G$ is $\theta$-spectral, then 



We show first that there is a $\theta$-eigenvectors $u=(u_1,...,u_n)\in\Eig_G(\theta)$ with
%
$$\Argmax_{k\in V} u_k=\{i_1,...,i_m\}$$
%
if and only if $\{v_{i_1},...,v_{i_m}\}$ (as defined in \cref{def:eigenpolytope}) is the vertex set of a face~of the $\theta$-eigenpolytope of $G$.
%
%By \cref{res:...} \msays{Here we need that $G$ is isomorphic to the edge-graph of $P_\theta(G)$.}
%A graph is $\theta$-spectral if and only if it is isomorphic to the edge-graph, say $G'$, of its $\theta$-eigenpolytop $P:=P_G(\theta)$.
%Let $\nu\:V(G)\to V(G')$ be the isomorphism.
%%, and the isomorphism is given by $\phi:V\ni i\mapsto v_i\in\RR^d$ (as constructed in \cref{def:eigenpolytope}).
%
Recall that a set $\{v_{i_1},...,v_{i_m}\}\subseteq \F_0(P)$ of vertices is the vertex set of a face of $P$ if and only if there is a vector $x\in\RR^d$ (a normal vector) with
%
$$\Argmax_{k\in V} \<x,v_k\> = \{i_1,...,i_m\}.$$
%
%Let $P=P_G(\theta)$ be the $\theta$-eigenpolytope of $G$, with $v_i$ defined as in \cref{def:eigenpolytope} and arrangement matrix $M\in\RR^{n\x d}$ (see \eqref{eq:arrangement_matrix}).
%
%Recall that $G$ is $\theta$-spectral if and only if it is (isomorphic to
%
%If $G$ is $\theta$-spectral (in the sense of \cref{def:spectral}), then it is~the skeleton of a polytope $P\subset\RR^d$ (its $\theta$-eigenpolytope) with vertex coordinates $v_i$ as constructed in \cref{def:eigenpolytope}, and arrangement matrix $M\in\RR^{n\x d}$ (see \eqref{eq:arrangement_matrix})
%
%Then, $ij\in E$ if and only if $\conv\{v_i,v_j\}$ is an edge of $P$.
%This is equivalent to the existence of a vector $x\in\RR^d$ for which the linear functional $\<x,\free\>$ attains its maximum exactly in $v_i$ and $v_j$.
%
Let $M$ be the arrangement matrix of $P$, set $u=(u_1,...,u_n):=Mx$, and let $e_k\in\RR^n$ be the $k$-th standard basis vector.
Then
%
$$\<x,v_k\> = \<x, M\T\! e_k\> = \<M x, e_k\> =\<u,e_k\> = u_k.$$
%
By $u=Mx$, the $x\in\RR^d$ are in one-to-one correspondence with the $u\in\Span M=\Eig_G(\theta)$, which are exactly the $\theta$-eigenvectors of $G$.
So $\{v_{i_1},...,v_{i_m}\}$ forms a face of $P$ if and only if
%
$$(*)\quad \Argmax_{k\in V} u_k = \Argmax_{k\in V} \<u,v_k\> = \{i_1,...,i_m\},$$

Condition $(i)$ and $(ii)$ are now the version of $(*)$ for vertices and edges of $P$, which correspond to vertices and edges of $G$ via the isomorphism $\phi$.

\fi
%
%\end{proof}

%This characterization of spectral graphs can be interpreted as follows: a spectral graph can be reconstructed from knowing a single eigenspace, rather than, say, all eigenspaces and their associated eigenvalues.
%\cref{res:spectral_2} can be seen as an instruction for the reconstruction.
In practice, to reconstruct a spectral graph from an eigenspace, the steps could be the following: given a subspace $U\subseteq\RR^n$ (the claimed eigenspace), then
%
\begin{myenumerate}
	\item choose any basis $u_1,...,u_d\in\RR^n$ of $U$,
	\item build the matrix $\Phi=(u_1,...,u_d)\in\RR^{n\x d}$ in which the $u_i$ are the columns,
	\item define $v_i$ as the $i$-th \emph{row} of $\Phi$,
	\item define $P:=\conv\{v_1,...,v_n\}\subset\RR^d$ as the convex hull of the $v_i$,
	\item the reconstructed graph $G=G_P$ is then the edge-graph of $P$.
\end{myenumerate}





\subsection{Properties of spectral polytopes}

We discuss two properties of spectral polytopes that make them especially interesting in polytope theory. 

\subsubsection*{Reconstruction from the edge-graph}
\label{sec:spectral_reconstruction}
The edge-graph of a general polytope carries little information about that polytope \ie\ given only its edge-graph, we can often not reconstruct the polytope from this (up to combinatorial equivalence).
Often, one cannot even deduce the dimension of the polytope from its edge-graph.
Reconstruction might be possible in certain special cases, as \eg\ for 3-dimensional polyhedra, simple polytopes or zonotopes.
The spectral polytopes provide another such class.

\begin{theorem}\label{res:reconstruction}
A $\theta_k$-spectral polytope is uniquely~determined by its edge-graph up to invertible linear transformations.
\end{theorem}

The proof is simple: 
every $\theta_k$-spectral polytope is linearly equivalent to the~$\theta_k$-eigenpolytope of its edge-graph (by \cref{res:naive} $(i)$).
Our definition of the \mbox{$\theta_k$-eigen}\-polytope already suggests an explicit procedure to construct it (a script for this~is included in \cref{sec:appendix_mathematica}).
This property of spectral polytopes appears more exciting when applied to graph classes that are not obviously spectral (see \cref{sec:edge_transitive}).

\subsubsection*{Realizing symmetries of the edge-graph}
\label{sec:spectral_symmetries}
Every Euclidean symmetry of a polytope induces a combinatorial symmetry on its edge-graph.
The converse is far from true.
%
Think, for example, about a rectangle that is not a square.
Even worse, it can happen that a polytope does not even have a realization that realizes all the symmetries of its edge-graph (\eg\ the polytope constructed in \cite{bokowski1984combinatorial}).
%Again, spectral polytopes are special in this regard.

We have previously discussed (in \cref{res:realizing_symmetries}) the existence of a homomorphism $\Aut(G)\to\Aut(P_G(\theta))$ between the symmetries of a graph $G$ and the symmetries of its eigenpolytopes.
There are two caveats:
%
\begin{myenumerate}
	\item this is not necessarily an isomorphism, and
	\item it says nothing about the symmetries of the edge-graph of $P_G(\theta)$, as this one needs not to be isomorphic to $G$
\end{myenumerate}
%
Still, it suffices to makes statement of the following form:
if $G$ is vertex-transitive, then so are all its eigenpolytopes.
This might not work with other transitivities, as for example edge-transitivity.

%We have previously discussed (in \cref{res:realizing_symmetries}) that an eigenpolytope of a graph $G$ \enquote{realizes} all the symmetries of $G$.
%This was meant in weak sense: it can happen that non-trivial symmetries of $G$ become trivial symmetries of the eigenpolytope.
%Still, if, for example, $G$ is vertex-transitive, so are all its eigenpolytopes.
%Other symmetries do not translate as well, \eg\ edge-transitivity.

This is no concern for spectral graphs/polytopes:

\begin{theorem} \quad
\label{res:symmetries}
\begin{myenumerate}
	\item If $G$ is $\theta$-spectral, then $P_G(\theta)$ realizes all its symmetries, which includes
%	
	$$\Aut(G)\cong\Aut(P_G(\theta))$$
	%
	 via the map $\sigma\mapsto T_\sigma$ given in \cref{res:realizing_symmetries}, as wells as that $T_\sigma$ permutes the vertices and edges of $P_G(\theta)$ exactly as $\sigma$ permutes the vertices and edges of the graph $G$.
	\item If $P$ is $\theta$-spectral, then $P$ has a realization that realizes all the symmetries~of its edge-graph, namely, the $\theta$-eigenpolytope of its edge-graph.
\end{myenumerate}
	%
%\begin{proof}
%If $G$ is spectral, then the vertices of $P_G(\theta)$ are exactly the $n$ distinct points $v_1,...,v_n$.
%As stated in \cref{res:realizing_symmetries}, $T_\sigma$ permutes the $v_i$ as prescribed by $\sigma$, which now applies to the vertices, and by this, also to the edges.
%A non-trivial symmetry $\sigma\in\Aut(G)$ does not fixes all vertices of $G$, and hence, neither can $T_\sigma$.
%Therefore, the homomorphism $\sigma\mapsto T_\sigma$ is an isomorphism.
%This proves $(i)$.
%
%
%
%\end{proof}

%
%If $G$ is $\theta$-spectral, then $\Aut(G)\cong \Aut(P_G(\theta))$. % via
%%%
%%$$\Aut(G)\ni \sigma \quad \mapsto\quad  \phi\circ \sigma\circ \phi^{-1}\in\Aut(P_G(\theta)),$$
%%%
%%where $\phi$ is the corresponding eigenpolytope map.
%
%In particular, every $\theta$-spectral polytope has a realization that realizes all the symmetries of its edge-graph, namely, the $\theta$-eigenpolytope of its edge-graph.
%
%\begin{proof}
%A homomorphism ... \msays{Here we need that $G$ is isomorphic to the edge graph of $P_G(\theta)$.}
%
%By \cref{res:naive_polytope}, a $\theta$-spectral polytope $P$ is linearly equivalent to $P_{G_P}(\theta)$, and so the latter is a realization of $P$.
%Since $G_P$ is $\theta$-spectral, $P_{G_P}(\theta)$ also realizes all the symmetries of $G_P$ (as proven above).
%\end{proof}
\end{theorem}

This is mostly straight forward, with large parts already addressed in \mbox{\cref{res:realizing_symmetries}}.
The major difference is that for spectral graphs $G$ the eigenpolytope has exactly the distinct vertices $v_1,...,v_n\in\RR^d$.
The statement from \cref{res:realizing_symmetries} that $T_\sigma$~per\-mutes the $v_i$ as prescribed by $\sigma$, then becomes, that $T_\sigma$ permutes the \emph{vertices} as prescribed by $\sigma$, and hence also the edges.
Also, since the $v_i$ are distinct, no non-trivial symmetry $\sigma$ can result in trivial $T_\sigma$, making $\sigma\mapsto T_\sigma$ into a group \emph{isomorphism}.

%This is also seen easily: by \cref{res:realizing_symmetries}, each symmetry of the graph corresponds to a symmetry of the polytope, and every symmetry of the polytope must restrict to a symmetry of the graph.
%In contrast to general eigenpolytope, this time no two vertices of $G$ get mapped to the same point, and so no non-trivial symmetry of $G$ can be mapped to the identity.
%
%\cref{res:realizing_symmetries} gave the explicit map
%%
%$$\Aut(G)\ni\sigma\quad\mapsto \quad T_\sigma:= \Phi\T\Pi_\sigma\Phi\in\Aut(P_G(\theta)).$$
%%
%This can be written as $\sigma\mapsto \phi\circ\sigma\circ\phi^{-1}$, where $\phi$ is the eigenpolytope map.

For part $(ii)$ merely recall that the eigenpolytope $P_{G_P}(\theta)$ is indeed a realization of $P$ by \cref{res:naive} $(i)$.

The major consequence of this is, that for spectral graphs/polytopes also more complicates types of symmetries translate between a polytope and its graph, as \eg\ edge-transitivity (see also \cref{sec:edge_transitive}).

%\begin{theorem}
%\label{res:realizing_symmetries_spectral}
%A $\theta$-spectral polytope $P$ has a realization $P'$ that realizes all~the symmetries of its edge-graph $G_P$, \ie\ $\Aut(G_P)\cong\Aut(P')$.
%
%One such realization $P'=P_{G_P}(\theta)$ is given by the $\theta$-eigenpolytope of $G_P$, and the isomorphism as in \cref{res:realizing_symmetries}.
%
%$$\phi\circ \sigma = T_\sigma \circ\phi.$$
%\end{theorem}
%
%That $P_G(\theta)$ is a realization of $P$ follows from \cref{res:naive_definition}. \TODO



\iffalse

But, we have to be careful: we cannot expect a general statement about symmetries of spectral polytopes, as \eg\ a rectangle and a square are both spectral (since they are linear transformations of each other), but one is apparently more symmetric, if by symmetry we understand a rigid motion.
There are two solutions: either, generalizing symmetries to general invertible linear transformations, or, restricting the polytopes about which we talk.
Both perspectives are equivalent, and we decided to choose the second.

Let us call a polytope \emph{normalized} if $M\T\! M=\Id$ for its arrangement matrix $M$, that is, the columns of $M$ form a orthonormal basis of $\Span M$.
By \cref{res:same_column_span}, every polytope is just one invertible linear transformation away from being normalized.
Also, the way in which we defined eigenpolytopes in \cref{def:eigenpolytope} ensures that they are normalized.
We have the following:

\begin{theorem}
\label{res:realizing_symmetries}
A normalized spectral polytope realizes all the combinatorial symmetries of its edge-graph as Euclidean symmetries.

More precisely, we have the following: if $\sigma\in\Aut(G_P)\subseteq\Sym(V)$ is a combinatorial symmetry of the edge-graph, and $\Pi_\sigma\in\Perm(\RR^n)$ is the associated permutation matrix, then
%
$$T_\sigma:=M\T \Pi_\sigma M \;\in\; \Ortho(\RR^d)$$
%
is a Euclidean symmetry of $P$ that permutes its vertices exactly as $\sigma$ permutes the vertices of $G_P$ (that is $T_\sigma v_i = v_{\sigma(i)}$).
%
%\begin{proof}
%\TODO
%\end{proof}
\end{theorem}

We should mention that this result is more generally true for all eigenpolytopes of a graph and was already proven in \cite[Theorem 2.2]{godsil1978graphs}.
Another proof in the context of spectral graph realizations can be found \cite[Corollary 2.9]{winter2020symmetric}.
%
%Indeed, the statement of \cref{res:realizing_symmetries} is more generally true for all eigenpolytopes as was already proven in \cite[Theorem 2.2]{godsil1978graphs}.
As a general consequence we have that if $G$ is vertex-transitive, then so are all its eigenpolytopes.
This does not extend to other kinds of symmetries, \eg\ edge-transitivity.

However, if $G$ is $\theta$-spectral, then the symmetries of $G$ and its~$\theta$-eigenpolytope translate into each other one-to-one.
For example, $G$ is edge-transitive if and only if $P_G(\theta)$ is.
We make use of this in later sections.

\fi











\section{The Theorem of Izmestiev}
\label{sec:izmestiev}

We introduce our, as of yet, most powerful tool for proving that certain polytopes are $\theta_2$-spectral.
For this, we make use of a more general theorem by Izmestiev \cite{izmestiev2010colin}, first proven in the context of the Colin de Verdière graph invariant.
The proof of this theorem requires techniques from convex geometry, most notably, mixed volumes, which we not address here.
%
We need to introduce some terminology.

%It can be interesting to study the properties that follow from a polytope being balanced or spectral.
%But it is equally interesting and important to actually determine what polytopes are spectral, or can be made spectral while preserving the combinatorial type.
%
%Of course, for each particular polytope it is an easy task to check whether it is balanced/spectral.
%Much harder it is to find other properties of polytopes that imply it being spectral.
%One tool that can be used for this is the following theorem of Izmestiev, first proved in the context of the Colin de Verdiere graph invariant:


%Large groups of polytopes can be recognized as $\theta_2$-spectral with the help of a result of Izmestiev.
%There is a remarkable construction due to Izmestiev \cite{izmestiev2010colin}.

As before, let $P\subset\RR^d$ denote a full-dimensional polytope of dimension $d\ge 2$, with~edge-graph $G_P=(V,E),V=\{1,...,n\}$ and vertices $v_i\in \F_0(P),i\in V$.
Recall, that the \emph{polar dual} of $P$ is the polytope
%
$$P^\circ:=\{x\in\RR^d\mid \<x,v_i\>\le 1\text{ for all $i\in V$}\}.$$
%
We can replace the $1$-s in this definition by variables $c=(c_1,...,c_n)$, to obtain% the following definition:
%
$$P^\circ(c):=\{x\in\RR^d\mid\<x,v_i\>\le c_i\text{ for all $i\in V$}\}.$$
%
The usual polar dual is then $P^\circ=P^\circ(1,...,1)$.

\begin{figure}[h!]
\includegraphics[width=0.85\textwidth]{img/P_dual_2}
\caption{Visualization of $P^\circ(c)$ for different values of $c\in\RR^n$.}
\end{figure}

In the following, $\vol(\free)$ denotes the volume of convex sets in $\RR^d$ (\wrt\ the usual Lebesgue measure).
Note that the function $\vol(P^\circ(c))$ is differentiable in $c$, and so we can compute partial derivatives \wrt\ the components of $c$.


\begin{theorem}[Izmestiev \cite{izmestiev2010colin}, Theorem 2.4]\label{res:izmestiev}
%Let $P\subset\RR^d$ be a polytope, $G_P$ its~edge-graph and $v\:V\to\RR^d$ its skeleton. 
%For $c=(c_1,...,c_n)\in\RR^n$ define
%%
%$$P^\circ(c):=\{x\in\RR^d\mid\<x,v_i\>\le c_i\text{ for all $i\in V$}\}.$$
%%
%Note that $P^\circ=P^\circ(1,...,1)$ is the polar dual of $P$.
Define a matrix $X\in\RR^{n\x n}$ with~compo\-nents
%
$$X_{ij}:=-\frac{\partial^2 \vol(P^\circ(c))}{\partial c_i\partial c_j}\Big|_{c=(1,...,1)}.$$
%
The matrix $X$ has the following properties:
%
\begin{myenumerate}
	%\item whenever $ij\in E$, and $\sigma_i,\sigma_j\in\F_{d-1}(P^\circ)$ are the dual faces to $v_i$ \resp\ $v_j$ in the dual polytope $P^\circ=P^\circ(1,...,1)$, 
	%then
	%
	%$$X_{ij}=\frac{\vol(\sigma_i\cap\sigma_j)}{\|v_i\|\|v_j\|\sin\angle(v_i,v_j)},$$
	
	\item $X_{ij}< 0$ whenever $ij\in E(G_P)$,
	\item $X_{ij}=0$  whenever $ij\not\in E(G_P)$,
	%\item $X_{ii}> 0$ for all $i\in V(G_P)$,
	\item $X\Psi=0$ (where $\Psi$ is the arrangement matrix of $P$),
	\item $X$ has a unique negative eigenvalue, and this eigenvalue is simple,
	\item $\dim\ker X=d$.
\end{myenumerate}
\end{theorem}

One can view the matrix $X$ as some kind of adjacency matrix of~a vertex- and edge-weighted version of $G_P$.
Part $(iii)$ states that $v$ satisfies a weighted form of the balancing condition \eqref{eq:balanced} with eigenvalue zero.
Since $\rank \Psi=d$, part $(v)$ states that $\Span \Psi$ is already the whole 0-eigenspace.
And part $(iv)$ states that zero is the second smallest eigenvalue of $X$.


\begin{theorem}\label{res:implies_spectral}
Let $X\in\RR^{n\x n}$ be the matrix defined in \cref{res:izmestiev}. 
If we have
%
\begin{myenumerate}
	\item $X_{ii}$ is independent of $i\in V(G_P)$, and
	\item $X_{ij}$ is independent of $ij\in E(G_P)$,
\end{myenumerate}
%
then $P$ is $\theta_2$-spectral.
%
\begin{proof}
By assumption there are $\alpha,\beta\in\RR$, $\beta>0$, so that $X_{ii}=\alpha$ for all vertices~$i\in$ $V(G_P)$, and $X_{ij}=\beta<0$ for all edges $ij\in E(G_P)$ (we have $\beta<0$ by \cref{res:izmestiev} $(i)$).
We can write this as
%
$$X=\alpha \Id + \beta A\quad\implies\quad (*)\;A=\frac\alpha\beta \Id+\frac1\beta X,$$
%
where $A$ is the adjacency matrix of $G_P$.
By \cref{res:izmestiev} $(iv)$ and $(v)$, the matrix $X$ has second smallest eigenvalue zero of multiplicity $d$.
By \cref{res:izmestiev}  $(iii)$, the columns of $M$ are the corresponding eigenvectors.
Since $\rank \Psi=d$ we find that these are all the eigenvectors and $\Span \Psi$ is the 0-eigenspace of $X$.

By $(*)$ the eigenvalues of $A$ are the eigenvalues of $X$, but scaled by $1/\beta$ and shifted by $\alpha/\beta$. Since $1/\beta <0$, the second-\emph{smallest} eigenvalue of $X$ gets mapped onto the second-\emph{largest} eigenvalue of $A$.
Therefore, $A$ (and also $G_P$) has second-largest eigenvalue $\theta_2=\alpha/\beta$ of multiplicity $d$, and $\Span \Psi$ is the corresponding eigenspace.
By definition, $P$ is then the $\theta_2$-eigenpolytope of $G_P$ and is therefore~$\theta_2$-spectral.
\end{proof}
\end{theorem}

It is unclear whether \cref{res:implies_spectral} already characterizes $\theta_2$-spectral polytopes, or even spectral polytopes in general (see also \cref{q:characterization}).

%\begin{corollary}
%Let $P\subset\RR^d$ be a polytope, so that
%%
%\begin{myenumerate}
%	\item its edge-graph is regular,
%	\item it is inscribed,
%	\item all edges are of the same length,
%	\item the ridges of $P^\circ$ have the same volume.
%\end{myenumerate}
%%
%Then $P$ is $\theta_2$-spectral.
%\end{corollary}



\tempnewpage
\section{Edge-transitive polytopes}
\label{sec:edge_transitive}

We apply \cref{res:implies_spectral} to edge-transitive polytopes, that is, to polytopes for~which the Euclidean symmetry group $\Aut(P)\subset\Ortho(\RR^d)$ acts transitively on the edge set $\F_1(P)$.
No classification of edge-transitive polytopes is known.
Some \mbox{edge-transitive} polytopes are listed in \cref{sec:classification}.

Despite the name of this section, we are actually going to address polytopes that are simultaneously vertex- and edge-transitive.
This is not a huge deviation from the title: as shown in \cite{winter2020polytopes}, edge-transitive polytopes in dimension $d\ge 4$ are always also vertex-transitive, and the exceptions in lower dimensions are few (a continuous family of $2n$-gons for each $n\ge 2$, and two exceptional polyhedra).
%The exceptions in lower dimensions are manageable: for $d=3$, there are only two 

%In this section we discuss the class of polytopes that are simultaenously vertex- and edge-transitive.
%This is clearly stronger than being just vertex-transitive.
%However, as shown in \cite{winter2020polytopes}, every edge-transitive polytope in dimendion $d\ge 4$ is also vertex-transitive, and so this distinction only matters for dimension up to three (in which there are only two exceptions, besides polygons).

\cref{res:implies_spectral} can be directly applied to simultaneously vertex- and edge-transitive polytopes, and so we have

\begin{corollary}
\label{res:vertex_edge_transitive_cor}
A simultaneously vertex- and edge-transitive polytope is $\theta_2$-spectral.
\end{corollary}

We collect all the notable consequences in the following theorem:

\begin{theorem}\label{res:edge_vertex_transitive}
If $P\subset\RR^d$ is simultaneously vertex- and edge-transitive, then
%
\begin{myenumerate}
\item $\Aut(P)\subset\RR^d$ is irreducible as a matrix group.
	%\item $\Aut(P)$ is irreducible,
	%\item $P$ is $\theta_2$-spectral, \ie\ $P$ is the $\theta_2$-eigenpolytope of its edge-graph,
%	\item the combinatorial type of $P$ is uniquely determined by its edge-graph, or~more precisely, $P$ is (up to invertible linear transformations) the unique simultaneously vertex- and edge-transitive polytope with~edge-graph $G_P$.
\item $P$ is uniquely determined by its edge-graph up to scale and orientation.\footnote{This shows that $P$ is \emph{perfect}, \ie\ is the unique maximally symmetric realization of its combinatorial type. See \cite{gevay2002perfect} for an introduction to perfect polytopes.}
%\item $P$ is the $\theta_2$-eigenpolytope of its its edge-graph 
%(among simultaneously vertex- and edge-transitive polytopes) 
	\item $P$ realizes all the symmetries of its edge-graph. 
%	\item $P$ is uniquely determined by its edge-graph, in the sense, that it is~the~unique simultaneously vertex- and edge-transitive polytope (up to scale and orientation) with edge-graph $G_P$.
%	\item $P$ is the unique simultaneously vertex- and edge edge-transitive realization of its combinatorial type (up to scale and orientation)\,\footnote{A polytope which is the unique most symmetric realization of its combinatorial type is also known as a \emph{perfect} polytope, see \eg\  \cite{gevay2002perfect}.}\!.
	\item if $P$ has edge length $\ell$ and circumradius $r$, then
	%
	\begin{equation}
	\label{eq:circumradius}
	\frac{\ell}r = \sqrt{\frac{2\lambda_2}{\deg(G_P)}} = \sqrt{2\Big(1-\frac{\theta_2}{\deg(G_P)}\Big)},
	\end{equation}
	%
	where $\deg(G_P)$ is the vertex degree of $G_P$, and $\lambda_2=\deg(G_P)-\theta_2$ denotes its second smallest Laplacian eigenvalue.
	\item if $\alpha$ is the dihedral angle of the polar dual $P^\circ$, then
	%
	\begin{equation}
	\label{eq:dihedral_angle}
	\cos(\alpha)=-\frac{\theta_2}{\deg(G_P)}.	
	\end{equation}
\end{myenumerate}
%
\begin{proof}
The complete proof of $(i)$ and $(ii)$ has to be postponed until \cref{sec:rigidity} (see \cref{res:edge_transitive_rigid}).
Concerning $(ii)$, from \cref{res:vertex_edge_transitive_cor} and \cref{res:reconstruction} already follows that $P$ is determined by its edge-graph up to \emph{invertible linear transformations}, but not necessarily only up to scale and orientation.

Part $(iii)$ follows from \cref{res:symmetries}.
Part $(iv)$ and $(v)$ were proven (in a more general setting) in \cite[Proposition 4.3]{winter2020symmetric}.
This applies literally to $(iv)$.
For $(v)$, note the following: if $\sigma_i\in\F_{d-1}(P^\circ)$ is the facet of the polar dual $P^\circ$ that corresponds to the vertex $v_i\in\F_1(P)$, then the dihedral angle between $\sigma_i$ and $\sigma_j$ is $\pi-\angle(v_i,v_j)$.
The latter expression was proven in \cite{winter2020symmetric} to agree with  \eqref{eq:dihedral_angle}.
\end{proof}
\end{theorem}

It is worth emphasizing that large parts of \cref{res:edge_vertex_transitive} do not apply to polytopes of a weaker symmetry, as \eg\ vertex-transitive polytopes.
Prisms are counterexamples to both $(i)$ and $(ii)$.
There are vertex-transitive neighborly polytopes (other than simplices) and they are counterexamples to $(ii)$ and $(iii)$.

%Finally, every simultaneously vertex- and edge-transitive polytope can be constructed from the edge-graph using only eigenpolytopes (up to scale and orientation). Again, this is not possible for vertex-transitive polytopes (consider a vertex-transitive neighborly polytope that is not a simplex).

%As a consequence, eigenpolytopes can be used to construct essentially all the simultaneously vertex- and edge-transitive polytopes (up to scale and orientation):

%\begin{corollary}
%If $G$ is the edge-graph of a simultaneously vertex- and edge-transi\-tive polytope, then its $\theta_2$-eigenpolytope is vertex- and edge-transitive.
%%
%\begin{proof}
%Let $P$ be a simultaneously vertex- and edge-transitive polytope of which~$G$ is the edge-graph, and let $M$ be its arrangement matrix.
%$\Aut(P)$ acts transitively on $\F_0(P)$, and by \cref{res:edge_vertex_transitive}, $\Aut(P)$ is irreducible.
%
%It is known that if an irreducible matrix group acts transitively on a set of points (as the vertices of $P$), then this implies $M\T \! M=\alpha\Id$ for some $\alpha >0$ (this follows as an application of Schur's Lemma, and was proven \eg\ in \cite[Proposition 4.7]{winter2019geometry} or \cite[Theorem 10.5]{waldron2018introduction}).
%\end{proof}
%\end{corollary}



\iffalse

A simultaneously vertex- and edge-transitive polytope can neither deformed nor projected to keep its edge-graph and symmetry.

The fact that $P$ is perfect can already be proven
 from classical rigidity results and thus can be formulated for a much larger class of polytopes:
 
\begin{theorem}[Alexandrov, \cite{...}]
\label{res:alexandrov_rigidity}
A polyope is uniquely determined (up to orientation) by its combinatorial type and the shape of its facets.
\end{theorem}

\begin{theorem}
An inscribed polytope with all edges of length $\ell$ is uniquely determined (up to orientation) by its combinatorial type.
%
\begin{proof}
The proof is by induction.
A 2-dimensional inscribed polytope with all edges of length $\ell$ ic clearly a regular polygon, hence of unique shape.

Now consider $P$ is a $d$-dimensional inscribed polytope with all edges of length $\ell$.
Then also each facet of $P$ is inscribed with this edge-length.
Also, the combinatorial type of each facet is determined by the combinatorial type of $P$.
By induction assumption, the shape of each facet is hence uniquely determined.
By \cref{res:alexandrov_rigidity} this uniquely determines the shape of $P$.
\end{proof}
\end{theorem}

\begin{corollary}
A simultaneously vertex- and edge-transitive polytope is perfect.
\end{corollary}

\fi

\begin{remark}
\label{rem:edge_not_vertex}
There are two edge-transitive polyhedra that are not vertex-transitive: the \emph{rhombic dodecahedron} and the \emph{rhombic triacontahedron} (see also \cref{fig:edge_transitive}).~Only the former is $\theta_2$-spectral, and the latter is not spectral for any eigenvalue (this was already mentioned in \cite{licata1986surprising}).
Since the rhombic dodecahedron is not vertex-transitive, nothing of this follows from \cref{res:vertex_edge_transitive_cor}.
However, this polytope satisfies the conditions of \cref{res:implies_spectral}, which seems purely accidental.
It is the only known spectral polytope that is not vertex-transitive.
\end{remark}




\subsection{Rigidity and irreducibility}
\label{sec:rigidity}

The goal of this section is to prove the missing part of \cref{res:edge_vertex_transitive}:

\begin{theorem}
\label{res:edge_transitive_rigid}
If $P\subset\RR^d$ is simultaneously vertex- and edge-transitive, then
%
\begin{myenumerate}
	\item $\Aut(P)\subset\Ortho(\RR^d)$ is irreducible as a matrix group, and
	\item $P$ is determined by its edge-graph up to scale and orientation.
	%\item $P$ is the $\theta_2$-eigenpolytope of its edge-graph up to scale and orientation.
\end{myenumerate}
\end{theorem}

To prove \cref{res:edge_transitive_rigid}, we make use of \emph{Cauchy's rigidity theorem} for polyhedra (with its beautiful proof listed in \cite[Section 12]{aigner2010proofs}).
It states that every~polyhedron is uniquely determined by its combinatorial type and the shape of its faces.
This was generalized by Alexandrov to general dimensions $d\ge 3$ (proven \eg\ in \cite[Theorem 27.2]{pak2010lectures}):

\begin{theorem}[Alexandrov]
\label{res:alexandrov}
Let $P_1,P_2\subset\RR^d, d\ge 3$ be two polytopes, so that
%
\begin{myenumerate}
	\item $P_1$ and $P_2$ are combinatorially equivalent via a face lattice~isomorphism~$\phi:\F(P_1)\to\F(P_2)$, and
	\item each facet $\sigma\in\F_{d-1}(P_1)$ is congruent to the facet $\phi(\sigma)\in\F_{d-1}(P_2)$.
\end{myenumerate}
%
Then $P_1$ and $P_2$ are congruent, \ie\ are the same up to orientation.
\end{theorem}

\begin{proposition}
\label{res:regular_rigid}
Let $P_1,P_2\subset\RR^d$ be two combinatorially equivalent polytopes,~each of which has
%
\begin{myenumerate}
	\item all vertices on a common sphere (\ie\ is inscribed), and
	\item all edges of the same length $\ell_i$.
\end{myenumerate}
%
Then $P_1$ and $P_2$ are the same up to scale and orientation.
%
\begin{proof}[Proof.\!\!]\footnote{This proof was proposed by the user \emph{Fedor Petrov} on MathOverflow \cite{petrovMO}.}
W.l.o.g.\ assume that $P_1$ and $P_2$ have the same circumradius, otherwise~re\-scale $P_2$.
It then suffices to show that $P_1$ and $P_2$ are the same up to orientation.

We proceed with induction by the dimension $d$.
The induction base is given by $d=2$, which is trivial, since any two inscribed polygons with constant edge length are regular and thus completely determined (up to scale and orientation) by their number of vertices.

Suppose now that $P_1$ and $P_2$ are combinatorially equivalent polytopes of dimension $d\ge 3$ that satisfy $(i)$ and $(ii)$.
Let $\phi$ be the face lattice isomorphism between them.
Let $\sigma\in\F_{d-1}(P_1)$ be a facet of $P_1$, and $\phi(\sigma)$ the corresponding facet in $P_2$.
In particular, $\sigma$ and $\phi(\sigma)$ are combinatorially equivalent.
Furthermore, both $\sigma$ and $\phi(\sigma)$ are of dimension $d-1$ and satisfy $(i)$ and $(ii)$. This is obvious for $(ii)$, and for $(i)$ recall that facets of inscribed polytopes are also inscribed.
By induction hypothesis, $\sigma$ and $\phi(\sigma)$ are then congruent.
Since this holds for all facets $\sigma\in\F_{d-1}(P_1)$, \cref{res:alexandrov} tells us that $P_1$ and $P_2$ are congruent, that is, the same up to orientation.
\end{proof}
\end{proposition}

We can now prove the main theorem of this section:

\begin{proof}[Proof of \cref{res:edge_transitive_rigid}]
By \cref{res:edge_vertex_transitive} the combinatorial type of $P$ is determined by its edge-graph.
By vertex-transitivity, all vertices are on a sphere.
By edge-transitivity, all edges are of the same length.
We can then apply \cref{res:regular_rigid} to obtain that $P$ is unique up to scale and orientation.
This proves $(ii)$.

Suppose now, that $\Aut(P)$ is not irreducible, but that $\RR^d$ decomposes as $\RR^d=W_1\oplus W_2$ into non-trivial orthogonal $\Aut(P)$-invariant subspaces.
Let $T_\alpha\in\GL(\RR^d)$ be the linear map that acts as identity on $W_1$, but as $\alpha\Id$ on $W_2$ for some $\alpha >1$.
Then $T_\alpha P$ is a non-orthogonal linear transformation of $P$ (in particular, combinatorially equivalent), on which $\Aut(P)$ still acts vertex- and edge-transitively.
By $(ii)$, this cannot be. Hence $\Aut(P)$ must be irreducible, which proves $(i)$.
\end{proof}




\subsection{A word on classification}
\label{sec:classification}

Despite the simple appearance of the definition of an edge-transitive polytope, %(one should have already thought about them, right?), 
no classification was obtained so far.

There exists a classification of the 3-dimension edge-transitive polyhedra: besides the Platonic solids, these are the ones shown in \cref{fig:edge_transitive} (nine in total).

\begin{figure}[h!]
\includegraphics[width=0.75\textwidth]{img/edge_transitive_polyhedra}
\caption{From left to right, these are: the cuboctahedron, the icosido\-decahedron, the rhombic dodecahedron, and the rhombic triacontahedron.}
\label{fig:edge_transitive}
\end{figure}

There are many known edge-transitive polytopes in dimension $d\ge 4$ (so we~are not talking about a class as restricted as the regular polytopes).
There are 15 known edge-transitive 4-polytopes (and an infinite family of duoprisms\footnote{The $(n,m)$-duoprism is the cartesian product of a regular $n$-gon and a regular $m$-gon. Those are edge-transitive if and only of $n=m$. Technically, the 4-cube is the $(4,4)$-duoprism but is usually not counted as such, because of its exceptionally large symmetry group.}), but already here, no classification is known.
It is known that the number of irreducible\footnote{Being not the cartesian product of lower dimensional edge-transitive polytopes.} edge-transitive polytopes grows at least linearly with the number of dimensions.
For example, there are $\lfloor d/2\rfloor$ \emph{hyper-simplices} in dimension $d$.
These are edge-transitive (even distance-transitive, see \cref{sec:distance_transitive}).

It is the hope of the author, that the classification of the edge-transitive polytopes can be obtained using their spectral properties.
Their classification can now be stated purely as a problem in spectral graph theory: 
the classification of the edge-transitive polytopes (in dimension $d\ge 4$) is equivalent to the classification of $\theta_2$-spectral edge-transitive graphs, and since \cref{res:spectral_2}, we have a completely graph theoretic characterization of spectral graphs. %, and the classification can be attacked from this perspective.

%To see this, note the following equivalent definition of \enquote{spectral graph}, not making explicit reference to polytopes:

%\begin{lemma}
%\label{res:spectral_2}
%A graph is $\theta$-spectral if and only if it satisfies both:
%%
%\begin{myenumerate}
%	\item for every vertrex $i\in V$ there is a $\theta$-eigenvector $u=(u_1,...,u_n)\in\RR^n$ with
%%
%$$\Argmax_{k\in V} u_k = \{i\}.$$
%	\item for all distinct vertices $i,j\in V$ we have that $ij\in E$ is an edge of $G$ if and only if there is a $\theta$-eigenvector $u=(u_1,...,u_n)\in\RR^n$ with
%%
%$$\Argmax_{k\in V} u_k = \{i,j\}.$$
%\end{myenumerate}
%\end{lemma}

%\begin{definition}
%\label{def:spectral_2}
%A graph $G$ is said to be \emph{$\theta$-spectral} for some eigenvalue $\theta\in\Spec(G)$, if $ij\in E$ is an edge if and only if there is a $\theta$-eigenvector $u=(u_1,...,u_n)\in\RR^n$ with
%%
%$$\Argmax_{k\in V} u_k = \{i,j\}.$$
%\end{definition}

%\begin{corollary}
%Let $G$ be an edge-transitive $\theta_k$-spectral graph.
%\begin{myenumerate}
%	\item If $G$ is vertex-transitive, then $k=2$.
%	\item If $G$ is not vertex-transitive, then $k=2$ and $G$ is the edge-graph of the rhombic dodecahedron (see \cref{fig:edge_transitive}).
%\end{myenumerate}
%\end{corollary}

\begin{theorem}
\label{res:edge_transitive_spectral_graph}
Let $G$ be an edge-transitive graph. If $G$ is $\theta_k$-spectral, then
\begin{myenumerate}
	\item $k=2$, and
	\item if $G$ is \ul{not} vertex-transitive, then $G$ is the edge-graph of the rhombic dodecahedron (see \cref{fig:edge_transitive}).
\end{myenumerate}
%
\begin{proof}
We first prove $(ii)$.
As shown in \cite{winter2020polytopes} all edge-transitive polytopes in dimen\-sion $d\ge 4$ are vertex-transitive.
If $G$ is edge-transitive, not vertex-transitive and $\theta_k$-spectral, then its $\theta_k$-eigenpolytope is also edge-transitive but not vertex-transitive, hence of dimension $d\le 3$.
One checks that the 2-dimensional spectral polytopes are regular polygons, hence vertex-transitive.
The remaining polytopes are polyhedra, and we mentioned in \cref{rem:edge_not_vertex} that among these, only the rhombic dodecahedron is spectral, in fact $\theta_2$-spectral.
This proves $(ii)$.

Equivalently, if $G$ is vertex- and edge-transitive, then so is its eigenpolytope.
By \cref{res:vertex_edge_transitive_cor} this is a $\theta_2$-eigenpolytope.
Together with part $(ii)$, we find $k=2$~in~all cases, which proves $(i)$.
\end{proof}
\end{theorem}

%\begin{corollary}
%Let $G$ be an edge-transitive graph. If $G$ is $\theta_k$-spectral, then $k=2$. If in addition it is \emph{not} vertex-transitive, then $G$ is the edge-graph of the rhombic dodecahedron (see \cref{fig:edge_transitive}).
%\end{corollary}




\subsection{Arc- and half-transitive polytopes}
\label{sec:arc_transitive}

In a graph or polytope, an \emph{arc} is~an incident vertex-edge-pair.
A graph or polytope is called \emph{arc-transitive} if its symmetry group acts transitively on the arcs.
Being arc-transitive implies both, being vertex-transitive, and being edge-transitive.
In addition to that, in an arc-transitive graph, every edge can be mapped, not only onto every other edge, but also onto itself with flipped orientation.

There exist graphs that are simul\-taneously vertex- and edge-transitive, but not arc-transitive.
Those are called \emph{half-transitive} graphs, and are comparatively rare.
The smallest one has $27$ vertices and is known as the \emph{Holt graph} (see \cite{bouwer1970vertex,holt1981graph}).

For polytopes on the other hand, it is unknown whether there eixsts a distinction being arc-transitive and being simultaneously vertex- and edge-transitive.
No \emph{half-transitive polytope} is known.
Because of \cref{res:edge_vertex_transitive} $(i)$, we know that the edge-graph of a half-transitive polytope must itself be half-transitive.
Since such graphs are rare, the existence of half-transitive polytopes seems unlikely.

\begin{example}
The Holt graph is not the edge-graph of a half-transitive polytope: the Holt graph is of degree four, and its second-largest eigenvalue is of multiplicity six, giving rise to a 6-dimensional $\theta_2$-eigenpolytope. 
But a 6-dimensional polytope must have an edge-graph of degree at least six, and so the Holt graph is not spectral.
\end{example}

The lack of examples of half-transitive polytopes means that all known edge-transitive polytopes in dimension $d\ge 4$ are in fact arc-transitive.
Likewise, a~classification of arc-transitive polytopes is not known.


%The following~result is known about the symmetry group of arc-transitive polytopes:

%\begin{theorem}[\!\cite{winter2020symmetric}, Theorem 4.10]
%If $P\subset\RR^d$ is arc-transitive, then its Euclidean symmetry group $\Aut(P)\subset\Ortho(\RR^d)$ is irreducible.
%\end{theorem}
%
%Here, \enquote{irreducible} is meant in the sense of representation theory, that is, $\RR^d$ is an irreducible subspace of itself \wrt\ the matrix group $\Aut(P)$.
%
%\begin{corollary}
%An arc-transitive polytope $P\subset\RR^d$ is uniquely determined by its edge-graph up to scale and orientation.
%%
%\begin{proof}
%Let $M\in\RR^{n\x d}$ be the arrangement matrix of $P$.
%As shown in \cite[Proposition 4.7]{winter2019geometry} (via Schur's Lemma) if $\Aut(P)$ is irreducible, then $M\T M=\alpha\Id$ for some $\alpha >0$, that is, the columns of $M$ are orthogonal and of the same length.~As~discussed in \cref{sec:choice_of_eigenvectors}, this determines $P$ up to scale and orientation.
%\end{proof}
%\end{corollary}
%



%In an arc-transitive polytope all edges can be flippen.
%
%\begin{theorem}
%If in an arc-transitive polytope $P$ each edge-flip is realized by a reflection, then $P$ is a Wythoffian polytope.
%\end{theorem}




\iffalse

\subsection{Half-transitive polytopes}
\label{sec:half_transitive}

Arc-transitivity implies vertex- and edge-transi\-ti\-vity, but for graphs, the converse is not true.
A graph (and we shall adopt this terminology for polytopes) is called \emph{half-transitive}, if it is both vertex- and edge-transitive, but not arc-transitive.
In a half-transitive graph, each edge can be mapped onto any other edge, but not onto itself with flipped orientation.

The existence of half-transitive graphs was proven first by Holt \cite{holt1981graph}.
Such graphs are relatively rare. The smallest half-transitive graph is now known as the Holt graph and has 27 vertices.

It is not known whether there are any \emph{half-transitive polytopes}.
However, by \cref{res:...} we can now conclude that they are at least as rare as the half-transitive graphs.

\begin{corollary}
The edge-graph of half-transitive polytope must be half-transitive.
\end{corollary}

It is known that the Holt graph is not the edge-graph of a half-transitive polytope.

\fi






\subsection{Distance-transitive polytopes}
\label{sec:distance_transitive}

Our previous results about edge-transitive polytopes already allow for a complete classification of a particular subclass, namely, the \emph{distance-transitive polytopes}, thereby also providing a list of examples of edge-transitive polytopes in higher dimensions.

The distance-transitive symmetry is usually only considered for graphs, and the distance-transitive graphs form a subclass of the distance-regular graphs.
The usual reference for these is the classic monograph by Brouwer, Cohen and Neumaier \cite{brouwer1989distance}.

For any two vertices $i,j\in V$ of a graph $G$, let $\dist(i,j)$ denote the graph-theoretic \emph{distance} between those vertices, that is, the length of the shortest path connecting them.
The \emph{diameter} $\diam(G)$ of $G$ is the largest distance between any two vertices in $G$.

\begin{definition}
A graph is called \emph{distance-transitive} if $\Aut(G)$ acts transitively on each of the sets
%
$$D_{\delta}:=\{(i,j)\in V\times V \mid \dist(i,j)=\delta\},\quad\text{for all $\delta\in\{0,...,\diam(G)\}$}.$$

Analogously, a polytope $P\subset\RR^d$ is said to be \emph{distance-transitive}, if its Euclidean symmetry group $\Aut(P)$ acts transitively on each of the sets 
%
$$D_{\delta}:=\{(v_i,v_j)\in \F_0(P)\times \F_0(P) \mid \dist(i,j)=\delta\},\quad\text{for all $\delta\in\{0,...,\diam(G_P)\}$}.$$
%
Note that the distance between the vertices is still measured along the edge-graph rather than via the Euclidean distance.
\end{definition}

Being arc-transitive is equivalent to being transitive on the set $D_1$.
Hence, distance-transitivity implies arc-transitivity, thus edge-transitivity.

By our considerations in the previous sections, we know that the \mbox{classification} of distance-transitive polytopes is equivalent~to the classification of the $\theta_2$-spectral distance-transitive graphs.
Those where classified by Godsil (see \cref{res:spectral_distance_regular_graphs}).

%By \cref{res:edge_vertex_transitive}, we known that the edge-graph $G_P$ of a distance-transitive polytope must be distance-transitive, and that the polytope is the $\theta_2$-eigenpolytope of $G_P$.
%%
%But Godsil already gave a classification of  $\theta_2$-spectral distance-regular graphs (see \cref{res:spectral_distance_regular_graphs}; all of which~turned out to be distance-transitive) allows a complete classification of distance-tran\-sitive polytopes.

In the following theorem we translated each such $\theta_2$-spectral distance-transitive graph into its respective eigenpolytope.
This gives a complete classification of the distance-transitive polytopes.

\begin{theorem}\label{res:distance_transitive_classification}
If $P\subset\RR^d$ is distance-transitive, then it is one of the following:
%
\begin{enumerate}[label=$(\text{\roman*}\,)$]
	\item a regular polygon $(d=2)$,
	\item the regular dodecahedron $(d=3)$,
	\item the regular icosahedron $(d=3)$,
	\item a cross-polytopes, that is, $\conv\{\pm e_1,...,\pm e_d\}$ where $\{e_1,...,e_d\}\subset\RR^d$ is the standard basis of $\RR^d$,
	\item a hyper-simplex $\Delta(d,k)$, that is, the convex hull of all vectors $v\in\{0,1\}^{d+1}$ with exactly $k$ 1-entries,
	\item a cartesian power of a regular simplex (also known as the Hamming polytopes; this includes regular simplices and hypercubes),
	\item a demi-cube, that is, the convex hull of all vectors $v\in\{-1,1\}^d$ with~an~even number of 1-entries,
	\item the $2_{21}$-polytope, also called Gosset-polytope $(d=6)$,
	\item the $3_{21}$-polytope, also called Schläfli-polytope $(d=7)$.
\end{enumerate}
%
The ordering of the polytopes in this list agrees with the ordering of graphs in the list in \cref{res:spectral_distance_regular_graphs}.
The latter two polytopes where first constructed by Gosset in \cite{gosset1900regular}.
\end{theorem}

We observe that the list in \cref{res:distance_transitive_classification} contains many polytopes that are not regular, and contains all regular polytopes excluding the 4-dimensional exceptions, the 24-cell, 120-cell and 600-cell.
The distance-transitive polytopes thus form a distinct class of remarkably symmetric polytopes which is not immediately related to the class of regular polytopes.

Another noteworthy observation is that all the distance-transitive polytopes are \emph{Wythoffian poly\-topes}, that is, they are orbit polytopes of finite reflection groups.
\Cref{fig:distance_transitive_Coxeter} shows the Coxeter-Dynkin diagrams of these polytopes.

\begin{figure}
\centering
\includegraphics[width=0.9\textwidth]{img/distance_transitive_Coxeter}
\caption{Coxeter-Dynkin diagrams of distance-transitive polytopes.}
\label{fig:distance_transitive_Coxeter}
\end{figure}







\iffalse

Finally, we can show that \cref{res:distance_transitive_classification} is the final word on distance-transitive (actually distance-regular) graphs that are spectral: we can show that such a graph cannot be $\theta_k$-spectral for any $k\not=2$.

\begin{theorem}
\label{res:distance_regular_theta_k}
If $G$ is distance-transitive (actually distance-regular) and $\theta_k$-spectral, then $k=2$.
\end{theorem}

The proof uses some special properties of distance-transitive (actually distance-regular graphs) that we are citing in place.
In general, we recommend the chapters 11 and 13 of \cite{godsil1993algebraic}, the latter of which contains all the tools we need.

\begin{proof}[Proof of \cref{res:distance_regular_theta_k}]

The $\theta_1$-eigenpolytope of any graphs is a single point.
Since we generally assumed that our polytopes ar non-trivial, \ie\ of dimension $d\ge 2$, we from now on assume $k\ge 2$.

Let~$v_i\in$ $\RR^d$ be the coordinates assigned to the vertices $i\in V$ of $G$ as given~in~\cref{def:eigenpolytope}.
We know that the arrangement of the points $v_i$ in $\RR^d$ is as symmetric as the underlying graph, which in the case of distance-transitive graphs means that the value of $\<v_i,v_j\>$ depends only on the distance $\dist(i,j)$ (more generally, the same holds for distance-regular graphs).

We can then define the so-called \emph{cosine sequence} $u_\delta:=\<v_i,v_j\>$ whenever $\dist(i,j)$ $=\delta$.
A well-known result for distance-transitive (actually distance-regular) graphs is, that the sequence $u_0,...,u_{\diam(G)}$ has \emph{exactly} $k-1$ sign changes (see \cite{godsil1993algebraic}, Chapter 13, Lemma 2.1).
It remains to show, that if the $v_i$ embedd $G$ as the skeleton of a polytope, then there can be at most one signs change, hence $k=2$.
%
\begin{center}
\includegraphics[width=0.4\textwidth]{img/5_gon_cut}
\end{center}

This property is occasionally known as the \emph{tightness} of the skeleton of a polytope.
It says that the skeleton cannot be cut into more than two pieces by any hyperplane. 
We give a formal proof below.

Suppose that there are at least two signs changes in $u_\delta$. This means, there exist $\delta>\delta'>0$ with $u_0u_{\delta'}<0$ and $u_{\delta'}u_{\delta}<0$, or equivalently $u_0 > u_\delta > 0 > u_{\delta'}$.
Suppose that the $v_i$ embedd $G$ as the skeleton of a polytope $P$.
Consider the linear optimization problem maximizing the linear functional $\<v_i,\free\>$ over $P$, which clearly attains its maximum in $v_i$.
Let $j\in V$ be a vertex with $\dist(i,j)=\delta$.
Applying the simplex algorithm yields a monotone path in the skeleton from $v_j$ to $v_i$.
But any such path must pass though a vertex $j'\in V$ with $\dist(i,j')=\delta'<\delta$. But we know that $\<v_i,v_{j'}\> = u_{\delta'} < 0 < u_{\delta}$.
So the path cannot have been monotone.
This is a contradiction, showing that there cannot have been two sign changes.
\end{proof}

Whether a similar argument is possible for larger classes of graphs is unknown.

\fi



\iffalse


\tempnewpage

\hrulefill

Let $G=(V,E)$ be a (simple, undirected) graph on the vertex set $V=\{1,...,n\}$.
From any eigenvalue $\theta\in\Spec(G)$ of $G$ (\ie\ of its adjacency matrix $A$)  of multiplicity $d$, we can construct a so-called \emph{spectral realization} (or \emph{$\theta$-realization}) $v\: V\to\RR^d$ of $G$ as follows.
Let $\{u_1,...,u_d\}\subset\RR^n$ be an orthonormal basis of the $\theta$-eigenspace of $G$ and define the \emph{arrangement matrix} $M:=(u_1,...,u_d)\in\RR^{n\x d}$ in which the $u_i$ are the columns.
This matrix has one row per vertex, and so we can obtain a realization $v$ by assigning $i\in V$ to the $i$-th row of $M$:
%
$$M :=
\begin{pmatrix}
	\;\horzbar\!\!\!\! & v_1\T & \!\!\!\!\horzbar\;\; \\
	& \vdots & \\[0.4ex]
	\;\horzbar\!\!\!\! & v_n\T & \!\!\!\!\horzbar\;\;
\end{pmatrix}\mathrlap{\in\RR^{n\times d}.}$$
%
The realization $V\ni i\mapsto v_i$ is called $\theta$-realization of $G$. The $\theta$-realization is unique up to re-orientation (depending only on the choice of the basis $\{u_1,...,u_d\}$).

\begin{definition}
The \emph{$\theta$-eigenpolytope} $P_G(\theta)$ of a graph $G$ is the convex hull of the $\theta$-realization $v$ of $G$:
%
$$P_G(\theta):=\conv\{v_i\mid i\in V\}.$$
\end{definition}



\fi


%To any such graph and any eigenvalue $\theta\in\Spec(G)$ thereof of multiplicity $d$ (\ie\ an eigenvalue of its adjacency matrix), we can associate a $d$-dimensional polytope $P_G(\theta)\subset\RR^d$ as follows: let $u_1,...,u_d\in\RR^n$ be an orthonormal basis of the $\theta$-eigenspace of $G$, and define the matrix $M:=(u_1,...,u_d)\in\RR^{n\x d}$ in which the $u_i$ are the columns.
%Then $M$ as the rows $v_1,...,v_n\in\RR^d$.
%The associated polytope is then given as
%%
%$$P_G(\theta):=\conv\{v_1,...,v_n\}.$$
%%
%This polytope is called the \emph{$\theta$-eigenpolytope} of $G$.




\iffalse

\tempnewpage

\section{The setting}
\label{sec:setting}

Throughout the paper, $P\subset\RR^d$ denotes a $d$-dimensional polytope of full dimen\-sion, that is, $P$ is the convex hull of finitely many points $v_1,...,v_n\in\RR^d$ (its \emph{vertices}), and $P$ is not contained in a proper affine subspace of $\RR^d$.
In particular, we assume the vertice to be labeled with the numbers $1$ to $n$.

By $\F_\delta(P)$, we denote the $\delta$-dimensional faces of $P$, in particular, its vertex set $\F_0(P)$, and its edge set $\F_1(P)$.

By $G_P=(V,E)$ we denote the \emph{edge-graph} of $P$, with vertex set $V=\{1,...,n\}$, so that $i\in V$ corresponds to the vertex $v_i\in \F_0(P)$, and each $ij\in E$ correspond to the edge $\conv\{v_i,v_j\}\in\F_1(P)$.
The term vertex (\resp\ edge) will be used for the elements of $V$ and $\F_0(P)$ (\resp\ $E$ and $\F_1(P)$) likewise, but no confusion is to be expected as these are in a one-to-one correspondence.

Finally, there are two matrices of major importance: for every polytope $P\subset\RR^d$ with labeled vertices $v_1,...,v_n$, the matrix
%
$$M :=
\begin{pmatrix}
	\;\horzbar\!\!\!\! & v_1\T & \!\!\!\!\horzbar\;\; \\
	& \vdots & \\[0.4ex]
	\;\horzbar\!\!\!\! & v_n\T & \!\!\!\!\horzbar\;\;
\end{pmatrix}\mathrlap{\in\RR^{n\times d}}$$
%
is called \emph{arrangement matrix} of $P$ (the vertices $v_i$ are the rows of $M$).
The matrix $A\in\{0,1\}^{n\x n}$ with
%
$$A_{ij}=\begin{cases} 1 & \text{if $ij\in E$}\\0&\text{if $ij\not\in E$}\end{cases}$$
%
is the usual \emph{adjacency matrix} of $G_P$.





\section{Two open questions}

Most of this book talks about the relation between polytopes and their edge-graphs.

It is well-known, that not every graphs is the edge-graph of polytope.
Since Steinitz, we know that the edge-graphs of polyhedra (3-dimensional polytopes) are exactly the 3-connected planar graphs, and each such graph determines a single combinatorial type of polytopes.
In contrast, no characterization of polytopes in dimension $d\ge 4$ is known, and even worse, if a graph is an edge-graph, then in general, it tells us little about the polytope.
That means, there can be many combinatorially distinct polytopes with the same edge-graph, even of the same dimension.

As a light in the dark, we have the result of Blind \& Mani (later refined by Kalai), that every \emph{simple} polytope (that is, a $d$-dimensional polytope whose edge-graph is of degree $d$) is uniquely determined by its edge-graph.
Similar results are known for other classes of polytopes, \eg\ zonotopes.
In this paper, we add another class of polyopes to that list: \emph{spectral polytopes}.
Given the definition of spectral polytope, this is not too surprising (it sounds like an algorithm to compute the polytope from its edge-graph), but the interesting bit is in the graphs that turn out to be spectral and which would not have been expected to be uniquely determined otherwise.

For example, consider highly symmetric polytopes.
Each regular polytopes is uniquely determined (among regular polytopes) by itd edge-graph. In other words, there are no two regular polytopes with the same edge-graph.
On the other hand, there are many distinct vertex-transitive polytopes with the same edge-graph (\eg\ any two vertex-transitive $n$-vertex neighborly polytopes).
So regularity is too strong to be interesting, but vertex-transitivity is too weak.
In this paper, we show that edge-transitivity also already gives unique reconstruction from the edge-graph, since they are spectral.


\fi




\iffalse



\tempnewpage
\section{Balanced and spectral polytopes}
\label{sec:balanced}

We now come back to the curious observations, that sometimes, a polytope is the eigenpolytope of its edge-graph.
A polytope with this property will be called \emph{spectral}.
However, for this section, we decided to go a different path, and introduce spectral polytopes from a different perspective: via balanced polytopes.

The overall goal of this section is to investigate how to can find out whether a given polytope already is spectral.







%
%From this section on let $P\subset\RR^d$ denote a full-dimensional polytope (\ie\ $P$ is not contained in a proper subspace of $\RR^d$) with edge-graph $G=(V,E)$ on the vertex~set $V=\{1,...,n\}$, and with skeleton $v\:V\to\RR^d$.

The precursor to spectral polytopes are the balanced polytopes that we introduce now.

\begin{definition}
$P\subset\RR^d$ is called \emph{$\theta$-balanced} (or just \emph{balanced})~for~a~num\-ber $\theta\in\RR$ if
%
\begin{equation}\label{eq:balanced}
\sum_{\mathclap{j\in N(i)}} v_j=\theta v_i,\quad \text{for all $i\in V$}.
\end{equation}
%
The value $\theta$ is actually an eigenvalue of $G$ (see \cref{res:eigenvalue} below).
If the~multi\-plicity of this eigenvalue $\theta$ is exactly $d$, then $P$ is called \emph{$\theta$-spectral} (or just \emph{spectral}).
\end{definition}

\begin{example}
All neighborly polytopes are balanced (if the barycenter of its vertices is the origin).
We can see this as follows:
%
$$\sum_{\mathclap{j\in N(i)}} v_j = -v_i + \underbrace{\sum_{\mathclap{j\in V}} v_j}_{=0} = -v_i.$$
%
Note that the spectrum of $K_n$ is $\{(-1)^{n-1},(n-1)^1\}$, and so $-1$ is indeed the second largest eigenvalue.
\end{example}

\begin{example}
All regular polytope are $\theta_2$-spectral.
This was first shown by Licata and Powers \cite{licata1986surprising} for all regular polytopes excluding the 4-dimensional exceptions (the 24-cell, 120-cell and 600-cell).
For the remaining polytopes this was proven in \cite{winter...} (Theorem ??).
Alternatively, the same follows from \cref{res:edge_vertex_transitive}.

Other polytopes that were recognized as spectral by Licata and Powers were the 
\emph{rhombic dodecahedron}, ... \TODO
\end{example}

\begin{example}
Probably all uniform polytopes have a realization that is spectral.

\end{example}

Note that all these polytopes are spectral to the \emph{second-largest eigenvalue $\theta_2$}.
This is plausible for different reasons, but no proof of this fact is currently known.

\begin{observation}
Nodal domains ...
\end{observation}


Being balanced can be interpreted in at least two different way.
One of which is in terms of rigidity theory (and applies more generally to graph realizations rather than just to skeleta of polytopes).
The other is purely in terms of spectral graph theory.

\begin{remark}
Being $\theta$-balanced can also be interpreted in the context of rigidity theory.
For an edge $ij\in E$, the vector $v_j-v_i$ is pointing from the vertex $v_i$ along the edge $ij$ and can be interpreted as a force pulling $v_i$ along this edge.
At each vertex, the sum of these forces behaves as follows:
%
\begin{equation}\label{eq:self_stress}
\sum_{\mathclap{j\in N(i)}} (v_j-v_i) = \sum_{\mathclap{j\in N(i)}} v_j - \deg(G)v_i =\big(\theta-\deg(G)\big) v_i.
\end{equation}
%
In the language of rigidity theory: if we put the ...

Equation \eqref{eq:self_stress} can also be written as $LM=\theta M$, where $L$ is the Laplacian of $G$.
\end{remark}

\begin{remark}
Let us call a graph \emph{$\theta$-spectral} if it is the edge-graph of a $\theta$-spectral polytope.
We can characterize such graphs purely in the language of spectral graph theory.
%
A graph is $\theta$-spectral if $i,j\in V$ are adjacent in $G$ if and only if there exists a $\theta$-eigenvector $u\in\RR^n$ that is maximized exactly on $i$ and $j$:
%
$$\Argmax_{k\in V} u_k = \{i,j\}.$$
\end{remark}





Now the central observation concerning balanced polytopes, paving the way to spectral polytopes, is the following:

\begin{observation}\label{res:eigenvalue}
The defining equation \eqref{eq:balanced} can be written as $AM=\theta M$, where $A\in\RR^{n\x n}$ (where the matrices $A$ and $M$ are defined as in \cref{sec:setting}).
In this form, it is apparent that $\theta$ is an eigenvalue of $A$, and the columns of $M$ are the corresponding eigenvectors.
\end{observation}

Since $P$ is assumed to have full dimension, the matrix $M$ has rank $d$, \ie\ its columns are linearly independent eigenvectors.
But they not necessarily span the whole eigenspace.
If they do, this is called a spectral polytope:
%In the extreme case, these columns span the whole eigenspaces.
%And this leads us to the definition of a spectral polytope:

\begin{definition}
A $\theta$-balanced polytope $P\subset\RR^d$ is called \emph{$\theta$-spectral} (or just \emph{spectral}), if any of the following equivalent conditions is satisfied:
%
\begin{myenumerate}
	\item $\theta\in\Spec(G_P)$ has multiplicity $d$ (the dimension of $P$),
	\item the columns of $M$ span the $\theta$-eigenspace of $G_P$.
\end{myenumerate}
\end{definition}


\subsection{Applications}

There are at least two interesting facts about spectral polytopes.

\begin{corollary}
A spectral polytope realizes all the symmetries of its edge-graph.
\end{corollary}

\begin{corollary}
A $\theta_2$-spectral polytope is uniquely determined by its edge-graph (among $\theta_2$-spectral polytopes).
\end{corollary}

Of course, $\theta_2$ can be replaced by any $\theta_i$.

\fi


